Shortchanged: Uncovering and Analyzing Intimate Partner Financial Abuse in Consumer Complaints

Digital financial services can introduce new digital-safety risks for users, particularly survivors of intimate partner financial abuse (IPFA). To offer improved support for such users, a comprehensive understanding of their support needs and the barriers they face to redress by financial institutions is essential. Drawing from a dataset of 2.7 million customer complaints, we implement a bespoke workflow that utilizes language-modeling techniques and expert human review to identify complaints describing IPFA. Our mixed-method analysis provides insight into the most common digital financial products involved in these attacks, and the barriers consumers report encountering when doing so. Our contributions are twofold; we offer the first human-labeled dataset for this overlooked harm and provide practical implications for technical practice, research, and design for better supporting and protecting survivors of IPFA.

==> figures/corpus_graphs/corpus-ip.tex <==
\begin{figure*}
    \centering
\includegraphics[width=0.8\textwidth]{figures/corpus_graphs/final_corpus_ip_counts.png}
    \caption{Total count of intimate partner related keywords in our corpus}
    \label{fig:enter-label}
\end{figure*}
% \includegraphics


==> figures/corpus_graphs/resolution-table.tex <==
\begin{table}[]
\begin{tabular}{@{}lr@{}}
\toprule
\textbf{Resolution}                    & \multicolumn{1}{l}{\textbf{Count}} \\ \midrule
Submitted complaint to FSP(s)          & \cellcolor[HTML]{E67C73}243        \\
Submitted complaint to CB(s)           & \cellcolor[HTML]{FBEAE8}82         \\
Not disclosed                          & \cellcolor[HTML]{FCECEA}79         \\
Reported IP to law enforcement         & \cellcolor[HTML]{FFFBFB}56         \\
C paid outstanding fees on FA product  & \cellcolor[HTML]{E4F4EC}44         \\
Took IP to court about FA product      & \cellcolor[HTML]{99D5B8}27         \\
Submitted complaint to CP (incl. FTC)  & \cellcolor[HTML]{5FBE90}14         \\
Gathered evidence of FA (no complaint) & \cellcolor[HTML]{57BB8A}12         \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:resolution}
\end{table}

==> figures/product-attack.tex <==
\begin{subfigure}
    \centering
    \includegraphics[scale=0.45]{figures/corpus_graphs/product-matrixes.png}
    \caption{\small Top 20 products to financial attack mapping identified from \set complaints. Attacks involving physical and digital credit card  are the most prevalent, while unauthorized opening of account in a Complainant (C)'s name is the most common attack type in this set. [\textit{Unspecified}] means not stated clearly or exactly, while, [\textit{Generic}] refers to a collective of general consumer banking products.}
    \vspace{-0.3cm}
    \label{fig:attack-product-matrices}
\end{subfigure}



==> figures/timelines-processes/tables/attacks-table-2.tex <==
% \footnotesize{
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l}
% \hline
% \textit{\textbf{Financial Negligence}} & \begin{tabular}[c]{@{}l@{}}Refusing to agree or cooperate to creating a financial agreement/obligation\\ Ignoring/Reverting on an established financial agreement/obligation\\ Failing to fulfill an established financial agreement/obligation and not informing the target\\ Ignoring requests to remove from credit/debt after established prior agreement\end{tabular} \\ \hline
% \textit{\textbf{Financial Deception}} & \begin{tabular}[c]{@{}l@{}}Lying about willingness to take on a financial agreement/obligation\\ Deceiving the target into believing that IP has removed them from credit/debt account\\ Asking the target for money and lying about its use\\ Assigning debt to the target without their permission and knowledge\\ Tricking target into co-signing on debts by claiming its a requirement\\ Filing taxes under the target's name after separation\\ Lying about or rationalizing theft of financial resources\end{tabular} \\ \hline
% \textit{\textbf{Unauthorized Access and Control of Target's Accounts}} & \begin{tabular}[c]{@{}l@{}}Taking out fraudulent checks to force an account lockout\\ Reporting valid transactions as fraudulent to create an account lockout\\ Intercepting and re-transferring deposits meant for the target to their personal accounts\\ Attempting to interact with FSP to gain access to the target's account and information\\ Attempting to impersonate the target when interacting with the FSP to gain access to the target's account and information\\ Leveraging physical surveillance to identify PIN numbers for ATM use (using cameras)\end{tabular} \\ \hline
% \textit{\textbf{Duress}} & \begin{tabular}[c]{@{}l@{}}Causing duress from the threat of divorce or separation\\ Causing duress by legal threat and legal action\\ Coercion through target's fear of other forms of abuse\\ Taking advantage of financial hardship being faced by the target\end{tabular} \\ \hline
% \textit{\textbf{Unauthorized Use of Financial Assets}} & \begin{tabular}[c]{@{}l@{}}Using credit cards opened under the target’s name to carry out fraudulent activity on \\ others\\ Transferring and holding the target's funds to coerce target into performing some financial action\end{tabular} \\ \hline
% \textit{\textbf{Fraudulent chargebacks}} & \begin{tabular}[c]{@{}l@{}}Disputing valid transactions to block the target from paying bills\\ Submitting insurance claims under the target's name to avoid insurance hits\end{tabular} \\ \hline
% \textit{\textbf{Unauthorized Opening of Accounts}} & \begin{tabular}[c]{@{}l@{}}Unauthorized opening of joint overdraft accounts\\ Unauthorized opening of utility accounts\end{tabular} \\ \hline
% \end{tabular}%
% }}

{\scriptsize
\begin{tabular}{L{0.25\textwidth}L{0.7\textwidth}}
    \toprule
    \textbf{Category} & \textbf{Attack} \\
    \midrule
    Financial negligence & \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Refuse to agree or cooperate to creating a financial agreement/obligation
    \item Ignore/renege on an established financial agreement/obligation
    \item Fail to fulfill an established financial agreement/obligation and not inform the target
    \item Ignore requests to remove target from credit/debt after established prior agreement
    \end{itemize} \\
    \midrule
    Financial deception &  \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Lie about willingness to take on a financial agreement/obligation
    \item Deceive the target into believing that IP has removed them from credit/debt account
    \item Ask the target for money and lying about its use
    \item Assign debt to the target without their permission and knowledge
    \item Trick target into co-signing on debts by claiming its a requirement
    \item File taxes under the target's name after separation
    \item Lie about or rationalizing theft of financial resources
    \end{itemize} \\
    \midrule
    Unauthorized access and control of Target’s accounts & \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Take out fraudulent checks to force an account lockout
    \item Report valid transactions as fraudulent to create an account lockout
    \item Intercept and re-transferring deposits meant for the target to their personal accounts
    \item Attempt to interact with FSP to gain access to the target's account and information
    \item Attempt to impersonate the target when interacting with the FSP to gain access to the target's account and information
    \item Leverage physical surveillance to identify PIN numbers for ATM use (using cameras)
    \end{itemize} \\
    \midrule
    Duress &  \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Cause duress from the threat of divorce or separation
    \item Cause duress by legal threat and legal action
    \item Coerce through target's fear of other forms of abuse
    \item Take advantage of financial hardship being faced by the target
    \end{itemize} \\
    \midrule
    Unauthorized use of financial assets &  \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Use credit cards opened under the target’s name to carry out fraudulent activity on others
    \item Transfer and hold the target's funds to coerce target into performing some financial action
    \end{itemize} \\
    \midrule
    Fraudulent chargebacks &  \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Dispute valid transactions to block the target from paying bills
    \item Submit insurance claims under the target's name to avoid insurance hits
    \end{itemize} \\
    \midrule
    Unauthorized opening of accounts & \begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Open joint overdraft accounts w/o authorization
    \item Open utility accounts w/o authorization
    \end{itemize} \\
    \bottomrule
\end{tabular}
}

==> figures/timelines-processes/tables/attacks-table-3.tex <==
\tiny
\begin{tabular}{L{.165\textwidth}L{.6\textwidth}L{.18\textwidth}}
    \toprule
    \textbf{Financial Process} & \textbf{Financial Attack Description} & \textbf{Attack Type} \\
    \midrule
    \multirow{4}*{Asset/Account Behavior} & Carrying out financial actions under the target's profile without their knowledge & Deception \\
    & Deception around the usage of borrowed or stolen funds & Deception \\
    & Intercepting funds for coercion & Coercion and Duress \\ 
    & Intercepting funds for financial gain & Access + Control \\
    \midrule
    \multirow{9}*{Asset/Debt Ownership} & Actively blocking/reversing previously-made payments on an established financial agreement/obligation & Negligence, Deception \\ 
    & Deceiving target regarding the fulfillment of financial obligations/agreements & Negligence, Deception \\
    & Ignoring/Reverting on an established financial agreement/obligation & Negligence \\
    & Non-compliance with an established financial agreement/obligation (not contacting target) & Negligence \\
    & Refusal to create a financial agreement/obligation & Negligence \\
    & Submitting insurance claims under the target's name & Deception \\
    & Tricking target into signing on financial obligations & Deception, Unfair Attribution \\
    & Unauthorized opening of joint accounts to implicate a target on overdrafts & Unfair Attribution \\
    & Unauthorized opening of phone or utility accounts & Unfair Attribution \\
    \midrule
    \multirow{4}*{\begin{minipage}{.11\textwidth}Customer-Firm Interactions\end{minipage}} & Leveraging duress of financial hardship for coercion & Coercion and Duress \\ 
    & Leveraging fear of other forms of abuse for coercion & Coercion and Duress \\ 
    & Leveraging threats of divorce or separation for coercion & Coercion and Duress \\
    & Leveraging threats of legal action for coercion & Coercion and Duress \\
    \midrule
    \multirow{3}*{Fraud and Disputes}  & Capitalizing on FSP fraud policies to restrict access to financial assets & Access + Control \\
    & Disputing valid transactions to create unanticipated debt & Access + Control, Unfair Attribution \\
    & Unauthorized use of financial assets for carrying out fraudulent activity with other parties & Unfair Attribution \\
    \midrule
    \multirow{2}*{\begin{minipage}{.13\textwidth}Information Release and Authentication\end{minipage}} & Interacting with an FSP to gain unauthorized access to financial accounts and information & Access + Control \\ 
    & Leveraging technologies for surveillance and unauthorized access to financial information (camera) & Access + Control \\
    \bottomrule
\end{tabular}

==> figures/timelines-processes/tables/attacks-table.tex <==
{\footnotesize
\begin{tabular}{L{0.48\textwidth}L{0.48\textwidth}}
\toprule
\textbf{New financial attacks from our analysis} & \textbf{Financial attacks from prior works that were not found in our analysis} \\
\midrule
\begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]
    \item Refusing to agree or cooperate to creating a financial agreement/obligation
    \item Ignoring/Reverting on an established financial agreement/obligation
    \item Failing to fulfill an established financial agreement/obligation and not informing the complainant
    \item 
\end{itemize} & 
\begin{itemize}[nosep, left=0pt,
        before={\begin{minipage}[t]{\hsize}},
        after ={\end{minipage}} ]   
    \item Delete/sell survivor’s digital purchases (e.g., stocks)
    \item Fraudulently report survivor of financial misconduct
    \item Post non-financial harmful content
    \item Post financial information on survivor
    \item Report survivor’s online business/fundraising campaign
    \item Dupe agency to re-direct salary
    \item Falsify/fabricate evidence of online accounts
    \item Recruit third parties to coerce secret financial info
    \item Surveil survivor via financial profiles
    \item Damage/destroy devices of survivor’s friends and family
    \item Steal survivor's financial information by dumpster diving
\end{itemize}\\
\bottomrule
\end{tabular}
}

==> figures/timelines-processes/tables/taxonomy.tex <==
\begin{table}[!t]
    \centering
    \input{figures/timelines-processes/tables/attacks-table-3}
    \caption{An overview of identified financial attacks in the \set, organized by the relevant financial process the attack might involve and the type of attack present.}
    \label{tab:attacks}
\end{table}



==> figures/timelines-processes/tables/topic_modelling.tex <==
\begin{table*}[!ht]
\scriptsize
\centering
\begin{tabular}{p{0.1cm}p{5.4cm}p{3cm}p{3.5cm}}
\toprule
\textbf{ID} & \textbf{Top 5 Class TFIDF Words} & \textbf{Top 3 Entities Mentioned} & \textbf{Suggested Topic} \\ 
\midrule
1 & `payments, paid' `balance' `payment' `money' & account, payment, loan & Payments and Money \\ 
\midrule
2 & `information' `transaction' `consent' `did' `card' & account, card, information & Suspicious and Harmful Activity \\ 
\midrule
3 & `attorney' `complaint' `law' `hire' `civil' & complaint, court, attorney & Legal and Judicial Actions \\ 
\midrule
4 & `police' `documents' `application' `copy' `sent' & account, information, document & Providing Proof for Financial Issue \\ 
\midrule
5 & `payment' `paid' `closed' `balance' `debt' `loan' & account, credit, payment & Payments \\ 
\midrule
6 & `opened' `security' `social' `know' `account' & account, name, security & Descriptions of Opened Accounts \\ 
\midrule
7 & `received' `did' `card' `authorized' `single' `open' & account, card, credit & Denying Responsibility for Financial Issue \\ 
\midrule
8 & `divorce' `ex' `husband' `divorced' `decree' & divorce, debt, name & Divorce, separation, Intimate Partners \\ 
\midrule
9 & `mortgage' `loan' `score' `pay' `home' & credit, loan, debt & Mortgage, Debt, and Loans \\ 
\midrule
10 & `help' `thank' `care' `just' `circumstance' & information, account, company & Emotional Distress and Toll \\ 
\midrule
11 & `report' `reporting' `credit' `removed' `remove' & credit, report, account & Credit Report Inaccuracies \\ 
\midrule
12 & `ex' `wife' `husband' `opened' `knowledge' `fraudulently' & account, name, credit & IPFA/FA \\ 
\midrule
13 & `refused' `called' `times' `calls' `phone' & account, time, call & Refusal of cooperation from other party \\ 
\midrule
14 & `kids' `life' `house' `work' `struggling' & time, house, year & Hardship and Emotional Toll \\ 
\midrule
15 & `document' `evening' `translated' `english' `attached' & name, account, address & Providing Context for Complaint\\
\bottomrule
\end{tabular}%
\caption{Summary of results from Topic Modeling sentences in our IPFA Corpus across 15 clusters. Of particular interest are clusters 8, 9, 10, 12, and 14.}
\label{tab:topic_modeling_sentence}
\end{table*}


==> sections/05_discussion.tex <==
\section{Discussion}

% RQ1. How do customer-authored descriptions of finan-
% cial abuse with digital financial products differentiate it
% from other forms of financial harm?
% • RQ2. What are the self-reported traits of IPFA in
% customer-authored complaints data and how can such
% traits inform improved threat models for financial abuse?
% • RQ3. How might large language modelling techniques
% enable the detection of intimate partner-led financial
% abuse?

% In this paper, we further confirm the short and long term harms of financial abuse in intimate partnerships, finding complainants often distinctly mention the compounding hardships from IPFA. 
% Given this, mitigating the harms of IPFA as \textit{early} as possible is vital in supporting a survivor, and can be greatly benefited from the early detection of IPFA within customer complaints, paired with established security protocols for protecting a survivor's accounts. 
We contributed the first differentiation of intimate partner financial abuse, from elder financial abuse, fraud, and harassment that can aid to identify future instances in customer accounts -- thereby answering our first research question (RQ1). 
We then conducted a sentence-based analysis to extract unique identifiers of specific types of attacks and areas for an intimate adversary to attack -- namely credit and loans (RQ2). 
Such actions clearly have devastating consequences for a survivor and we urge interested parties to invest attention in helping to mitigate such harms. This work suggests one possible workflow towards the goal of collecting possible IPFA cases in large datasets (RQ3.).

We demonstrated the risk factors and impacts surrounding IPFA in complaints language (such as the mention of divorce/separation, and descriptions of hardship), common vectors of abuse, and the possibility for isolating IPFA complaints using language models -- all of which can be leveraged as useful tools for building such a detect-and-act system in financial institutions. 
Further, we provided a robust definition of IPFA, along with an initial dataset of IPFA within customer complaints that can serve as a benchmark for the development of future detection research. 
We highlight several future research opportunities in the remainder of this section along with limitations of our study.

\paragraph{Determining Causality in Datasets.}
Throughout our study, we identified IPFA when it primarily occurs for the complainant themselves (i.e. the intimate partneris an intimate partnerof the complainant themselves, and the complainant is the primary target of abuse). 
However, we also observed cases where IPFA occurs for a trusted party of the complainant. 
From a technology security perspective, these cases pose a significant threat to complainants and should be considered as a possible vector of harm. 
In this study, our aim was to provide a focused, initial set of IPFA complaints, and although these cases are not included, we view these cases as vital for future study. 

We note that it is well-established that LLMs, as reflections of the data on which they are trained, can be biased (e.g., \cite{abid2021persistent, vig2020investigating}). 
This bias may impact the ability of an LLM-based approach to detect IPFA. 
In the case of our particular approach, the LLM's ability to distinguish between cases in which a complainant spoke about their intimate partner as a \textit{shared victim} of financial harm versus cases in which the complainant spoke of their intimate partner as the \textit{cause} of a financial harm, appeared to be key to detecting IPFA complaints.
Consequently, our method may yield fewer cases of IPFA in which the survivor is uncertain that their intimate partner has caused the financial harm and it may be sensitive to particular patterns or forms of accusatory language. 
Additional experimentation is needed to determine if pretrained LLMs can be used to identify cases of \textit{potential} IPFA that do not include accusatory language and to explore how comprehensively LLMs detect IPFA when complainants implicate IPs.
We see fruitful research that explores this challenge further.

\paragraph{Language-Based IPFA Detection.} Given the tools developed in this paper, we suggest further work in developing means of automating language-based detection of IPFA, and pairing it with different protocols for securing common products that are affected by IPFA, such as credit cards or mortgage loans. Securing common products could entail strategies from enforcing additional authentication for the use of vulnerable assets, to additional auditing of consumer transaction data. 

Large Language Models such as BERT are typically trained on a wide variety of data from the internet. Although, the word-embeddings generated through this process can be used across a wide-variety of NLP tasks, they do not have specific context and understanding around financial abuse and IPV literature. As mentioned in~\Cref{sec:relwork}, fine-tuning large language models for different cases of harm and abuse have proven fruitful, and we encourage the development of such models within the context of IPFA. Enacting such an approach may enable the mitigation of \textit{future} harms a survivor may face, and provide means of studying the existing impacts of a case of IPFA in detail.   

% \paragraph{Open Questions from the Behavioral Elements of IPFA} In our work, we identify several traits and patterns of IPFA that open new avenues for further study to better serve survivors. First, 
% we identify several common vectors of abuse occuring, such as the unauthorized opening of financial assets. Further, we define financial abuse as requiring the presence of a present or former 
% interpersonal relationship. With this, we add to a growing body of evidence that in the cases where an interpersonal relationship exists, the threat of financial harm is not guaranteed to stem from an external adversary, but rather an adversary who may have access to a survivor's personal devices and sensitive information. 
% Prior work addressing Technology-enabled abuse in IPV has demonstrated how this enables both simple and complex attacks that bypass the existing threat model for abuse. From this work, we see that similar notions may exist for financial abuse, and further study should be done on how well existing threat models 
% around identity theft and fraud apply to IPFA, given the legal and interpersonal complexities. Similarly, exploration can be done in understanding the 
% potential value of educating both employees interacting with survivors, and survivors themselves, in the ways IPFA can occur and cause harm. Finally, the traits identified may provide foundational steps towards raising flags with respect to compromised assets, and further work may look at 
% understanding \textit{if} such flags can even be raised, and \textit{how} this detection may be acted on, if at all possible.

%{Towards Additional Sensitivity in Asset Opening User-flows.}
% \paragraph{Behavior-Based IPFA Detection.} In our work, we identified the unauthorized opening of assets as a primary vector of financial abuse. 
% Previous work has shown that online consumer banking has focused largely in preventing financial \textit{fraud}\knote{[needs citation]}. 

% We propose that security workflows in digital finance should pay closer attention towards additional forms of verification when new assets are opened. 

% For instance, considering \textit{previous} asset opening behavior when new assets are opened, can provide institutions with ways to differentiate the behavior of \textit{one} identity, even if that identity is being misused by a suvivor's intimate partner. Behavioral biometrics is an emerging field of authentication relying on certain modes of consistent behavior that a user carries out, such as their cadence of typing, moving, or walking \cite{alsaadi2021study}. This form of authentication has been touted and studied for use in authenticating sensitive apps on mobile devices, and has even been considered as a safeguard against technology-enabled identity theft \cite{alzubaidi2016authentication, moskovitch2009identity}. The integration of sensitive behavioral biometrics in asset opening flows may aid in preventing the unauthorized opening of accounts in cases where an abusive intimate partner is not \textit{coercing} the survivor into gaining access, but is attempting to do so without the survivor's knowledge. This is a result of abusive intimate partners being unable to mimic the exact motions of a survivor. No single technique will provide adequate support for these threat models, and hence work must be done in creating mitigations that span across multiple layers of defense. 
\paragraph{Behavioral elements of IPFA.} In our work, we studied financial harm instigated by an adversary who---through their interpersonal relationship with the survivor---abuses physical access to the survivor's personal devices and sensitive personal information. Prior studies have shown that technology-enabled IPV enables attacks that aren't considered in prevalent threat models in the research community. Similarly, our results identify additional considerations that need to be addressed before a framework can be developed to aid IPFA survivors. We highlight the need for further studies to identify more behavioral elements of IPFA and to determine best practices. The traits identified may provide foundational steps towards raising flags with respect to compromised assets, and further work may look at understanding if such flags can even be raised, and how this detection may be acted on. Another important research area is understanding the value of educating customer support employees who interact with survivors, and educating survivors themselves, on the ways IPFA can occur and cause harm.

%\paragraph{Limitations and Future Work.}
\paragraph{Limitations.}
We acknowledge several limitations in our work, such as the size and scope of our IPFA corpus. 
The CFPB dataset itself is often a last-resort resource for customers, and hence represent a population of complainants that may have \textit{already} attempted to resolve harms with respective financial instituitions prior to filing a complaint. 
Consequently, the language used in these complaints, particularly amongst survivors of IPFA, may differ from the language used in complaints submitted earlier in the lifetime of a survivor's experience with financial abuse. 
Despite this, we expect our dataset to provide a good baseline for the development of future datasets ulooking at complaints submitted at different parts of this timeline, and provide a robust set of definitions to do so. 

Further, although we identify certain traits of IPFA within our corpus, we believe this is under-representative of the true breadth of traits that describe IPFA across financial institutions and across different sectors of financial products. 
For building reliable defenses and mitigations of IPFA in digital financial services, we think further study is needed into the different forms of harm and language surrounding self-reported IPFA to identify potential vectors of abuse that may have been missed within this work. 

% Discussion outline 

% Lessons for folks who know IPV 
% 	What have we learned?

% Lessons for designers/researchers
% 	Focus around consent and financial product design 
% 	(CFPB form, where were the pitfalls what questions to ask)

% Lessons for at-risk users
% 	Work on large data sets and IPV work 
% 	Investigate overlap with other at-risk groups? 

% Challenges,
% 	Causality, Intentionality in narrative accounts
% 	Can we gather multiple different sources of information 
% 	Inferences; judgment calls 

% Future work
% 	Behavioural work, customer accounts

% (Takeaways for financial orgs?)


==> sections/05_discussion_new.tex <==
\section{Discussion}
\label{sec:discussion}
\noindent We have provided a first step toward identifying consumer complaints in the CFPB dataset that describe accounts of IPFA through a bespoke workflow leveraging NLP approaches and careful human review (\textbf{RQ1}). 
Our subsequent analysis on the resulting corpus from this workflow helps to measure who submits such online complaints, the abusers they describe, and the reported losses they experience.
Doing so also helps us to identify commonly-reported attacks and responses (\textbf{RQ2}); and in addition, we identified the barriers complainants report experience in their interactions with financial institutions (\textbf{RQ3}). 
Our approach demonstrates that survivors of intimate partner financial abuse are reaching out to consumer complaint services, often with complex service journeys spanning across several digital financial products and attacks.
Here, we reflect on the limitations of our work, reconcile perspectives across the answers we have contributed to our research questions, and discuss areas that HCI researchers, financial service providers, and developers can explore to better service this pressing concern to digital-safety.
%Nevertheless, ample amount more work is required before this suggested approach may become a reality, and we reflect on the further role that financial organizations, product developers and researchers might play in addressing this pervasive, hidden harm.

\paragraph{Limitations.}
\noindent As with any study reliant on self-reported data, customers may over-report specific elements of their financial history due to social desirability bias \cite{bhatia2022complaint}, or to prompt action via evoking an empathetic response to alleviate financial burdens \cite{gambetta2015complaints}.
There is also a potential skew regarding who may choose to write a complaint \cite{joudaki2015using}; people with more negative experiences may be more motivated to do so, while some with extremely negative experiences may fear repercussions or societal stigma that prevent them from doing so \cite{freed_digital_2017, sharp2015review}.
Our primary goal nevertheless was to understand \edit{what specific financial attacks and barriers complainants report experiencing within our dataset.}

% \textit{why} complainants write about specific financial attacks and barriers they report experiencing.

Our dataset is modest compared to some fraud datasets \cite{ftc_data_2013, ftc_explore_2019}, so our results should be interpreted cautiously.
Namely, our keyword proximity assumption may not always apply to actual cases of IPFA or technology-enabled financial abuse, and keyword searches can limit the discovery of new IPFA patterns for survivors who do not use such terms.
The subsequent use of our workflow intends to mitigate this issue, but still relies on the results of keyword-based approaches as a reference set.
Further study is needed to explore different forms of harm and language used in self-reported IPFA.
Our study, while not representative of all survivors, nevertheless, offers a substantial cross-section of survivor accounts to U.S.-based financial institutions, providing valuable insights for institutions dealing with financial abuse concerns, particularly via digital devices.
% As financial services are expected to play a growing role in responding to concerns of financial abuse, it is essential to bolster efforts that help financial institutions be better equipped with anticipating a wide range of different concerns.

\paragraph{Characterizing the IPFA complainant.}
%Our work takes a tentative step towards 
We have augmented the understanding of abusers and complainants in IPFA cases through careful human review involving experts in IPV, financial abuse, and perpetrator behavior. 
Our corpus shows that complainants often do not characterize their experiences as abuse, despite describing behaviors and experiences that meet technology abuse definitions. 
In addition, while the relationship between intimate partners is often described as having ended (e.g., an ex-spouse) complainants are often still entangled in relationships from a legal standpoint (e.g., divorce may be in progress or yet to be initiated) \cite{freed_digital_2017}. 
% These insights suggest that when studying or addressing IPFA, a broad range of complainant language should be anticipated and a focus on the attributes of the complainant experience may prove to be key in identifying supportive services.
\edit{The lack of explicit characterization highlights the importance of scrutinizing attributes of complainant experiences when studying or addressing IPFA in the future. A broad range of complaint language should be anticipated within complaints, but the attributes uncovered should be further tested with alternative data sources; for instance, by studying how the kinds of financial abuse carried out evolve before, during, and after legal involvement for a target. Further analysis along these attributes may prove to be key in identifying appropriate support services.}
We note that
despite our best efforts to be considerate and transparent in our identification approach (\secref{fig:model_pipeline}), there is the potential
%are undeniably ethical tensions in how this approach may unfairly 
to stigmatize or label individuals with language that may only partially describe their experience.
%not used by themselves. 
It is well-established that language models, are reflections of the data on which they are trained, thus mirroring any embedded biases \cite{abid2021persistent, vig2020investigating}.
We note that only a small minority of complainants self-identified their experiences with the self-identification of abuse (\secref{sec:analysis-intro}), or being a survivor of violence, necessitating a careful synthesis of machine learning approaches and human review.
%Our work aimed to shed light on a societal harm that leaves devastating harm in its wake, yet the loss of potential confidentiality or control a survivor may have over their financial products, such as through surveillance, forecasting, and regulation cannot be ignored.
Such bias may be driving the reliance of our identification approach on distinguishing cases in which the complainant spoke of their intimate partner as the \textit{cause} of financial harm from those in which intimate partner is a \textit{shared} survivor of financial harm.
%In the case of our particular approach, our approach to distinguishing between cases in which a complainant spoke about their intimate partner as a \textit{shared} survivor of financial harm versus cases in which the complainant spoke of their intimate partner as the \textit{cause} of a financial harm, appeared to be key to detecting IPFA complaints.
Indeed, our approach method may yield fewer cases of IPFA in which the complainant is not completely aware that their intimate partner has caused the financial harm.
Thus, our model may be sensitive to forms of accusatory language that may not always match how survivors express financial abuse. 
%make sense of their experiences with financial products.
Additional experimentation is needed to determine if pre-trained sentence transformer models can be used to identify cases of \textit{potential} IPFA that do not include accusatory language and to explore how comprehensively language modeling can be used to detect IPFA when complainants implicate intimate partners. \edit{Altogether, our method produces a corpus of complaints that represent a \textit{subsample} of possible IPFA, and more study is required to understand the larger space of self-reported IPFA within complaints. Despite the bespoke nature of our corpus, we observe that it begins to reveal \textit{some} attributes that can be used by both researchers and developers in improving services for targets of IPFA.}

We see fruitful future research that explores this challenge further, such as with supervised approaches. 
Given the relatively small size of our corpus of representative complaints, one possible direction could be to use few-shot learning techniques that rely on fine-tuned sentence transformer models for classifying IPFA \cite{tunstall2022efficient, gao2021simcse} with our corpus as training data. 
Such a model could then replace \textbf{\circled{3}} and \textbf{\circled{4}} in our workflow, and enable iterative model improvement as new complaints involving IPFA are discovered.
Recent study has also shown significant performance increases in language modeling tasks with techniques involving large language models (LLMs), step-by-step reasoning, and rationales \cite{hsieh2023distilling, zhang2023multimodal, huang2022large} in few-shot learning contexts; these techniques, when used with expert reviewers, may prove fruitful in creating an improved supervised model from our corpus. \edit{Automated methods, if sufficiently accurate, can also \textit{augment} existing human-centered support and referral systems for targets, particularly in the scaled triage of possible IPFA; being able to identify such cases at scales may prove fruitful for support organizations in the direct referrals of targets to appropriate resources (i.e. financial, legal, and technology services).}

\paragraph{Understanding how technical attacks build over time.}
We found that the majority of financial attacks reported by complainants mirror the broader set of identity-related crimes \cite{moskovitch2009identity}. 
However, we also identify that financially abusive crimes may be subtle, such as the surreptitious theft of confidential financial information, and the creation of accounts in the complainant's name (\secref{sec:analysis-attacks}).
Finding instances of technology-enabled abuse can be challenging, prompting the creation of bespoke interventions such as security clinics and digital forensic diagnostic tooling \cite{havron_clinical_2019, freed_is_2019}. 
We found that complainants in our corpus were already reaching out to relevant financial institutions concerning the repercussions of technology-enabled financial abuse, even before submitting a complaint to the CFPB.
As such, our work highlights that public datasets that sport customer complaints (e.g., building better businesses), may \edit{reveal valuable insights into the disconnect between provided services by financial insitutions and the needs of complainants}.
We envision complaints submitted \textit{directly} to financial institutions may be another valuable source of information to leverage in characterizing the harms of IPFA, and encourage this as a possible avenue of future work.
Such complaints may provide a rich insight into how accounts may change overtime, across the life-cycle of digital financial products \edit{, allowing for improved monitoring and clarity around the specific financial services and systems affected by different forms of attack.}

Interpersonal relationships can naturally complicate traditional approaches to resolving disputes with digital technologies \cite{levy_privacy_2020}, even in areas that exist outside of abuse.
Namely, couples may have to pool their financial resources to pay for specific assets or experiences (e.g., houses, vacations) which often require shared account access and permissions \cite{park_can_2020} --- with financial services actively encouraging users to do so \cite{HowcanIs54:online}.
Unofficial proxies \cite{latulipe_unofficial_2022} (adults who assist older adults), carers \cite{mentis_upside_2019}, and intimate partners \cite{mcdonald_realizing_2020, Bellini2023paying} also often know the authentication information of those they assist. \edit{In fact, several descriptions of abusive behavior that were found in our corpus, such as the unauthorized opening of accounts, intentional misuse of digital financial resources, and the direct theft of financial capital, have been observed across the context of \textit{other} interpersonal relationships, such as in cases of caretakers and an elder vulnerable individual \cite{black2008not, noauthor_metlife_nodate} as a direct result of this shared access and permission changes.}
Identifying how and when these changes happen over digital financial products with both the common forms of attack across different forms of interpersonal relationships \textit{as well} as the forms of attack that have been highlighted as unique to the intimate partner context may be invaluable to identify when specific digital-safety risks may occur. 
From a service standpoint, this could also be valuable for providers to identify when a vulnerable customer may be more likely to reach out for help.
After all, our workflow is evaluated with a focus on finding consumer complaints involving IPFA \textit{specifically} within CFPB data. 
To assess the efficacy and generalisability of this type of method for finding complaints describing IPFA at large, we suggest that the NLP techniques and human review elements of our workflow in analysing complaints may be valuable to apply to other contexts. \edit{Given the aforementioned commonalities in IPFA and other forms of interpersonal abuse, we suggest that the methods presented here are tested within these other populations, which may provide valuable insights into the role automation and NLP-based techniques can play in identifying, analyzing, and uncovering financial abuse by close or intimate relations generally.}
Alternatively, self-reported accounts on social media platforms may also prove to be rich sources of analysis on issues ranging from self reported accounts of IPV, to descriptions of hate speech \cite{caselli2020hatebert}.
% As such, the discoveries of work around survivors of technology-enabled financial abuse may also have the potential to help those with similar concerns around financial harm by close or intimate relations.


\paragraph{Combating the service barriers of IPFA.}
Scholars have  suggested several strategies to address technology and financial abuse from the perspective of the financial institution, including, an increased focus on training \cite{Bellini2023paying, postmus_building_2023}, improved professional referral pathways \cite{surviving_economic_abuse_conversation_2021} and a refocus on authentication and customer consent \cite{bellini2023digitalsafety}. 
We build on these suggestions by 
%focusing on related areas; namely, the ability to 
collating attack evidence and expanding the understanding of attack timelines.

A major, specific barrier highlighted by our complainants is  the struggle to attain evidence of abuse that is accepted 
%or to have such evidence of abuse or attestation to innocence accepted 
by the necessary institutions (\secref{sec:analysis-barriers}).
Concrete evidence that validates the experience of abuse is  vital to  combating the %extreme forms of harm that are often intersected with 
psychological harm associated with deception and negligence
%abuse 
\cite{postmus_building_2023, sharp2015review}.
%; deception and negligence.
We are nevertheless hesitant to claim that
%cautious to recommend 
an improvement in evidence collection practices could immediately lead to improved outcomes for survivors, as many have already highlighted that the process of collecting evidence can be exhausting if not traumatizing \cite{freed_digital_2017}. 
Indeed, our narratives show that even gaining access to evidence often appeared to be an impossible feat, given that many  organizations lost documentation, failed to respond to requests for information, or did not permit complainants to know particular pieces of information about accounts opened with their information (e.g, social security number).
%We anticipate 
Our analysis demonstrates the need for mechanisms that make information about accounts involving the personal information of
%an attested 
survivors of financial abuse 
%that pertain 
%involving their personal information 
 (e.g., accounts opened in their name)  more easily accessible \cite{havron_clinical_2019}.
%; such as a freedom of information request, or patients requesting health records.
In addition, clarity is needed regarding what constitutes sufficient evidence 
%of these harms is nevertheless far from an easy task as what is considered evidence or proof is 
as our data show this is often contested and nuanced.
%a high degree of nuance is needed to examine pathways that make this a viable option to users who have their digital-safety threatened.

Our work highlights that attacks may vary over time, causing survivors to continuously reach out to different financial institutions about their technology concerns.
%discovery our work points to is understanding the timeline of attacks alongside their nature.
%Specifically, we refer to our discovery that akin 
Similar to survivors of tech abuse, complainants report experiencing a multitude of different types of technology-enabled financial attacks; with features that may overlap and vary in intensity. %often overlapping and intensifying features.
While financial harms such as fraud and scams are often approached on an incident-basis --- a single event that can be delineated into before and after --- we suggest viewing IPFA
%this form of financial harm 
as an on-going, persistent threat more akin to online harassment or hate.
As such, we see the potential in training  financial professionals in not only IPV, but also in providing technical techniques, such as mapping and financial timelines to help customers better contextualize their financial history, and identify specific areas or products that are consistently targeted by abusers at key stages (\figref{fig:attack-product-matrices}).
Although financial institutions are substantially different from service providers of online and digital services \cite{zou_role_2021, Bellini2023paying}, there is a potential to draw broader lessons from their approach to protecting vulnerable users over a longer period of time.
Our work also identifies a lack of clarity around when complainants discover technology enabled financial abuse in IPFA. One possible cause of this could be a lack of explicit direction to address such aspects of IPFA when submitting a complaint. \edit{We observe that the types of technology-enabled financial attacks experienced by a target can evolve with changing circumstances, such as in the case of legal proceedings or added financial impact on a target's children. Guiding complainants to provide details such as point of discovery may be a valuable area of future study, with implications in identifying the \textit{appropriate} means of support for a complainant, based on their circumstances.} Particularly, the results of our analysis, and our corpus, may prove of use to the CFPB, allowing for further study into different ways of intaking information surrounding technology enabled financial abuse that may address information gaps such as discovery.  
% \jnote{Can we make 'online service providers' more specific? Financial institutions also provide online services.}


% In our research on intimate partner financial abuse, we acknowledge several limitations: the size of our dataset, our choice of focus from the CFPB, and the potential lack of representation of all survivors of IPFA.

==> sections/05_discussion_new_two.tex <==
\section{Discussion}
\label{sec:discussion}
\noindent We have provided a first step toward identifying consumer complaints in the CFPB dataset that describe accounts of IPFA through a bespoke workflow leveraging NLP approaches and careful human review (\textbf{RQ1}).
Our subsequent analysis on the resulting corpus from this workflow helps to measure who submits such online complaints, the abusers they describe, and the reported losses they experience.
Doing so also helps us to identify commonly-reported attacks and responses (\textbf{RQ2}); and in addition, we identified the barriers complainants report experience in their interactions with financial institutions (\textbf{RQ3}). 
Our approach demonstrates that survivors of intimate partner financial abuse are reaching out to consumer complaint services, often with complex service journeys spanning across several digital financial products and attacks.
Here, we reflect on the limitations of our work, reconcile perspectives across the answers we have contributed to our research questions, and discuss areas that HCI researchers, financial service providers, and developers can explore to better service this pressing concern to digital-safety.
%Nevertheless, ample amount more work is required before this suggested approach may become a reality, and we reflect on the further role that financial organizations, product developers and researchers might play in addressing this pervasive, hidden harm.

\paragraph{Limitations}
\noindent As with any study reliant on self-reported data, customers may over-report specific elements of their financial history due to social desirability bias \cite{bhatia2022complaint}, or to prompt action via evoking an empathetic response to alleviate financial burdens \cite{gambetta2015complaints}.
There is also a potential skew regarding who may choose to write a complaint \cite{joudaki2015using}; people with more negative experiences may be more motivated to do so, while some with extremely negative experiences may fear repercussions or societal stigma that prevent them from doing so \cite{freed_digital_2017, sharp2015review}.
Our primary goal nevertheless was to understand \edit{what specific financial attacks and barriers complainants report experiencing within our dataset.}

% \textit{why} complainants write about specific financial attacks and barriers they report experiencing.

Our dataset is modest compared to some fraud datasets \cite{ftc_data_2013, ftc_explore_2019}, so our results should be interpreted cautiously.
Namely, our keyword proximity assumption may not always apply to actual cases of IPFA or technology-enabled financial abuse, and keyword searches can limit the discovery of new IPFA patterns for survivors who do not use such terms.
The subsequent use of our workflow intends to mitigate this issue, but still relies on the results of keyword-based approaches as a reference set.
Further study is needed to explore different forms of harm and language used in self-reported IPFA.
Our study, while not representative of all survivors, nevertheless, offers a substantial cross-section of survivor accounts to U.S.-based financial institutions, providing valuable insights for institutions dealing with financial abuse concerns, particularly via digital devices.
% As financial services are expected to play a growing role in responding to concerns of financial abuse, it is essential to bolster efforts that help financial institutions be better equipped with anticipating a wide range of different concerns.

\paragraph{The Difficulties of Gathering Evidence of IPFA and its Effects on Resolution.}
\edit{Our work shows that the evidence gathering and resolution process for cases of possible IPFA are blockaded by a \textbf{lack of clarity around what is sufficient evidence} and \textbf{complex procedures for resolving issues}, some of which put the target at further risk. 
The evidence gathering process can be inherently difficult due to the nature of financial attacks, but may be required by financial institutions or legal policies to take any step towards resolving actions.} 
Further, concrete evidence that validates the experience of abuse is vital to combating the psychological harm associated with deception and negligence \cite{postmus_building_2023, sharp2015review}. 
We are nevertheless hesitant to claim that an improvement in evidence collection practices could immediately lead to improved outcomes for survivors, as many have already highlighted that the process of collecting evidence can be exhausting if not traumatizing \cite{freed_digital_2017}.
Indeed, our narratives show that even gaining access to evidence often appeared to be an impossible feat, given that many organizations lost documentation, failed to respond to requests for information, or did not permit complainants to know particular pieces of information about accounts opened with their information (e.g, social security number). 
\edit{Further, we show that the evidence gathering process itself can be an endless cycle of working with different stakeholder, making resolution a seemingly impossible goal, and sometimes what constitutes as sufficient evidence is not clear to the complainant. 
The complexities of the subsequent resolution procedures also come to light, often placing complainants at increased risk of abuse by requiring signatures or approval from former (and often uncooperative) intimate partners. 
The HCI research community is well-versed in designing accessible means of representing complex processes and information for different audiences. \anote{need an example}. 
Given this expertise, we suggest that the improved representation of resolution processes of financial burden stemming from IPFA for survivors is an apt and profoundly impactful area of further study, such as through the study of mapping and financial timelines to help customers better contextualize their financial history, and identify specific areas or products that are consistently targeted by abusers at key stages (\figref{fig:attack-product-matrices}).}

\paragraph{Technology-Enabled IPFA, Fraud, and Intimate Partner Technology Abuse}
\edit{In our work, we demonstrate the short- and long- term harms of technology enabled IPFA, which shares similarities with intimate partner technology abuse. 
Similar to survivors of tech abuse, complainants report experiencing a multitude of different types of technology-enabled financial attacks; with features that may overlap and vary in intensity.} %often overlapping and intensifying features.
While financial harms such as fraud and scams are often approached on an incident-basis --- a single event that can be delineated into before and after --- we suggest viewing IPFA as an on-going, persistent threat more akin to online harassment or hate. \edit{Moreover, we observe how the effects of IPFA can cascade and amplify over time, burdening complainants with increasing amounts of debt, duress, and personal harm. 
We observe that this stems from immediate and future monetary loss, efforts to shield children or other interpersonal family members from financial burdens, and the difficulties in evidence gathering and financial resolution. 
These effects bear a resemblance to the continued harm survivors of technology abuse face from the likes of harassment on social media and the release of private information to unauthorized parties \cite{freed2018stalker}. 
With technology-enabled IPFA, we see the emergence of a new aspect of technology-enabled harm as a byproduct of financial and monetary loss having a passive compounding effect on targets, making it similarly difficult for complainants to find resolution in financial infrastructure today. 
High amounts of debt or other financial burden, when unresolved, can have severe impacts on consumers in the long term in regards to mental, physical, and financial health \cite{sweet2013high}; for instance, future financial opportunities (as a result of continually stacking fees and impacts on credit) can be limited or closed off entirely as a result of being unable to resolve financial issues presented. 
We suggest that this increases the \textbf{urgency} of addressing burdens placed on targets of IPFA, and emphasize the \textbf{time-sensitive} nature of addressing IPFA once uncovered.} 

\edit{One approach to addressing the time-sensitive nature of intervention relies on the existing infrastructure and work on technology-enabled intimate partner abuse.}Finding instances of technology-enabled abuse can be challenging, prompting the creation of bespoke interventions such as security clinics and digital forensic diagnostic tooling \cite{havron_clinical_2019, freed_is_2019} \edit{and, we suggest that technology-enabled financial abuse \textit{necessitates} the augmentation of these forms of support with a particular focus on the compounding effects of financial debt and other burden, through the design and development of new or improved clinical tools.}

Our work also identifies a lack of clarity around when complainants discover technology enabled financial abuse in IPFA. 
One possible cause of this could be a lack of explicit direction to address such aspects of IPFA when submitting a complaint. 
\edit{We observe that the types of technology-enabled financial attacks experienced by a target can evolve with changing circumstances, such as in the case of legal proceedings or added financial impact on a target's children. 
Guiding complainants to provide details such as point of discovery may be a valuable area of future study, with implications in identifying the \textit{appropriate} means of support for a complainant, based on their circumstances.} 
Particularly, the results of our analysis, and our corpus, may prove of use to the CFPB, allowing for further study into different ways of intaking information surrounding technology enabled financial abuse that may address information gaps such as discovery.  

\edit{Finally, we see an urgent need for the development of trainings that help financial CSAs provide \textit{effective} and \textit{informed} support to targets of IPFA.}
Existing computer security support infrastructure has been shown to fall short in cases of addressing the unique threat model of intimate partner technology abuse, resulting in the development of carefully designed security clinics \cite{tseng2022care, havron_clinical_2019}. 
\edit{Our work suggests that a parallel gap may exist between financial support provided by customer service agents at financial institutions and the needs and considerations that need to be taken into account when addressing the impacts of financial abuse.}
Further, our work highlights that attacks may vary over time, causing survivors to continuously reach out to different financial institutions about their technology concerns\edit{, as well as to other organizations such as the CFPB.}
Although financial institutions are substantially different from service providers of online and digital services \cite{zou_role_2021, Bellini2023paying}, there is a potential to draw broader lessons from their approach to protecting vulnerable users over a longer period of time. 

% Financial institutions and researchers alike should consider these gaps when designing financial support infrastructure moving forward, working closely with the considerations of financial policy, safety planning, and the risks of retraumatization from evidence gathering to inform the pathways to resolution presented to customers facing harm as a result of IPFA.} 

\paragraph{Working Towards Clarity in Account/Asset Ownership and Financial Policies}
\edit{Our findings show that a common point of weakness against financial attacks in digital financial systems may be rooted in a \textbf{lack of clarity around account/asset ownership and authorization}. 
For instance, the novel form of attack uncovered by our work in the unauthorized use of a complainant's accounts to carry out criminal activity, results in the complainant being held responsible for the repercussions of this activity despite not authorizing this misuse of their accounts and assets. 
Similarly, in cases of financial negligence and deception a complainant is held responsible for a joint account they were previously unaware of. 
This lack of clarity propagates throughout the entire resolution process for many of these scenarios, resulting in difficulties gathering evidence to absolve a complainant 
from the financial harm due to account misuse or unexpected responsibilities in debt. 
Moreover, even when such concerns are raised, financial institution policies around the handling of joint accounts and authorization 
prevent meaningful resolution from being enacted. 
As observed in instances of technology abuse,} interpersonal relationships can naturally complicate traditional approaches to resolving disputes with digital technologies \cite{levy_privacy_2020}, even in areas that exist outside of abuse.
Namely, couples may have to pool their financial resources to pay for specific assets or experiences (e.g., houses, vacations) which often require shared account access and permissions \cite{park_can_2020} --- with financial services actively encouraging users to do so \cite{HowcanIs54:online}.
Unofficial proxies \cite{latulipe_unofficial_2022} (adults who assist older adults), carers \cite{mentis_upside_2019}, and intimate partners \cite{mcdonald_realizing_2020, Bellini2023paying} also often know the authentication information of those they assist. 
\edit{In fact, several descriptions of abusive behavior that were found in our corpus, such as the unauthorized opening of accounts, intentional misuse of digital financial resources, and the direct theft of financial capital, have been observed across the context of \textit{other} interpersonal relationships, such as in cases of caretakers and an elder vulnerable individual \cite{black2008not, noauthor_metlife_nodate} as a direct result of this shared access and permission changes. 
This warrants cause for a few reconsiderations moving forward. }

\edit{Foremost, future digital fraud and criminal activity detection and evidencing policies should be designed with the consideration of account misuse and how shared accounts can obfuscate the true perpetrator. 
Second, further transparency and clarity around account ownership should be designed and integrated into existing user financial flows. 
One possible avenue of doing so is with frequent safety 'check-ins' on a user's financial account. 
Frequent safety check-ins have shown to be effective in helping individuals manage devices, and perhaps something of a similar nature can be explored for existing financial systems \cite{}. 
Similarly, as of recent, safety checks have been integrated into popular mobile and desktop systems with an intention to provide survivors a means of performing their own audit of their devices for signs of technology abuse.
HCI researchers and developers alike may choose to explore and study similar approaches to auditing an individual's \textit{financial} accounts to look for signs of unexpected behavior or attribution. 
Overall, our analysis demonstrates the need for mechanisms that make information about accounts involving the personal information of survivors of financial abuse (e.g., accounts opened in their name) more easily accessible \cite{havron_clinical_2019}.} 

\paragraph{The role of Automation in Identifying, Analyzing, and Addressing IPFA}
We note that despite our best efforts to be considerate and transparent in our identification approach (\secref{fig:model_pipeline}), there is the potential
%are undeniably ethical tensions in how this approach may unfairly 
to stigmatize or label individuals with language that may only partially describe their experience.
%not used by themselves. 
It is well-established that language models, are reflections of the data on which they are trained, thus mirroring any embedded biases \cite{abid2021persistent, vig2020investigating}.
We note that only a small minority of complainants self-identified their experiences with the self-identification of abuse (\secref{sec:analysis-intro}), or being a survivor of violence, necessitating a careful synthesis of machine learning approaches and human review.
%Our work aimed to shed light on a societal harm that leaves devastating harm in its wake, yet the loss of potential confidentiality or control a survivor may have over their financial products, such as through surveillance, forecasting, and regulation cannot be ignored.
Such bias may be driving the reliance of our identification approach on distinguishing cases in which the complainant spoke of their intimate partner as the \textit{cause} of financial harm from those in which intimate partner is a \textit{shared} survivor of financial harm.
%In the case of our particular approach, our approach to distinguishing between cases in which a complainant spoke about their intimate partner as a \textit{shared} survivor of financial harm versus cases in which the complainant spoke of their intimate partner as the \textit{cause} of a financial harm, appeared to be key to detecting IPFA complaints.
Indeed, our approach method may yield fewer cases of IPFA in which the complainant is not completely aware that their intimate partner has caused the financial harm.
Thus, our model may be sensitive to forms of accusatory language that may not always match how survivors express financial abuse.
%make sense of their experiences with financial products.
Additional experimentation is needed to determine if pre-trained sentence transformer models can be used to identify cases of \textit{potential} IPFA that do not include accusatory language and to explore how comprehensively language modeling can be used to detect IPFA when complainants implicate intimate partners. 
\edit{Altogether, our method produces a corpus of complaints that represent a \textit{subsample} of possible IPFA, and more study is required to understand the larger space of self-reported IPFA within complaints. 
Despite the specific nature of our corpus, we observe that it begins to reveal \textit{some} attributes that can be used by both researchers and developers in improving services for targets of IPFA.}

We see fruitful future research that explores this challenge further, such as with supervised approaches. 
Given the relatively small size of our corpus of representative complaints, one possible direction could be to use few-shot learning techniques that rely on fine-tuned sentence transformer models for classifying IPFA \cite{tunstall2022efficient, gao2021simcse} with our corpus as training data. 
Such a model could then replace \textbf{\circled{3}} and \textbf{\circled{4}} in our workflow, and enable iterative model improvement as new complaints involving IPFA are discovered.
Recent study has also shown significant performance increases in language modeling tasks with techniques involving large language models (LLMs), step-by-step reasoning, and rationales \cite{hsieh2023distilling, zhang2023multimodal, huang2022large} in few-shot learning contexts; these techniques, when used with expert reviewers, may prove fruitful in creating an improved supervised model from our corpus. \edit{Automated methods, if sufficiently accurate, can also \textit{augment} existing human-centered support and referral systems for targets, particularly in the scaled triage of possible IPFA; being able to identify such cases at scales may prove fruitful for support organizations in the direct referrals of targets to appropriate resources (i.e. financial, legal, and technology services).}

\paragraph{The Importance of Characterizing the IPFA Complainant}
\edit{Our work exemplifies the importance \textbf{characterization} plays in addressing the harms both from technology enabled IPFA and other forms of technology-augmented abuse. 
Thus far, we've discussed several elements of our findings that call for awareness, re-considerations, and improvements in how we continue to approach digital finance and the technologies used to interact with financial systems with a lens that acknowledges the unique forms of harm from financial abuse. 
These areas of discussion are tightly connected to the characterization of IPFA complainants within our dataset itself, and we suggest that there is much room for further study in this characterization, that can contribute to the progression of research and development in this area.} 
In this study, we have augmented the understanding of abusers and complainants in IPFA cases through careful human review involving experts in IPV, financial abuse, and perpetrator behavior. 
Our corpus shows that complainants often do not characterize their experiences as abuse, despite describing behaviors and experiences that meet technology abuse definitions. 
In addition, while the relationship between intimate partners is often described as having ended (e.g., an ex-spouse) complainants are often still entangled in relationships from a legal standpoint (e.g., divorce may be in progress or yet to be initiated) \cite{freed_digital_2017}. 
% These insights suggest that when studying or addressing IPFA, a broad range of complainant language should be anticipated and a focus on the attributes of the complainant experience may prove to be key in identifying supportive services.
\edit{The lack of explicit characterization highlights the importance of scrutinizing attributes of complainant experiences when studying or addressing IPFA in the future. 
A broad range of complaint language should be anticipated within complaints, but the attributes uncovered should be further tested with alternative data sources; for instance, by studying specifically how the kinds of financial abuse carried out evolve over time. 
Further analysis along these attributes may prove to be key in identifying appropriate support services and improving processes for the future.}

==> sections/06_conclusion.tex <==
% \section{Conclusion}
% \knote{This conclusion doesn't add anything insightful... suggest striking and ending the paper here.}
% This paper begins to answer three crucial questions surrounding IPFA for the development of methods to secure digital finance for survivors of this form of harm. First, we leverage prior literature and manual coding to develop robust definitions of IPFA, and how it differs from other forms of financial harm. Using these definitions, we begin building a corpus of IPFA complaints for use in future study. Next, we examine how existing language modelling techniques can isolate IPFA, providing basic insights for future work in language-based detection, as well as leveraging the results to build our data set further. Finally, we topic model our final dataset of 527 complaints to identify self reported traits of IPFA as represented in complaints, finding key insights that can be leveraged for improving the security of digital finance against these harms. To conclude, we reiterate the value of these contributions towards significant future work surrounding IPFA, and suggest potential verticals of study moving forward. 

==> sections/07_acknowledgements.tex <==
\section{Acknowledgements}
\begin{acks}
\noindent We thank Fannie Liu and Francesca Mosca for their feedback on this work. We are also grateful to our associate chairs and reviewers, whose comments helped to improve the manuscript. 

Rosanna Bellini's contributions are supported in part by NSF Award CNS-1916096 and a research award from JPMorgan Chase.

% This paper was prepared for informational purposes by the Artificial Intelligence Research group of JPMorgan Chase \& Co. and its affiliates (``JP Morgan''), and is not a product of the Research Department of JP Morgan. JP Morgan makes no representation and warranty whatsoever and disclaims all liability, for the completeness, accuracy or reliability of the information contained herein. This document is not intended as investment research or investment advice, or a recommendation, offer or solicitation for the purchase or sale of any security, financial instrument, financial product or service, or to be used in any way for evaluating the merits of participating in any transaction, and shall not constitute a solicitation under any jurisdiction or to any person, if such solicitation under such jurisdiction or to such person would be unlawful.

This paper was prepared for informational purposes in part by the CDAO group of JPMorgan Chase \& Co. and its affiliates (``J.P. Morgan'') and is not a product of the Research Department of J.P. Morgan. J.P. Morgan makes no representation and warranty whatsoever and disclaims all liability, for the completeness, accuracy or reliability of the information contained herein.  This document is not intended as investment research or investment advice, or a recommendation, offer or solicitation for the purchase or sale of any security, financial instrument, financial product or service, or to be used in any way for evaluating the merits of participating in any transaction, and shall not constitute a solicitation under any jurisdiction or to any person, if such solicitation under such jurisdiction or to such person would be unlawful.  
\end{acks}

==> sections/analysis-reorg/04c_analysis_attacks.tex <==
\subsubsection{What financial attacks do survivors report in CFPB complaints?}

\begin{table}[!htb]
    \centering
    \input{figures/tables/attacks-table-2}
    \caption{A summary of the new financial attacks in the IPFA corpus ($n=513$) grouped by category. \ronote{We'll need to highlight which ones have been seen before}}
    \label{tab:attacks}
\end{table}

\edit{Our analysis was able to uncover 30 novel financial attacks as reported by complainants in their CCNs.
For clarity, we categorize these attacks into five categories (\Cref{tab:attacks}), some 
In \Cref{tab:attacks}, we categorize these attacks in to \catNum overarching types; \ronote{to fill in when ready....}. 
We discover that our analyses validate and extend known financial and technical attacks as reported by Bellini et al. \cite{Bellini2023paying} and Freed et al. \cite{freed2018stalker}, such as account and device compromise, exposure of private information, deception, and, harassment.
Our efforts were able to uncover an entirely new attack; \textit{financial negligence}; the refusal to, reneging or failing to fulfil an established financial agreement, and significantly extend Bellini et al. \cite{Bellini2023paying}'s \textit{financial deception} category}.
We now visit each in turn.

% While we were able to identify most of the prior attacks in the CCNs we analyzed, there were several not seen in our analysis, such as the IP posting financial or non-financial harmful content, duping an agency to re-direct salary, and falsifying evidence of online accounts. While these may have surfaced had we reviewed more CCNs, we hypothesize that these attacks may not be present due to the different focus of each dataset (i.e., financial abuse v.s. tech abuse).

\edit{We identified 30 novel financial attacks in our analysis of complaints. In \Cref{tab:attacks}, we categorize these attacks in to five overarching types. We describe the nuances of each of these types below.}

\paragraph{Financial Negligence}
Financial Negligence involves attacks where a financial agreement/obligation between the target and their IP is the centerpoint of abuse, resulting in harm on the target. Examples of such agreements can be both legal in nature (such as directed child support or division of debts during a legal separation), or informal (such as an IP being responsible for a portion of rent). Abuse by financial negligence then, can include attacks ranging from the refusal to cooperate in creating or managing the terms of an agreement in the first place to reverting on a prior established agreement. 
We see a particularly indicative example of an IP refusing to cooperate in complaint 2417487, where the IP refuses to provide their signature in helping manage and paying off a loan after separation:
\begin{quote}
    \textit{"...My Ex-husband & I consolidated school loans prior to divorce in 2004. Since that time, I have tried numerous ways to take care of this account. Due to the fact, I was court ordered to be responsible for repayment of entire amount exceeding 25[redacted]. They will rarely speak with me and I can not submit any documents with out my ex-husband of 14yrs signature. This is just NOT POSSIBLE. He is bitter and will not cooperate..."}
\end{quote}

Interestingly, we also observe cases where an IP actively or passively avoid fulfilling a financial agreement. We see an example of this in complaint 3838460, where the IP is described as not paying child support and adhering to unpaid debts assigned to them during divorce: 
\begin{quote}
    \textit{"...My ex-husband didn't adhere to the stipulations of the divorce pertaining to unpaid debts, nor did he pay child support as he is over {\$90000.00} past due... "}
\end{quote} 
In total, we observe XXXX complaints where the target is impacted by IPFA in the form of some sort of financial negligence. \\

\paragraph{Financial Deception}
We also see complaints where financial abuse roots from some form of deceptive behavior from the IP, which we categorize as Financial Deception. Financial deception can involve a wide range of behaviors from deceiving a target into believing they have been removed from a credit/debt that they are not responsible for, to tricking the target into co-signing on debts by claiming co-signing as a requirement. We see an example of the latter in complaint 3134442, where the IP convinces the target to sign onto a loan, resulting in unanticipated debt later on when the loan goes into arrears.
\begin{quote}
    \textit{"...In 2013 my husband applied for a HELOC loan. According to my husband, it would be necessary for me to sign the papers for said loan. I was unsure why, as I am not on the mortgage and I am a homemaker with no monetary income.But, as I was told by the bank and my husband that it was just a " Florida Thing '' and strictly a formality. However, I am on the deed. The entire amount of the loan was deposited in to my husband 's account. I had no access to the HELOC account at all. I am divorcing my husband of 35 years. I have since discovered that the house, mortgage and HELOC are all in arrears, I am once again stuck with the burden of responsibility when I was not ever given any choice in this matter..."}
\end{quote}
Similarly, we see another form of deception in complaint 4731741, where an IP submits an insurance claim under the target's insurance, resulting in financial harm.
\begin{quote}
    \textit{"... I didnt have these insurance policy on the date of [MM/DD/YYYY] with [redacted] for the amount of {\$3100.00} or [redacted] for two other accounts for {\$130.00} dated : [MM/DD/YYYY] and for {\$330.00} dated : [MM/DD/YYYY]... I tried to explain to the insurance agent maybe another family member Divorced husband ) May have opened this claim at [redacted]  & [redacted]  because Ive been divorced for 6 years and it definitely was not myself..."}
\end{quote}

Financial deception can have some overlap with financial negligence, in that deception or lying may play a part \textit{alongside} reverting or refusing to fulfill a previously established financial agreement or obligation. 

We observe a total of XXXXX complaints that fall under this subtype from our corpus.\\

\paragraph{Duress} 
We categorize cases where a target describes being coerced or pressured by an IP into a financial action against their will as cases where the attack is carried out by causing Duress. Duress appears in several forms within our corpus, such as through threats of legal action or divorce as seen in complaint 4536981, where the IP forces the target to sign onto a reverse mortgage:
\begin{quote}
    \textit{"...In the year [redacted], my husband and his colleague forced me into a reverse mortgage against my will. This loan was orchestrated under severe duress for fear of divorce. Both my husband and the loan officer knew of my objections and the fact that I did not want to sign the loan documents. I had repeatedly expressed my fear and duress about this type of loan..."}
\end{quote}

We also see duress occur under fear of an IP, such as in complaint 1336631. 
\begin{quote}
    \textit{"... have a judgement against me by [redacted] [redacted]. They are located in [redacted], MN. The judgement is from [redacted] against debt I owed to Chase Manhattan Bank.  My story : I was married to a very [redacted] man. [redacted]. My ex-husband had me apply for several credit cards that he used at his discretion. I complied out of fear..."}
\end{quote}

In many cases where Duress is identified, it is \textit{also} accompanied by another attack or type of IPFA (n = 11/12 total complaints identified), showing a possible chain of attack that can have escalating impacts on a target and may be useful for any future work exploring how FSPs can detect IPFA. 


\paragraph{Blocking a target's Financial Actions, Assets, and Access}
In our corpus, we observe several attacks that result in a target's financial assets, access to these financial assets, or performing actions on these financial assets being blocked. One way this culminates is in account freezes as a result of an IP taking out fraudulent checks from the target's account, as seen in complaint 4883504:
\begin{quote}
    \textit{"...I went thru a traumatic divorce, so my ex-wife did fraudulent checks on my account and the bank put a freeze on my accounts..." }
\end{quote}
We also see account lockout as a result of an IP disputing transactions between them and the target such as in complaint 4252133:
\begin{quote}
    \textit{"I was sent three legitimate [redacted] transfers for rent/bills to my Wells Fargo checking account ... by my ex-boyfriend. On [MM/DD/YYYY] I found myself locked out of my Wells Fargo App and the Wells Fargo Website... Upon contacting them, customer service vaguely transferred me to their Fraud department where I was asked if I could account for the reason for the three transfers. I stated they were probably from my ex-boyfriend, as I could not access my accounts at that time to look at the said transfers she rattled off since I was still locked out of account access, to pay bills such as rent... She then proceeded to tell me that my extra-boyfriend has claimed that these legitimate [redacted] transfers made two and three months prior were reported as fraudulent by my ex boyfriend to his bank, [redacted]..."}
\end{quote}
In this case, the target is further impacted by being unable to pay rent, showing again how certain attacks can cause escalating harms on the target. 
\\

\paragraph{Unauthorized Access, Usage, and Opening of Financial Assets}
The final type of attack we observe involves an IP broadly carrying out unauthorized behaviours with a target's financial assets. One way this culminates is in attacks involving an IP trying to get information about a target's financial assets from Financial Service Providers, either through impersonation or persuasion. An example of this is seen in complaint 4096714, where the IP is able to impersonate the target to an automated phone banking system using the target's information:
\begin{quote}
    \textit{"...My ex husband used the automated IVR phone system for Comenity Bank to obtain my current credit card balance and last payment information to use against me. He knew my phone number, address and last 4 of SSN to use the automated system to obtain information he is not authorized to access. There is no way via the automated system to block him using any additional security measure, like a PIN, to deny access to this private information. If he calls into a live rep, I have added a password to deny access..."}
\end{quote}
We also observe an attack where the IP uses the target's credit cards to carry out fraudulent activity on \textit{others}, leaving the target on the hook for any repercussions for the fraud when it is discovered (Complaint 2349007):
\begin{quote}
    \textit{"It came to my attention recently that an ex-girlfriend had fraudulently used my [redacted] credit cards. One had a limit of $ [redacted] and the other $ [redacted]. I notified [redacted] and filed a police report. The fraud included a gentleman facilitating phone calls and posing as me. Both parties have been charged...About three days later, [redacted] called and said that since i had been a beneficiary of the fraud, even though it was unknowingly, they could not substantiate it as fraud. I agreed to handle the process through the courts to seek the return of property acquired and restitution..."}
\end{quote}
Physical surveillance to identify a target's personal information is also reported. For instance, in complaint 4030524
\begin{quote}
    \textit{"...While I was with my ill daughter her husband had cameras set up snd I know thats how he got pin. When you log into their system it asks for a pin. My daughters soon to be x hasnt. Even able to be evicted cause of COVID. This man also stole my clothes snd all my belongings I arrived with. He stole his uncle clean car many times along with his valuables. The police were notified..."}
\end{quote}

This highlights what has been observed in cases of technology abuse in the past, where an intimate partner may leverage methods of surveillance to gain information and control a survivor \cite{add-citation}.
\\

\Cref{tab:attacks}

==> sections/analysis-reorg/04c_analysis_barriers.tex <==
\subsection{What barriers do complainants report experiencing at financial organizations?}
\noindent \edit{For this analysis, we consider barriers that were positioned by complainants as an obstacle that prevented them from moving forward, or accessing a valuable resource.
A poignant reason for contacting the CFPB was that they had received an unsatisfactory resolution from their FSP, CB, or CP (n=83) --- a situation that CFPB's \textit{Customer Complaints Initiative} was explicitly designed for \cite{consumer_financial_protection_bureau_cfpb_2023}.
% As the \textit{CFPB Customer Complaints} program exists to respond to consumers who are dissatisfied with the response from organizations under their remit, this is somewhat unsurprising.
We consider what \textit{types} of resolutions (or lack of) may trigger a complainant to reach out; of which we identified credit cards, debt, and mortgages to be the most prevalent for a survivor to receive an outcome that necessitated escalation of this complaint (mostly mirroring other general customer trends \cite{consumer_financial_protection_bureau_cfpb_2023}).
As addressing barriers to socio-technical systems for recourse from abuse has significant implications, we identify four sub-types that constitute barriers to addressing technology-enabled financial abuse; escalating digital-safety risks; documentation and evidencing; and policy design to accommodate financial abuse in intimate partnerships.}

\paragraph{Elevating digital-safety risks.}
\edit{Many financial products we identified in our analysis were often co-shared or connected to a person inflicting harm on a complainant, including bank accounts, house loans, car insurance, and utility bills.
Relationships with abusive partners can present unique digital-safety risks, such as fraudulent purchases, identity theft, or social engineering to elicit financial information through social engineering \cite{wood_financial_2017, freed_digital_2017, freed2018stalker}.
Our analysis revealed that customer service agents (CSA) are broadly unaware of such a risk, and made multiple recommendations for a complainant to directly \textit{challenge} an IP until the concern was resolved.
In spite of explaining concerns about being unable to resolve the issue on their own, CSAs and branch staff would recommend complainants \textit{``take the issue up''} with an IP (3601686).
As one complainant described after reporting a card opened in their name:}

\begin{quote}
    \textit{``I called today to find out the status, and was told [by the CSA] that I benefited from this. I don't understand how I benefited from being the victim of domestic abuse. They said I had to file a police report, but, if I did that, my husband could possibly hurt me physically ... ''} (Complaint 2913103)
\end{quote}

\edit{In general, complainants reported being afraid of physical retaliation after approaching the person of concern, citing \textit{``feeling fearful and scared''} of the person that they had been admonished for \textit{``trusting them [IP]''} by a financial representative (3626113).
While CSAs should not be expected to provide direct IPV support to complainants who describe this, such results point to the need for CSAs to have training on how to handle such complaints without discrediting or putting a complainant at further risk (c.f., \cite{zou_role_2021}.}

\edit{Many complainants also described significant financial stressors and burdens as a result of the lack of resolution regarding their financial assets which put them at-risk of other harms.
For instance, some complainants described being a single mother, facing the threat of homelessness, or unemployment alongside or directly caused by the financial abuse experience, with one complainant sharing: \textit{``I am barely surviving on the income I have''} (3193403).
Namely, complainants were often encouraged by representatives at financial organizations to find another source of income, forgo claims for theft of financial assets, hire an attorney to pursue legal action (\ref{sec:results-}), to \textit{``find another bank''} (1369215), or even to pay off the outstanding debt. 
In response of being recommended to modify a loan took out through coercion (`coerced debt') by a FSP representative, one complainant exclaimed: \textit{``I am not looking to modify this loan, I am looking to be free of this loan!''} (2664406).}

\paragraph{Lack of documentation and proving abuse.}
\edit{Despite multiple adversities, some complainants attempted to take on the complexities of their specific financial case independently, but were met with a \textit{lack of a response} from the financial organization (n=34).
We identified that the threshold for being able to demonstrate proof of financial abuse was considerably high, namely, that when complainants attempted to contest authorized opening of credit cards in their name, a financial organization would turn around and ask for `proof' as so:}

\begin{quote}
    {\textit{... My ex-wife has continued to obtain new credit in my name. I have disputed many accounts that appear on all 3 credit bureaus only to have them respond with ''we need proof''. ... nothing changes or helps ... I'm really just stuck ... This is insane.}}
\end{quote}

\edit{In addition to the quality of the evidence, screenshots and transcripts often weren't taken into account as they were judged to not meet the threshold expected to dispute such harms.
Such actions were also prevalent in complainants whom provided detailed descriptions of trauma in collecting their own evidence as a consequence of the high entry barrier (n=11).
Evidence gathering was distressing for many survivors who had already reported that they had been affected by such an approach during legal proceedings, such as divorce or restraining orders.
However, this reportedly trapped them in what a survivor described as a `vicious cycle' --- that to get proof they needed to ask the financial organization to send over the documentation, whom would then refuse to do so without first seeing `proof' of abuse.}

\edit{While some financial organizations aimed to assist complainants with the challenge in documenting their experiences, this also incurred barriers, such as a complainant failing to receive documentation, having to share intimate details about themselves (e.g., salary, location history), or being unequipped to receive documentation that a FSP could share.
In one scenario, an complainant received the requested statements from an IP opening an account via an email from an FSP, but was \textit{``unable to open the zipped attachment to see the contents''} (2905125).}

% I have asked for proof of this debt a number of times from Portfolio Recovery and have never received any documentation in the mail.

% I have no supporting documentation that this account was open fraudulently as I have no contact with my

% Please see the attached screenshot I took

% (2905125) I told her I needed the statements from the time my wife opened the account up to today. She immediately obliged and sent an email with an attachment containing the statements and a fraud kit, I think she said. The trouble was, I was unable to open the zipped attachment to see the contents.

% (2572979) requested a copy of the complete records and application for the account. On [MM/DD/YYYY], Barclay mailed a copy of the credit application. The report provided by Barclay was a one page printout that only had basic information about me on it, including my name, DOB, income, mortgage expense, and address. There was no signature or anything else in that " application '' that could have been used as verification that I was the one opening the account. My attorney sent follow up correspondence to Barclay regarding our fraud claim on [MM/DD/YYYY], [MM/DD/YYYY], [MM/DD/YYYY], [MM/DD/YYYY], and [MM/DD/YYYY]. Barclay has never responded to any of these letters, provided any response to our fraud claim, and continues to send monthly statements on this account


% So while I'm waiting, the late fee and interest was intact, and I was billed still. This has taken a severe toll on my emotional and financial health. What about PNC 's best practices? Do you even practice ethical, sound business practices? I was violated. Am I to understand that PNC prides themselves on protecting customers? If so, how was I victimized? I'm not even a customer. I didn't open the card, and I am not the card holder. So why is my name on the card, and why is this seriously affecting my credit score? 

\paragraph{Policy design to address financial abuse.}
\edit{Mirroring work in other areas of digital finances, we identified that many complainants were poorly served by company policy in managing financial abuse cases.
While policy is a common area of contention in other settings outside of IPV, we identify two commonly occurring challenges; authorized transactions, and, consent-based concerns.}
\edit{Identifying the difference between \textit{authorized} and \textit{unauthorized} transactions was a common problem for many complainants; where receiving a judgement of unauthorized would trigger a fraud investigation, while authorized could result in a lack of action.
While P2PP services were a rare occurrence in our dataset (as many companies do not as of yet earn over \$10B in assets), we identified several complainants who cited that previous interactions with an IP banned frauduluent transactions from being considered fraduluent.
While fraud and theft are common in other areas other than our specific focus, we noted a notable lack of consistency in how a complainants experience was categorized in our dataset.
For instance, one complainant shared the following after having a phone stolen:}

\begin{quote}
    \textit{``... there was a fraudulent transaction from my account issued to ``[fake-name]'' in the amount of {\$6000.00}. This ``[fake name]'' was an ex-boyfriend who had stolen my phone and sent the money to himself after turning off my notifications to my number. I immediately contacted [P2PP] and inform them of the fraudulent transaction ... I was able to get nothing resolved until far after the time to which they informed me that it was a non fraudulent transaction because said `` [fake name] '' and I had previous transactions''} (4996862)
\end{quote}

\edit{In this situation, the fact that a complainant had previously interacted with an IP in this context --- despite a clear description of device compromise --- was enough to categorize this transaction as non-fraudulent; resulting in a substantive loss of money for a complainant.
In some cases, while complainants stated that employees of financial organizations were more sympathetic to their concerns, yet most reported an inability for policy to permit them to do so:}
% \begin{quote}
%     \textit{``I completed the necessary paperwork and provided the proof required ... the bank manager explained to me that they had thousands of accounts and there was no way they could keep up with everyone's personal problems and who had what in their account''} (1336631)
% \end{quote}

\begin{quote}
    \textit{``My husband has 100\% control of all of our money ... I attempted repeatedly to get into my account to get funds to hire an attorney ... I was then told I never had an account there ... I pleaded with the teller who quietly told me she believes me but she would lose her job if she tried to help me''} (4492998)
\end{quote}

% (1840984) I have bad credit and no home, so how can I now mover forward to rebuild because I will now have a foreclosure on my credit report. Please help!

% Low SES, struggling to get through. 

% \edit{The overwhelming majority of complainants cited that either the FSP or CB they had first approached with a claim or complaint produced no or an unsatisfactory resolution (n=83).
% Such a finding is to be expected when the 
% Nevertheless, identifying what \textit{types} of resolutions may trigger a survivor to form a complaint to the CFPB was worth investigating.

% \paragraph{Obscuration of intimate threats.}
% \edit{We found most complaints reported surprise at how financial institutions were not designed for the consideration of an intimate threat; namely, a partner who had access to private and confidential information but could perform malicious actions.
% Even more concernedly, we several complaints where an IP was permitted to conduct their attacks without standard checks by leveraging their close proximity to a survivor.
% For instance:}

% \begin{quote}
%     \textit{``He had a credit line also on the checking account which I wasn't even aware of. When we married he put me on as a secondary signer [on the account]. My husband filed bankruptcy and [bank] decided to attack my credit which I find incredibly unacceptable.''}
% \end{quote}

% Confront the abuser

\subsection{What are the common characteristics of consumers who submit a complaint describing financial abuse?}
\edit{We found that in our dataset complainants did not withhold from sharing their experiences of other forms of abuse, namely emotional, physical and (occasionally) financial.
These disclosures were most commonly reported in past tense, such as historic accounts of abuse in the past (from a range of 6 --- 12 years ago) that were still having an considerable impact on the complainant.
These past disclosures of abuse were predominant with the complainant sharing that they wished to `move on' with their relationship, and the prior use of harmful behaviors was holding them back.
Nevertheless, while such complainants did identify other kinds of abuse as abuse, we identified that it was rare to extend this description to the reason that they were complaining was caused by financial abuse.}

\subsubsection{What are the common characteristics of financial abusers?}
\edit{Many scholars approach understanding perpetration through the creation of `illegitimate' complaints; such as a customer deliberately fabricating problems to gain free service options.
While Bellini et al. \cite{Bellini2023paying} provides advocacy perspectives on why financial abusers may be motivated to do so, but we go one step further to communicate important contextual factors that are otherwise unknown.}
We identified that most authors of a complaint described their offender as being an ex-partner (n = 281) at the point of complaint submission. 
We note however, that many individuals did not specify whether the partner was a former partner at the time of attack. The second most common relationship described is of a current partner (n = 163). 
Finally, we observe a small set of complaints that describe a deceased partner (n = 7), which we propose as a new target-perpetrator relationship in this piece. 
Although a perpetrator cannot actively perform IPFA when deceased, we note that this highlights how targets may discover the harms of an attack or report the harms of an attack after their partner passes away. 
From the seven complaints, we find that five describe the point of discovery of IPFA. 
In four out of five complaints, we note that the complainant describes finding out about attacks \textit{after} the IP passes away. 
Although the sample size is small, this provides new insight into how targets of IPFA might discover and reach out to FSPs about abuse from a now-deceased IP, and warrants further work identifying the prevalence and nuances of such cases. 

\edit{In our analysis, we identified three significant risk factors related to financial abuse. 
The first risk factor was the occurrence of financial abuse started when a survivor was in the hospital, or fell physically ill to necessitate seeking out healthcare.
The other location we identified as being poignant was when a survivor was incarcerated; thus leaving a shared domestic environment:}

\begin{quote}
    \textit{``On [MM/DD]/2019, I was arrested on a [redacted]. During my [redacted] my ex boyfriend withdrew {\$1100.00} from my bank account. I was released on [MM/DD]/2019. the  following day I went to my local PNC bank and explained the situation. I was told to file a dispute and my money would be refunded due to him taking my money while i was incarcerated. I provided the proper paperwork to show proof and the bank even printed out a report on how the money was withdrawn while I was [redacted].''}
\end{quote}
 
\edit{This finding suggests that individuals may become vulnerable to financial exploitation during periods of limited mobility or reduced control over their finances. 
The hospitalization or incarceration of a person may create opportunities for perpetrators to gain access to their financial resources while a survivor is otherwise distracted and manipulate them for their own benefit.}

\edit{Another notable risk factor we observed was when an intimate partner was employed in the digital and financial service industry.
This association raises concerns about the misuse of professional knowledge and access to financial systems by individuals in positions of power. 
Intimate partners who work in these industries may possess advanced knowledge and skills that enable them to exploit their partner's financial assets or manipulate financial transactions without detection.}


==> sections/analysis-reorg/04c_analysis_discovery.tex <==
\subsubsection{How do financial survivors discover and respond to financial abuse?}
We discover that while the majority of survivors do not report a point of discovery (n=236), we observed credit reports (n=33), and credit score checks (n=24) were prevalent sources of notice for complainants.
Complainants would mention that they did not realize that they had a financial issue until checking their credit, which falls in line with the common financial advice of checking one's credit score regularly for irregularities \cite{}.
Further, often a complainant was unaware of a debt until that debt had already gone to collections, at which point it had not only affected their credit, but now came with additional near-term consequences such as wage garnishment and harassment from collections agencies.
When contacted by a collections agency, complainants often reported that this was the first point of contact of the existence of (often) coerced debt: 



As incidents escalate after discovery, resolving IPFA financial issues becomes more complicated, but we suggest treating customers who have accrued coerced debt in such a manner that befits their needs.
For instance, Zou et al. \cite{zou_role_2021} and Bellini et al. \cite{Bellini2023paying} highlight the need for further training to ensure a survivor is not re-traumatized by an unncessarily callous response.

% We discover that the majority of survivors did not disclose a point of discovery (n=236).


% We found that the overwhelming majority (n=236) of narratives did not disclose a point of discovery. This could be due to fact that the intake form on the CFPB website does not ask complainants to recall when they first discovered the abuse. Another consideration can be made in the point of engagement when consumers make their complaints, leading to less specificity (e.g., after repeated complaints elsewhere).

% Beyond this, we observed that credit reports (n = 44), contact by a collections agency (n = 33), and credit score checks (n = 24) were the most prevalent sources for discovering IPFA from our corpus. Many complainants would mention that they did not realize that they had a financial issue until checking their credit, which falls in line with the common financial advice of checking one's credit score regularly for irregularities. Further, often a complainant was unaware of a debt until that debt had already gone to collections, at which point it had not only affected their credit, but now came with additional near-term consequences such as wage garnishment and harassment from collections agencies. Resolving financial issues from IPFA can be complex, and as matters escalate from the point of discovery, the steps towards resolution can vary as well. 

Most complaints in our corpus detailed filing a complaint with the affected FSP (n=243) as a method of resolution. 
Further, we observe that complainants in our corpus reach out to the relevant FSP to help resolve issues either \textit{prior} to reaching out to the CFPB, or \textit{in addition} to it. 
This highlights the importance of our work in uncovering the role FSPs play in addressing the financial harms of IPFA, since it is evident that complaints and contact \textit{is} made by a large proportion of complainants. 
Further, we confirm our hypothesis that complaints submitted to the CFPB can be further downstream in a target's resolution journey, marking direct-to-FSP complaints as a valuable source for study in future work that could yield (a) a higher magnitude of possible IPFA, and (b) even more granular information surrounding a target's experiences living with the harms of IPFA.

We also note an unfortunately high proportion of targets paying off debts associated with IPFA as a means of resolving harms (n = 44). This results in further harm from the original instances of IPFA, and perpetuates the long term harms of this form of abuse. 
Further, we observe that complainants most often pay off outstanding debts from IPFA \textit{alongside} performing some other form of resolution, such as paying off debts \textit{and} submitting a complaint to an FSP (n = 24), or paying off debts \textit{and} submitting a complaint to credit bureaus (n = 5). This could be a result of targets attempting to address the immediate, short-term repercussions of IPFA, and to prevent these short term repercussions from escalating later on while their financial issues are investigated by other stakeholders. Indeed, an example of such can be seen in the following sample from complaint 3356032, where the complainant reaches out to their respective FSP, but also pays off the debt as a result of potential credit impact, as advised by a collections agency: 
\begin{quote}
   \textit{... On [MM/DD/YYYY], [redacted] collections called me with indicating that if I didn't make a payment that day, there would be negative reporting on my credit because we were " at the 40-day mark. I went ahead and MADE A PAYMENT THAT SAME DAY, [MM/DD/YYYY]. Because I was told this payment would avoid negative reporting, I am here alleging erroneous late payment reporting by [redacted] ... } 
\end{quote}
Although we \textit{do} see a majority of complainants within our corpus reaching out to FSPs when attempting to resolve the harms from financial abuse, we clearly see cases where the target needs to take multiple resolution steps that involve multiple stakeholders and potential financial loss. This speaks to the need for further study in understanding how best to support targets in navigating the complexities of resolution, across FSPs and other stakeholders. 


==> sections/analysis-reorg/04c_analysis_intro.tex <==
\section{Analysis of IPFA Complaints}
\label{sec:findings}
\noindent \edit{On a trial run of automatic encoding of our dataset to highlight the disparity in financial abuse detection systems (c.f., \cite{}), only 13 CCNs were automatically coded as pertaining to abuse, with many requiring explicit identification and description by the complainant as `abuse'; a mere 2.8\% of our total dataset. 
Such results further emphasized the need for us to leverage a multi-agent human coder team.}

\edit{In analyzing our dataset of \setdupe complaints, we combined two qualitative approaches to determine how IPFA complaints differ from those containing information on intimate partners and financial hardship.
In the first round of analysis, we used a deductive approach through our machine learning tools that was based on Ritchie and Spencer's \textit{Framework Analysis} (FM) \cite{becker_epistemological_2007}.
We identified this could help to test preconceived hypotheses (as stated in \secref{sec:intro}), and organize our data to undergo systematic comparison.
To complement the common pitfalls of FM \cite{gale_using_2013}, we complemented our findings with a discourse analysis through a manual, hand-coded approach to further probe survivor's experiences of financial abuse, paying attention to the consequences of such harms, and areas for financial service providers to intervene.
Such approaches are epistemologically compatible \cite{becker_epistemological_2007}, as FM is epistemologically neutral \cite{burgess_analyzing_1994}, while discourse analysis can help to surface pre-existing power relationships (a vital component of many IPV-related research projects) \cite{harris_im_2012, van_dijk_principles_1993}.
% Using both in a complementary style can help to identify different elements of the same phenomenon under scrutiny \cite{}. 
% In this section, we first characterize this dataset of \setdupe complaints, and then cover our Methods in greater depth.
In the interest of the growing transparency around work with data \cite{muller_designing_2021, park_facilitating_2021}, particularly with respect to at-risk groups \cite{warford_sok_2022}, we make all of the documentation of the data analysis process transparent in our Appendix \ref{sec:appendix}.}

\paragraph{Framework analysis.}
\edit{
% Framework analysis (FM) originated as an independent qualitative approach by Jane Ritchie and Liz Spencer \cite{}.
FM can be adapted to research that has specific questions \cite{}, a relatively limited timeframe \cite{}, a pre-designed sample (e.g., customers of financial services) \cite{}, and a priori issues (e.g., a lack of organizational responses to financial abuse) that necessitate being dealt with \cite{}.
In FM, data is sifted, charted and sorted in accordance with key issues and themes through familiarization, identification of a thematic framework, indexing, charting, mapping, and interpretation.
% Framework analysis provides an
% excellent tool to assess policies and procedures from the very people that they affect. 
As such, a \textit{framework} in this context refers to an organization of codes, developed jointly by researchers involved in data analysis, that is used to manage and organise data.
We stress that this is different from a theoretical framework (often a research output and contribution in and of itself), described by Eistenhart \cite{eisenhart_conceptual_1991} \textit{``a structure that guides research by relying on a formal theory…constructed by using an established, coherent
explanation of certain phenomena and relationships''}.}

\edit{This framework helped us to summarize and reduce the data to help us answer predefined research questions (\secref{sec:intro}) by providing a new structure for the data.
% As an alternative to using an entirely unstructured approach to the richness of novel data, Framework Method was chosen for this project.
Such a method is optimal when the dataset is already organized via a strict set of schema \cite{eisenhart_conceptual_1991}, such as that of the CFPB data categories. 
As an authorship team, we nevertheless were cautious to resist the pitfalls of conflating framework analysis with an `easier' version of richer qualitative analyses (e.g., Thematic Analysis, Grounded Theory) -- as is commonly reported. 
For instance, we acknowledged that an appropriate interpretation of the matrix and the generation of descriptions, categories, explanations, and typologies require qualitative research skills \cite{gale_using_2013}. 
Moreover, reflexivity, rigor and quality are still key components of the analysis, just as they are in other qualitative methods. 
Therefore, we ensured our study that used the FM was supported by several qualitative researchers (second, third and last authors) with extensive experience in a wide range of analytical methods.}

\paragraph{Data cleaning and analysis}
\label{sec:analysis-character}
\noindent \edit{Our 513 dataset of positive-identified cases of IPFA were first manually reviewed by the second author for any repeat entries (duplicates) or submissions of nearly identical (over 98\% content match) content to different companies (resubmissions).
We discovered that complainants may submit more than one entry if they resubmit their complaints while listing other organizations, while duplicates may be due to server-side errors.
Furthermore, we speculated that there may be services available (e.g., legal offices, support services \cite{}) that assist a survivor of financial abuse to file a complaint with the CFPB, thus expanding the possibility of different destinations being selected as being suitable to receive the complaint.
Following this manual review, we identified 61 total duplicates (4) and re-submissions (57) pertaining to 42 unique customers which were removed from the dataset.
These excluded cases were validated by the first author of this work, and reviewed by the final author.
This resulted in a total of 464 narratives for further analysis.}

\edit{As shown in prior work \cite{bastani2019latent}, user-selected \textit{Product}, \textit{Sub-Product}, \textit{Issue}, and \textit{Sub-Issue} proved to have low levels of accuracy to adequately represent the concerns raised by the customer.
We confirmed this discovery via parsing a randomized sample of 52 entries (10\%) where 36 entries (69.2\% of sample) correctly described at least one of the financial products, while a mere 28 entries described an appropriate issue.
Thus, we chose to exclude these fields and use framework analysis for a deeper dive into better characterizing this dataset \cite{becker_epistemological_2007}.}

% Of a randomized sample of 10\% of this dataset (52 entries), we identified only 36 entries (69.2\%) correctly described one or more of the financial products and a mere 28 entries that identified an appropriate issue (53.8\%). 
% This was determined by reading each narrative and recording multiple services and issues.

\input{figures/tables/framework-table}

% \ronote{TODO: make a table that summarizes this framework}

\paragraph{Crafting a thematic framework.}
\edit{To construct an analytical framework, four researchers deliberated on the `a priori' issues and discussion points identified in the IPFA dataset for creating overarching categories to achieve a \textit{``detailed index''} of our data into \textit{``manageable chunks for subsequent retrieval and exploration''} \cite{ritchie_qualitative_2013}.
We identified which core tenets of IPFA were essential, namely: what their relationship status was (\textit{Relationship Status}); what financial products  were involved (\textit{Financial Product(s)}), and what types of financial abuse were present (\textit{Type of Financial Abuse}).
To help codify some initial categories for the latter, we used a synthesis of pre-existing taxonomies of technology abuse \cite{freed2018stalker}, intimate partner surveillance \cite{tseng2020tools}, technology-enabled financial abuse \cite{Bellini2023paying} and wider economic abuse \cite{bruno_economic_2022}.}

\edit{We then also sought to focus on how survivors of IPFA uncovered this abuse (if covert) by an intimate partner (\textit{Point of Discovery}), and the impact that this abuse had on their health, financial wellbeing, and ability to live a life free from coercive and controlling behaviors (\textit{Consequences of Financial Abuse}).
Finally, with a mind to focus on policy and procedural change, we examined what strategies a complainant could use to achieve a self-identified resolution to this abuse (Method of Resolution), and if they perceived any challenges to attaining this (\textit{Barriers to Help}).
Complainants did not have to explicitly describe this phenomenon as financial abuse in accordance with muted group theory \cite{ardener_ardeners_2005}, which contends that survivors of abuse rarely use the terms that describe their experiences.
Such a procedure of extracting case characteristics from secondary data sources has also been used to great effect by other researchers to better characterize financial abuse in interpersonal settings.}

\edit{Over the space of four weeks, five coders (all co-authors on this work) independently assessed and extracted the relevant data from each CCN in three primary coding rounds.
Coding involved carefully reading each CCN, extracting the information into structured spreadsheets, and converting the data into another format prepped for in-depth analysis.
Each coder coded 20 CCNs cases each to ensure consistency and resolve disagreement.
Second, once consistency was agreed upon in the prior stage, a set of 10 identical CCNs were coded separately to calculate inter-rater reliability early in the process. 
Cohen's kappa was calculated at Product (0.97), Abuse (0.96), Discovery (0.6), and Resolution (0.98) indicating a `near perfect agreement' score for all variables bar \textit{Point of Discovery} \cite{Cohen07}. 
The team identified this disparity was caused by a disagreement between what terminology constituted discovering new information by a survivor, which was subsequently resolved in the following round (0.89).
As inter-rater reliability was high, a decision was made not to double code and compare further CCNs.
All further data were coded by one of the researcher team.
A final round of consistency checking was conducted by one author 
%the second author of this work.
}

\edit{In accordance with the next stage of FM, we rearranged the data and thematic framework to create order, akin to the iterative principle of grounded theory.
We applied this stage as a principle for synthesising and developing our final coding framework through a process of abstraction, in order to derive all the detail from the data and ensure that we were coding elements that may have been missed with simply an a priori approach.
To investigate how our themes relate to each other, we conducted a final stage of mapping and interpreting which involved graphically representing these relationships via a qualitative analysis software Atlas.ti.
Mapping and interpreting essentially are ways of representing pictorially or graphically all of the themes and investigating how each of the themes relates to each other. 
This detailed exploration of the iteratively developed and revised thematic framework enabled us to gain a clearer understanding and explanation of the ‘bigger picture’. 
For instance, we examined the association between our `a priori` categories first identified in our analysis, and we were able to identify and offer explanations for individual discrepancies between these three categories.}

\section{Findings}
\noindent \edit{Our data promotes that there is no a single, common profile of customers whom report financial abuse when they create a complaint to the CFPB.
Namely, while Foohey \cite{foohey_calling_2017} suggest that individuals with higher SES may be more likely to submit a complaint, we identified that survivors represented a spread of different SES, reporting financial losses in the range of \$140 --- \$72,000. \ronote{graph?}
We also hypothesized that survivors may reach out to the CFPB if in a financially safer and more stable position (e.g., post-separation \cite{}); we identified many CCNs that described narratives of severe adversity, desperation, and despair.
Therefore, survivors may be motivated to reach out to submit a formal complaint without a minimum financial threshold being reached.}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.56]{figures/corpus_graphs/product-prop-bre.png}
    \caption{\small The proportion of products described in our analysis, which extend to credit, loan, insurance, debt, utilities, payment, claims, mortgage, and online accounts. The label [unspecified] determines that a complainant mentions the high-level category but not the low-level.}
    \vspace{-0.6cm}
\end{figure}

\edit{We identified that only a single complaint (n=1) identified their experiences as \textit{`financial abuse'}. 
While such terms are relatively newly applied to intimate partner contexts, and survivors rarely use official terminology to describe these forms of behaviors \cite{stylianou2018economic, ardener_ardeners_2005}, we note that this is particularly pressing given our prior discovery --- that a mere 13 CCNs were automatically detected and labelled. 
This clearly highlights the limitation of relying on customers to self-disclose or self-identify such behaviors as financial abuse.}

% attacks
\input{sections/04c_analysis_attacks}

% discovery
\input{sections/04c_analysis_discovery}

% resolutions, next steps
\input{sections/04c_analysis_resolution}

% barriers
\input{sections/04c_analysis_barriers}

==> sections/analysis-reorg/04c_analysis_resolution.tex <==
\subsubsection{How do financial survivors discover and respond to financial abuse?}

We found that the overwhelming majority (n=236) of narratives did not disclose a point of discovery. This could be due to fact that the intake form on the CFPB website does not ask complainants to recall when they first discovered the abuse. Another consideration can be made in the point of engagement when consumers make their complaints, leading to less specificity (e.g., after repeated complaints elsewhere).

Beyond this, we observed that credit reports (n = 44), contact by a collections agency (n = 33), and credit score checks (n = 24) were the most prevalent sources for discovering IPFA from our corpus. Many complainants would mention that they did not realize that they had a financial issue until checking their credit, which falls in line with the common financial advice of checking one's credit score regularly for irregularities. Further, often a complainant was unaware of a debt until that debt had already gone to collections, at which point it had not only affected their credit, but now came with additional near-term consequences such as wage garnishment and harassment from collections agencies. Resolving financial issues from IPFA can be complex, and as matters escalate from the point of discovery, the steps towards resolution can vary as well. 

Most complaints in our corpus detailed filing a complaint with the affected FSP (n = 243) as a method of resolution. Further, we observe that complainants in our corpus reach out to the relevant FSP to help resolve issues either \textit{prior} to reaching out to the CFPB, or \textit{in addition} to it. This highlights the importance of our work in uncovering the role FSPs play in addressing the financial harms of IPFA, since it is evident that complaints and contact \textit{is} made by a large proportion of complainants. Further, we confirm our hypothesis that complaints submitted to the CFPB can be further downstream in a target's resolution journey, marking direct-to-FSP complaints as a valuable source for study in future work that could yield (a) a higher magnitude of possible IPFA, and (b) even more granular information surrounding a target's experiences living with the harms of IPFA. 

We also note an unfortunately high proportion of targets paying off debts associated with IPFA as a means of resolving harms (n = 44). This results in further harm from the original instances of IPFA, and perpetuates the long term harms of this form of abuse. 
Further, we observe that complainants most often pay off outstanding debts from IPFA \textit{alongside} performing some other form of resolution, such as paying off debts \textit{and} submitting a complaint to an FSP (n = 24), or paying off debts \textit{and} submitting a complaint to credit bureaus (n = 5). This could be a result of targets attempting to address the immediate, short-term repercussions of IPFA, and to prevent these short term repercussions from escalating later on while their financial issues are investigated by other stakeholders. Indeed, an example of such can be seen in the following sample from complaint 3356032, where the complainant reaches out to their respective FSP, but also pays off the debt as a result of potential credit impact, as advised by a collections agency: 
\begin{quote}
   \textit{... On [MM/DD/YYYY], [redacted] collections called me with indicating that if I didn't make a payment that day, there would be negative reporting on my credit because we were " at the 40-day mark. I went ahead and MADE A PAYMENT THAT SAME DAY, [MM/DD/YYYY]. Because I was told this payment would avoid negative reporting, I am here alleging erroneous late payment reporting by [redacted] ... } 
\end{quote}
Although we \textit{do} see a majority of complainants within our corpus reaching out to FSPs when attempting to resolve the harms from financial abuse, we clearly see cases where the target needs to take multiple resolution steps that involve multiple stakeholders and potential financial loss. This speaks to the need for further study in understanding how best to support targets in navigating the complexities of resolution, across FSPs and other stakeholders. 

% For example, a complainant detailed suffering financial damage after their IP verbally agreed to take on a debt but changed their mind when it was time to put it into writing (\textbf{financial deception}) \knote{Arka, can you revise this narrative for lying about willingness to take on financial agreement accordingly based on what you saw?}. We also saw cases of an IP tricking the complainant into co-signing onto debts and loans by claiming that their signature was necessary and / or reassuring that the complainant would not be responsible (\textbf{financial deception)}. In 11 complaints, we saw the IP falsely requesting chargebacks---a means for consumers to dispute fraudulent transactions---on the complainant's account in order to cause financial damage (\textbf{fraudulent chargebacks}). Some cases involved the IP disputing valid payments so that the complainant would be unable to pay bills, and in another an IP submitted a false insurance claim under the complainant's name to tarnish their standing.

% These new attacks provide nuances in the ways IPFA occurs, and can lead to better tailoring of advice in turn...
% What did survivors do immediately after realising? 
  % Got in touch with their bank, which is consistent with identity theft literature (I think this is the most popular approach), but we evidence that this also includes a whole host of different types of financial abuse which are not identity theft.

  % We should draw out that survivors often use protective strategies that seem counterintuitive to someone unfamiliar w/ IPV e.g., paying off initial debts.

% Did we find any differences in attack depending on if person was in a relationship or not? 
%   Arka: Yes/No.

% What about elderly? 
%   Not really, to our knowledge.

\Cref{tab:attacks}

==> sections/assessing_performance_CHECK.tex <==
%, and further motivates the use of our workflow for identifying a wider range of complaints. 
% While the keywords that help initiate our workflow are well-grounded in the literature, if our workflow just relied upon them it would have the same limitations. 



%Overall, we observed that our workflow yielded new IPFA complaints that were not present in our IPFA corpus thus far, and also isolates existing IPFA complaints from our reference set well. As seen in \Cref{fig:simcse}, a large proportion of our reference set yield fell into a few clusters. Notably, we observed that cluster 6 encompasses 54.2\% of this initial set. Clusters 3, 6, and 7 encompass 84\% of this initial set. The other clusters contained very small proportions of IPFA reference set complaints when compared to the aforementioned clusters. Upon using our workflow and labeling cluster samples, we found 233 \textit{new} complaints that were not previously identified by keyword matching or during our initial review of the dataset.
%The workflow of \Cref{sec:pipeline} found 225
%\textit{new} complaints that were not previously identified by keyword matching or during our initial review of the dataset
%\paragraph{Keyword Matching.}
%Only 4 of the 233 \textit{new} complaints could be retroactively flagged by keyword search, and were hence missed during the human labelling step of our keyword search method. 
%Only 4 of the 225 new complaints satisfy the keyword matching criteria of \Cref{sec:pipeline} (i.e., at least one keyword or phrase from each of {\tt abuse\_keywords} and {\tt intimate\_partner\_keywords} in close proximity). Hence the LLM-based workflow does expand IPFA identification recall, indeed,
%This shows the high recall of our manual labelling, and demonstrates that even with 100\% recall in manual labelling, 
%over 98\% of complaints identified by the workflow are not identified when \textit{only} using the keyword search method. 

% \begin{enumerate}
%     \setlength\itemsep{0em}
%     \item The complainant \textit{explicitly} refers to an intimate partner using keywords contained in {\tt intimate\_partner\_keywords}.
%     %identifies %and mentions the abusive behavior using keywords contained in {\tt abuse\_keywords}.
%     \item The complainant \textit{explicitly} 
%     %attributes the abusive behavior to the intimate partner and mentions this as the first point / focus of a complaint, hence attributing 
%     mentions abuse using keywords contained in {\tt abuse\_keywords} within a 10 word window of at least one keyword in {\tt intimate\_partner\_keywords}. %\jnote{the commented out text says abuse has to be near an IP mention, but I don't see that in Section 3.3 so I commented it out}
%     %within a certain textual vicinity of the first mention %of an intimate partner.
% \end{enumerate}



% In the final IPFA corpus of 527 complaints, 233 complaints were new complaints found using \textit{only} our LLM pipelines, 176 complaints were found using \textit{only} our keyword search, and 118 were found by \textit{both} of the above methods. Of the 233 complaints produced \textit{only} by our LLM pipeline, just four matched the criteria of our keyword search. That is, over 98\% of complaints identified with our LLM approaches were unidentifiable by the keyword search approach, demonstrating that our LLM pipeline found a wider and larger corpus of IPFA complaints. 


% (the others coming from random sampling (3) and our keyword search (176) and only 2 of these satisfy the keyword match criteria. 
% RESOLVE: change in tense
%\paragraph{Alternative Strategies.}

% To appendix
%\begin{table*}[t]
%\small
%\begin{tabular}{L{.36\textwidth}C{.25\textwidth}C{.1\textwidth}L{.16\textwidth}}
%\hline
%\textbf{S1: Sampling and Preprocessing} & \textbf{S2: Model} & \textbf{S3: Number of Clusters} & \textbf{S4: Est. IPFA Yield from Top Clusters} \\ \hline
%\begin{tabular}[c]{@{}l@{}}\textbf{Experiment 1}\\\textbf{Sample:} 50000 randomly sampled CFPB \\ complaints and reference set/\\\textbf{Preprocessing:} Removed named entities,\\ punctuation, numbers, and stopwords.\\ Lemmatized all tokens.\end{tabular} & bert-large-nli-stsb-mean-tokens & 20 & 0.1 \\ \hline
%\begin{tabular}[c]{@{}l@{}}\textbf{Experiment 2}\\\textbf{Sample:} 44,604 randomly sampled IP \\ complaints and reference set.\\\textbf{Preprocessing:} None\end{tabular} & sup-simcse-roberta-base & 8 & 0.26 \\ \hline
%\end{tabular}
%\caption{A summary of 2 workflows experimented with. The experiment in row 1 samples from the entire CFPB dataset, while row 2 is sampled from the IP Complaints (the preferred workflow). While all experiments isolate IPFA in a small number of clusters, the latter experiment has an IPFA yield that is more than twice the yield of experiment 1. The latter experiment is described in more detail in~\Cref{sec:assess}.}
%\label{tab:experiments}
%\end{table*}

% \begin{table*}[ht]
% \small
% \begin{tabular}{L{.003\textwidth}L{.36\textwidth}C{.25\textwidth}C{.1\textwidth}L{.16\textwidth}}
% \toprule
% & Experiment summary & LLM & Number of Clusters (K) & Est. IPFA yield by cluster \\
% \midrule
% 1 & \textbf{Sample:} $50K$ randomly selected complaints and $359$ IPFA Corpus complaints\newline\textbf{Preprocessing}: Removed named entities, punctuation, numbers and stopwords; lemmatized &
%   %We preprocessed these complaints by removing \\ named entities, punctuation, numbers, and stopwords. \\ Then, we lemmatized and passed the entire processed \\ complaints into the modeling pipeline.\end{tabular} &
%   bert-large-nli-stsb-mean-tokens &
%   20 &
%  % \begin{tabular}[c]{@{}c@{}}50000 randomly selected complaints\\ and 359 high-confidence IPFA complaints\\ from keyword search.\end{tabular} &
%   Max: $.1$\newline
%  2 clusters: $.02$ \newline
%  other clusters: $0$\\  
% \midrule
%   %2 & \begin{tabular}[c]{@{}c@{}}Random sample of $50,000$ and initial IPA corpus ($n=359$).\\
%  % All complete complaints?\\
% % \end{tabular} &
% % miniLM? & 5 & [\textit{don't need this?}] & %\begin{tabular}[c]{@{}c@{}} Max: $.033$\\
% % 2 clusters: $.033$ \\
% % other clusters: 0
% % \end{tabular} \\ \hline
% %\begin{tabular}[c]{@{}c@{}} 
% 2 & \textbf{Sample}: $44,604$ randomly selected \textit{IP complaints} \newline\textbf{Preprocessing}: Removed numbers, redacted content; trimmed to $\sim$5 sentence  window around first mention of IP & 
%  %We preprocessed these complaints by removing\\ redacted content and numbers. After, we trimmed \\ each complaint to be a $\sim$5 sentence  window around \\ the first mention of an IP. Then, we passed the trimmed \\ complaints into the modeling pipeline\end{tabular} &
%   sup-simcse-roberta-base &
%   12 &
%   %44464 complaints containing IP keywords &
%   Max: $.3$\newline
%   2 clusters: $.3$;\newline 1 cluster: $.15$ \newline
%   other clusters: $\leq{.05}$ \\  
% \midrule 
% 3 &
% \textbf{Sample}: $44,604$ randomly selected \textit{IP complaints} \newline\textbf{Preprocessing}: None  &
  
%   %We performed no preprocessing on the complaints. \\ Then, we passed the complaints into the \\ modeling pipeline.\end{tabular} &
%   sup-simcse-roberta-base &
%   8 &
%   %44464 complaints containing IP keywords &
%   Max: $.26$\newline
%   other clusters: $\leq{.06}$\\  
% \bottomrule 
% \end{tabular}
% \label{tab:experiments}
% \caption{A summary of 3 experiments instantiating the detection pipeline of Figure~\ref{fig:model_pipeline}. The experiment in row 1 samples from the entire CFPB complaint narrative corpus, while rows 2 and 3 are sampled from the IP Complaints (i.e. complaints that include at least 1 IP term). While all experiments isolate IPFA in a small number of clusters, the latter two experiments have an IPFA yield that is more than twice the yield of experiment 1. The third experiment is described in more detail in~\Cref{sec:isolating}.}
% % \ronote{missing reference}
% \end{table*}

% We summarized three experiments testing this hypothesis in Table~\ref{tab:experiments}. 
%We also tested our hypothesis that restricting our input sample to IP Complaints in \textbf{S1} improves \textit{IPFA yield} over using a \textit{random sample} of CFPB complaints (see \Cref{tab:experiments} for exact parameters). We find that the experiments sampling from IP Complaints provide an IPFA yield of 0.26 in its top clusters, which is more than twice the alternative workflow which has a yield of 0.1 across its top clusters.



% Experimental Evidence

%\paragraph {Assessing Yield.}
%We observe that 
% Experiment 3 yielded new IPFA complaints that were not present in our IPFA corpus thus far, and also isolates existing IPFA complaints from our reference set well.

% \begin{figure}[!ht]
%     \includegraphics[width=\columnwidth, trim={0 0 0 1cm}, clip]{figures/ipfa_approach_simcse.png}
%     \caption{The distribution of complaints from our reference set present in the corpus that was clustered in experiment 3. Note the evidently higher proportion of reference set complaints contained in clusters 3, 6, and 7.}
%     \label{fig:simcse}
% \end{figure}

% As seen in \Cref{fig:simcse}, a large proportion of our reference set uyield fell into a few clusters. Notably, we observed that cluster 6 encompasses 54.2\% of this initial set. Clusters 3, 6, and 7 encompass 84\% of this initial set. The other clusters contained very small proportions of IPFA reference set complaints when compared to the aforementioned clusters. 

\paragraph{SHAPs scores.}
\label{sec:qual}
In the context of language modeling, SHAP scores identify particular words or phrases that either \textit{positively} or \textit{negatively} contribute to the likelihood that a body of text is assigned a particular class or cluster. 
In executions of the workflow, SHAP scores were used to identify words that have \textit{positive} and \textit{negative} influence on a complaint being assigned to a particular cluster. 
We calculated SHAP scores for a particular, IPFA-dense, cluster by training a random forest classifier on a workflow invocation's results. We used the TF-IDF vectors of each complaint as an input to this classifier, and each complaint's cluster assignment as its classification. 

% The Class TFIDF scores of experiment 3 provided additional evidence proving the notion that LLMs can isolate IPFA. The highest scoring Class TFIDF words (or n-grams) of a particular class are words that are particularly important to the complaints in that class, or in this case, to the cluster assigned to a set of complaints. As a result, these can be used to determine the traits that describe a particular cluster, and contribute to the regional locality of the text embeddings of complaints in the projected vector space. 
% RESOLVE: Change in tense
% For cluster 6, the cluster with the highest proportion of reference set IPFA complaints, we observed the presence of words describing previous intimate partners ("ex husband", "ex wife", "ex spouse"). Further, we noted that \textit{no} other clusters have such a high density of ex intimate partners in their highest scoring Class TFIDF words. Recall from our definitions that IPFA necessitates a pre-existing trusted relationship. The highest scoring Class TFIDF words included the mention of pre-existing trust relationships, and showed that this aspect of IPFA plays a role in the text embeddings produced by LLMs. 

% †c

\input{figures/corpus_graphs/multi-graph-SHAPs}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\columnwidth]{figures/train_explainer/6_train_explainer.png}
%     \caption{\small \sedit{SHAP scores for words in an IPFA-dense cluster in one workflow iteration. Each dot represents a complaint where a SHAP score was calculated. Right of 0.0 indicates a positive influence, left a negative one. Dot color represents the SHAP value magnitude. Note "ex" and "my" positively influence, while "we," "our," and "us" have a negative impact.}}
    
%     % Note how self-possessive words such as "my", as well as the word "ex" describing a previous intimate partner, weight complaints \textit{towards} being classified as a part of cluster 6. On the other hand, words such as "we" and "us" weight complaints \textit{against} being classified in this cluster.}
%     \label{fig:six_shap}
% \end{figure}

% The summary of SHAP scores for cluster 6, the cluster with the highest reference set yield, is shown in \Cref{fig:six_shap}. 

% This summary shows the 20 words with the highest influences on the classification of a complaint as a part of cluster 6. 

We found that the word "ex" had a high positive impact on multiple complaints as being classified as a part of this cluster, further confirming the prevalence of prior intimate partners as an influence in our identification workflow.

If \textit{both} a complainant and their intimate partner are being harmed, 
%we observed that 
the incentive for harming the IP becomes less clear, and IPFA is more difficult to determine. %often results in cases where IPFA is not present at all or more difficult to parse. 

% An example of this, from our CFPB dataset is as follows (from complaint 3735484):

% \begin{quote}
%     \textit{``My husband and I have had a \redact{Capital One} credit card for several years. Due to the COVID-19 State of Delaware mandates, non essential businesses were ordered closed on XX/XX/20 ... my husband is XXXX and the XXXX  he XXXX  and XXXX  was ordered to shut down indefinitely due to the crisis. We contacted our landlord, utility companies and creditors[...]``}
% \end{quote}

% The above complaint does not contain IPFA, and both the complainant and their IP are being harmed by the financial issue being discussed. 

In our SHAP summary, we saw that words such as "our", "we", and "us" had negative impacts on a complaint being classified as a part of the target cluster. Complaints mentioning words such as "our", "we", and "us", may refer to a complainant and their IP as \textit{both} being financially harmed, and may: (1) not satisfy the definition of IPFA 
%fall outside the classification of IPFA according to our definitions 
or (2) involve IPFA that cannot be easily identified due to the abuse having harmful repercussions for the IP and the complainant. For instance, we observe (2) when the complainant explains that \textit{``[w]e were never made aware of this and therefor[e] though payments were being made and made on time they continued to report to our credit bureau...``} (3235817), while describing an undisclosed debt shared between the complainant and their ex-husband. This shows that our workflow
%will be less distinguishing of 
% are less likely to identify IPFA within complaints with inclusive language.
%, matching our observations and definitions.
can distinguish the nature of how complainants describe harm within complaints that can be fundamental for identifying IPFA. 
%\jnote{Arka, let's discuss what is commented out here}
%I think the following is actually orphaned text that accidentally got uncommented, so I am commenting it out, but will add a visible note so that we can discuss
%We present evidence that our iterative workflow supports the isolation and identification of cases of IPFA, and aids in identifying complaints beyond what can be found with other methods. \ronote{We'll need to go further than stating this; we don't provide very much evidence that our system is clearly better than other approaches, and we do not provide evidence that it is able to differentiate fraud or harassment.}
%The iterative executions of the pipeline resulted in a final set of IPFA examples (the ``IPFA Corpus'') of size $n=513$.

% \subsection{Assessing the IPFA Workflow}
% \label{sec:assess}
% \noindent  In this section we provide evidence that  our workflow improves upon IPFA identification via keywords (specifically, those in {\tt abuse\_keywords} and {\tt intimate\_partner\_keywords}).   
% %our workflow synthesizing language models and human review works towards fulfilling the possible issues raised around keyword search. 
% In addition, as mentioned in \Cref{sec:relwork}, language models can lead to biased outcomes and don't have the natural interpretability of keyword matching. 
% We try to explore the bias and linguistic behaviours in language models in our workflow using an explainability technique from cooperative game theory, Shapley values (e.g., \cite{shapley1953value, holzinger2020explainable}. Through this, we aim to better understand how language models help identify complaints aligned with our definition.

==> sections/commented_out.tex <==
% In this work, we conduct the first study that investigates \textit{how} survivors of financial abuse reach out to financial institutions, and \textit{what} kinds of digital-safety challenges they share with respect to financial products. 
% To begin, we systematize previous work to concretely describe the unique characteristics of \textit{intimate partner financial abuse} (IPFA). 

% accounts of consumers who report instances of IPFA in complaints to financial institutions. 
% \jnote{'craft' suggests the results are hard to replicate, can we revise this? Also, is it 524 or 513?}
% Finally, we analyze this dataset using mixed-method analysis to quantitatively measure the lifecycle of a complaint, the customers, and the financial institution response to such harms.
% Using a synthesis of two qualitative analysis approaches --- framework analysis \cite{ritchie_qualitative_2013} and critical discourse analysis \cite{blommaert_critical_2000, kress_critical_1990, fairclough_critical_2012} --- we surface rich insights guided by the following research questions:
% \begin{enumerate}[leftmargin=1cm,label=\bfseries Q\arabic*:]
%     \item What are the key characteristics of \target and \targetter described in complaints containing IPFA?
%     \item What are commonly reported attacks in complaints describing IPFA, and how do these relate to financial institutional processes?
%     \item What barriers do complainants about IPFA concerns report experiencing?
% \end{enumerate}

% into the types of financial harms consumers report experiencing, how they discovered such harms, and the barriers they experienced in reaching out to financial institutions. 


% \jnote{is there a way to work the RQs into the intro? Seems a bit late to be presenting them.}
% \edit{\begin{itemize}
%     \setlength\itemsep{0em}
%     \item \textbf{RQ1.} How do customer-authored descriptions of financial abuse with financial products differentiate it from other forms of financial harm?
%     \item \textbf{RQ2.} What are the self-reported traits of IPFA in customer-authored complaints data that can potentially inform how financial institutions support targets of IPFA in the future?
%     \item \textbf{RQ3.} How might language modelling techniques enable the efficient collection of intimate partner-led financial abuse in large complaints datasets?
% \end{itemize}}


% insights into the financial attacks, common points of discovery, and the barriers faced by survivors in consumer-authored complaints to financial institutions.}

% To summarize, our contributions are: a) we provide the first accessible, human-labelled data-set of /setdupe complaints of intimiate partner financial abuse that is available on request, and b) provide insight into the financial attacks, common points of discovery, and the barriers faced by survivors in customer-authored complaints to financial institutions. To accomplish \textit{a}, we also highlight a definition differentiating intimate partner financial abuse from other harms, as well as an approach for finding instances of intimate partner financial abuse that synthesizes language model-based automation and human review. 

 % \begin{itemize}
 %    \setlength\itemsep{0em}
 %     \item Assembly of a human-labelled data-set of \setdupe complaints of intimate partner financial abuse that is available on request.
 %     \item A workflow for building a corpus of intimate partner financial abuse complaints that blends language model-based automation and human-review to encourage broad coverage of potential cases. 
 %     %\item A workflow for identifying complaints that match our definition of IPFA within large complaints datasets to aid in exploration and triaging.
 %     \item Insight into the forms of financial attack, common points of discovery of IPFA, barriers experienced by survivors and the methods used by survivors to resolve financial hardship caused by IPFA.
 %     %An analysis of our corpus to identify key attacks and traits of self-reported IPFA in consumer complaints, and how these connect to the role of financial institutions in supporting targets of IPFA.
 % \end{itemize}


%%%%%%%%%%%%%%%%%%%%% USENIX INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% surprisingly few works address how digital technologies might address financial abuse in intimate partnerships directly.

% from enabling an abuser to restrict access to their financial accounts, to surveilling a survivor's expenditure online.

% \noindent \edit{Financial institutions face increasing societal pressure to prevent harm to consumers from the growth of digital-safety concerns from the digitization of financial services.}
% % In the past decade, significant progress has been made in protecting older adults, young adults, and low-income people from financial exclusion, fraud, and economic collapse.
% Survivors of intimate partner violence (IPV) face discrete forms of financial harms often lack the ability to recover from sudden financial shocks, which include sudden and unexpected loss of income and/or a sudden and uncontrollable increase in expenditure.
% As a pervasive phenomenon, estimates suggest that 1 in 3 women, 1 in 4 men, and 1 in 2 people in non-binary and transgender community will experience IPV across their lifetime \cite{cdc}.
% Such estimates suggest that survivors of IPV, despite being overlooked as an underserved community represent a substantive subsection of customers who use financial products \cite{}.
% % This is despite an increase in known attack surfaces with the growth of online and digital financial technologies that clearly demonstrate their vulnerability to intimate threats.
% % How digital systems might detect and prevent financial abuse in IPV contexts remains an understudied area, with substantial challenges to security, safety, and right to financial freedom.  While a small number of works have addressed the role of technology in IPV relationships, and how they exacerbate financial harm, surprisingly few works address how digital technologies might address financial abuse in intimate partnerships directly.
% Recent research has highlighted the malicious role that digital technologies can play in exacerbating existing forms of harm.
% Examples include using readily available consumer-facing software to stalk and surveil a survivor without their consent 
% The digitization of consumer finance extends this malicious use-case, percolating its harms across multiple domains that make up a survivor's financial footprint.

% Mitigating financial abuse in IPV contexts necessitates more than an understanding of technology.
% %security and privacy concepts. 
% These are sociotechnical harms, with both technical methods and social factors involved. Therefore, solutions must also be grounded in awareness of challenges that survivors may face---whether it be physical, psychological, or economical. Financial institutions play a key role here, as they continue to update their digital offerings while pledging to advocate for at-risk populations. Mitigiation also necessitates a holistic understanding of how financial abuse in IPV occurs through financial products, how it is described by customers, and the financial products that abusers target to compromise or disrupt.

% Motivated to mitigate such harm to the most vulnerable, we contribute this in-depth investigation into how systems might better detect and contextualize intimate partner financial abuse.

% % One group that often lacks the ability to recover from sudden financial shocks, which include sudden and unexpected loss of income and/or a sudden and uncontrollable increase in expenditure, are survivors of intimate partner violence (IPV).}


% % This is in spite of recent research that suggests that a better understanding of the digital safety violations that at-risk users face might lead to improved approaches to protecting all users of digital technologies. 
% % Such an aspiration is undoubtedly benefrom the potentially long-term repercussions of financial harm.


% \noindent The growth of online and mobile consumer banking has made it convenient for customers to pay bills, monitor finances, and invest~\cite{king2018bank}.
% %partake in investment opportunities~\cite{king2018bank}.
% At the same time, this digital transformation has %perplexed 
% aggravated efforts to protect groups at risk of financial exploitation and harm. 
% Technical attacks on such groups motivated by for-profit adversaries can manifest in subtle ways, thus introducing challenges for detection and prevention.
% Elder financial abuse \cite{deliema2018elder, fraga2022elder, kemp2005elder}, romance scams \cite{schrag2020measurement}, and identity theft \cite{bhargav2006privacy} are just some areas in which prevalent security threat models can be misguided by inaccurate assumptions about device usage and digital safety practices.
% For example, traditional advice for online security, such as the use of strong passwords and multi-factor authentication techniques, need to be appropriately tailored to the specific mental models and technical capabilities of those who are the most vulnerable to attack \cite{roy2018deep, noor2019machine}.
% %JS: commenting out the following sentence; I don't quite understand it and it may be more security-focused than is needed for CSCW?
% %Further challenges come from calls for the cybersecurity community to assist and facilitate in detection and prevention of such attacks in-situ, prior to the devastation that may caused \cite{strohmayer_trust_2021, mckay_standing_2021}.

% One form of subtle, yet highly pervasive harm is that of intimate partner violence (IPV), which is experienced by more than 40\% of women and 25\% of men across their lifetime \cite{IPVsurveillance}. 
% Financial abuse---the control of access to, and maintenance of, financial resources---is anticipated to be present in the majority of IPV contexts \cite{SEA, postmus2012understanding}.
% Recent research has also highlighted the malicious role that digital technologies can play in exacerbating existing forms of harm.
% Examples include using readily available consumer-facing software to stalk and surveil a survivor without their consent \cite{chatterjee_spyware_2018} and collaboration within wide communities of would-be attackers online to share tools and tactics to best enact abuse \cite{tseng2020tools, bellini2021so}.
% The digitization of consumer finance extends this malicious use-case, percolating its harms across multiple domains that make up a survivor's financial footprint. 

% % How digital systems might detect and prevent financial abuse in IPV contexts remains an understudied area (see, \cite{Bellini2023paying} for an overview of available research), with substantial challenges to security, safety, and right to financial freedom.  While a small number of works have addressed the role of technology in IPV relationships, and how they exacerbate financial harm, surprisingly few works address how digital technologies might address financial abuse in intimate partnerships directly. 
% % This is in spite of recent research that suggests that a better understanding of the digital safety violations that at-risk users face might lead to improved approaches to protecting all users of digital technologies. 
% % % Such an aspiration is undoubtedly benefrom the potentially long-term repercussions of financial harm.
% % Motivated to mitigate such harm to the most vulnerable, we contribute this in-depth investigation into how systems might better detect and contextualize intimate partner financial abuse.

% % Add lines about S&P implications as well as financial institutions
% Mitigating financial abuse in IPV contexts necessitates more than an understanding of technology.
% %security and privacy concepts. 
% These are sociotechnical harms, with both technical methods and social factors involved. Therefore, solutions must also be grounded in awareness of challenges that survivors may face---whether it be physical, psychological, or economical. Financial institutions play a key role here, as they continue to update their digital offerings while pledging to advocate for at-risk populations. Mitigiation also necessitates a holistic understanding of how financial abuse in IPV occurs through financial products, how it is described by customers, and the financial products that abusers target to compromise or disrupt. 

% One valuable source of information on such a `hidden' topic, is provided by consumers, customers, and survivors of IPV themselves.
% \edit{Nevertheless, reaching survivors of financial abuse is fraught with difficulties, namely, that such individuals are marginalized, highly vulnerable, and subject to substantive digital-safety risks from a targeted adversary.
% While researchers and advocates have done invaluable work to understand the extent of financial and economic abuse, we take a different approach by focusing on the organizations and the issues they might raise.}
% In this work, we analyze customer complaints submitted to the Consumer Financial Protection Bureau (CFPB)---an agency of the United States government responsible for consumer protection in the financial sector---through 
% %the synthesis of 
% a three-part study.  
% %We first explore the feasibility of using large language models (LLMs) to isolate financial abuse complaints, before analyzing positive matches cases to elicit new understandings from financial abuse.
% %We identify that financially abusive behaviors are more closely aligned to complex social goals, such as power and control, than financial benefit alone. 
% %This results in complaints of financial abuse being correctly categorized as fraud, such as accumulating charges on a credit card, yet incorrectly overlooking the goal of an adversary to damage a survivor's financial well-being may be non-financial.
% First, we systematize previous work on abuse and other financial harms to develop
% %this finding by offering 
% a robust definition of intimate partner financial abuse (IPFA).
% We then present a workflow using
% %discover through the use of 
% BERT-based, pre-trained, language models for collecting a dataset of complaints within large datasets  that satisfy our definition of IPFA. 
% We iteratively deply this workflow to build a corpus of potential IPFA complaints. %This workflow provides a benchmark for future work in triaging, exploring, and studying problems of at-risk populations through consumer complaints.
% Finally, we qualitatively analyze the corpus 
% %perform a deep-dive on the resulting dataset of 
% %a set of 
% %carefully reviewed 
% %examples of IPFA 
% to identify an abusive intimate partner's goals, targets, and potential strategies for causing financial harm (intimate partner is used interchangeably with abbreviation ``IP'' in this manuscript). 
% To the best of our knowledge, we are the first to use language modeling techniques to collect a %dataset for informing novel understandings of how
% data set enabling deeper understanding of how digital financial products are implicated in intimate partner financial abuse contexts. This corpus is available for further study at...\jnote{Ok to link to the github repo given anonymity requirements?}
% To summarize, our contributions are:
%  \begin{itemize}
%     \setlength\itemsep{0em}
%      \item Assembly of a human-labelled data-set of \setdupe complaints of intimate partner financial abuse that is available on request.
%      \item A workflow for building a corpus of IPFA complaints that blends language model-based automation and human-review to encourage broad coverage of potential IPFA cases. 
%      %\item A workflow for identifying complaints that match our definition of IPFA within large complaints datasets to aid in exploration and triaging.
%      \item An analysis of the corpus including the forms of financial attack, common points of discovery of IPFA, barriers experienced by survivors and the methods used by survivors to resolve financial hardship caused by IPFA.
%      %An analysis of our corpus to identify key attacks and traits of self-reported IPFA in consumer complaints, and how these connect to the role of financial institutions in supporting targets of IPFA.
%  \end{itemize}


%%%%%%%%%%%%%%%%%%%%% BEGIN ORIGINAL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \noindent The growth of online and mobile consumer banking has made it convenient for customers to pay bills, monitor their finances, and partake in investment opportunities~\cite{king2018bank}.
% %As a stable contribution to security community, 
% At the same time, this digital transformation has perplexed efforts to protect groups at risk of financial exploitation and harm. 
% Technical attacks motivated by for-profit adversaries can manifest in subtle ways, thus introducing challenges for detection and prevention.
% Elder financial abuse \cite{deliema2018elder, fraga2022elder, kemp2005elder}, romance scams \cite{schrag2020measurement}, and identity theft \cite{bhargav2006privacy} are just some areas whereby existing security approaches can be misguided by inaccurate assumptions about device usage and digital safety practices.
% For example, traditional recommendations for online security, such as the use of strong passwords and multi-factor authentication techniques, need to be appropriately tailored to the specific mental models and technical capabilities of those who are the most vulnerable to attack \cite{roy2018deep, noor2019machine}.
% Further challenges come from
% %More broadly, however, are 
% calls for security to assist and facilitate in detection and prevention of such attacks in-situ, prior to the devastation they may cause \cite{strohmayer_trust_2021, mckay_standing_2021}.

% One form of subtle, yet highly pervasive harm is that of intimate partner violence (IPV), which is experienced by more than 40\% of women and 25\% of men across their lifetime \cite{IPVsurveillance}. 
% Financial abuse---the control of access to, and maintenance of financial resources---is anticipated to be present in the majority of IPV contexts.
% Research has recently highlighted the malicious role that digital technologies can play in exacerbating existing forms of harm.
% Examples include using readily available consumer-facing software to stalk and surveil a survivor without their consent \cite{chatterjee_spyware_2018} and collaboration within wide communities of would-be attackers online to share tools and tactics to best enact their abuse \cite{tseng2020tools, bellini2021so}.
% The digitization of consumer finance extends this malicious use-case, percolating its harms across multiple domains that make up a survivor's financial footprint. 

% How digital systems might detect and prevent financial abuse in IPV contexts remains an understudied area \cite{Bellini2023paying}, with substantial challenges to security, safety, and right to financial freedom.
% While a small number of works have addressed the role of technology in IPV relationships, and how they exacerbate financial harm, surprisingly few works address how digital technologies might address financial abuse in intimate partnerships directly. 
% This is in spite of recent research that suggests that a better understanding of the digital safety violations that at-risk users face might lead to improved approaches to protecting all users of digital technologies. 
% % Such an aspiration is undoubtedly benefrom the potentially long-term repercussions of financial harm.
% Motivated to mitigate such harm to the most vulnerable, we contribute this in-depth investigation into how systems might better detect and contextualize intimate partner financial abuse.

% Mitigation of financial abuse in IPV contexts necessitates a holistic understanding of how it occurs through financial products, how it is described by customers, and the financial products that abusers target to compromise or disrupt. One valuable source of information on such a ``hidden'' topic, is provided by consumers, customers, and survivors of IPV themselves. 
% In this work, we analyze customer complaints submitted to the Consumer Financial Protection Bureau (CFPB)---an agency of the United States government responsible for consumer protection in the financial sector---through 
% %the synthesis of 
% a three-part study.  
% %We first explore the feasibility of using large language models (LLMs) to isolate financial abuse complaints, before analyzing positive matches cases to elicit new understandings from financial abuse.
% %We identify that financially abusive behaviors are more closely aligned to complex social goals, such as power and control, than financial benefit alone. 
% %This results in complaints of financial abuse being correctly categorized as fraud, such as accumulating charges on a credit card, yet incorrectly overlooking the goal of an adversary to damage a survivor's financial well-being may be non-financial.
% First, we systematize previous work on abuse and other financial harms to develop
% %this finding by offering 
% a robust definition of intimate partner financial abuse (IPFA).
% We then leverage a workflow using
% %discover through the use of 
% BERT-based, pre-trained, language models for collecting a dataset of complaints within large datasets  that match our constructed definition of IPFA. This workflow provides a benchmark for future work in triaging, exploring, and studying problems of at-risk populations through consumer complaints.
% Finally, we perform a deep-dive on the resulting dataset of 
% %a set of 
% carefully reviewed 
% examples of IPFA to identify an abusive intimate partner's goals, targets, and potential strategies for causing financial harm (intimate partner is used interchangeably with abbreviation ``IP'' in this manuscript).
% To the best of our knowledge, we are the first to use large-scale modeling techniques to collect a dataset for informing novel understandings of how digital financial products are implicated in financial abuse contexts.
% To summarize, our contributions are:
%  \begin{itemize}
%     \setlength\itemsep{0em}
%      \item A robust definition of IPFA and a first application to the CFPB database, resulting in a set of  $n=527$ IPFA complaints that we will make publicly available. 
%      \item A workflow for identifying complaints that match our definition of IPFA within large complaints datasets to aid in exploration and triaging.
%      \item An analysis of IPFA traits reported by survivors to the CFPB and recommendations for future work securing financial services based on the analysis.
%  \end{itemize}

%%%%%%%%%%%%%%%%%%%%% END   ORIGINAL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \paragraph{RQ1: What is financial abuse? How does it differ from other forms of financial harm?} Because the abuser’s goal is more closely aligned with control than financial gain, IPFA can involve a broad range of behaviors that make it hard to define. For example, while an abuser may accumulate unauthorized charges on their partner's credit card (acts of fraud) they may also more passively damage their partner’s financial health by stopping child support payments or failing to remove their partner from shared loan obligations. In this work, we produce a robust definition of IPFA and a related dataset of $n = 527$ customer complaints that satisfy this definition. 

% \paragraph{RQ2: How can existing language modelling techniques enable the detection of IPFA?}
% %design secure systems for detecting IPFA?} 
% IPFA occurs through a myriad of different technological origins, and may be hard to recognize from just text or verbal descriptions during interactions with survivors. Subtle language differences distinguish between cases in which partners are both financially harmed versus when one partner harms the other. 

% For example, in this redacted complaint filed with the Consumer Financial Protection Bureau (CFPB), a government agency responsible for ensuring consumers are treated fairly by financial organizations,while the following CFPB complaints mentions abuse, the cause of the abuse is not the complainant’s IP: 

% \textit{``XXXX approached my husband and me in XXXX, XXXX about refinancing a mortgage…At this point, our frustration at what we consider to be clearly abusive behavior prompts us to make this complaint…”} 

% In contrast, while the following CFPB complaint characterizes the harm as fraud, it appears to be a case of IPFA: \textit{``my x wife has opened multiple fraudulent accounts in my name, she has opened an account at ginny’s mail order and as such a collection account has been placed on my credit report.’’}. 

% Previous work also shows that IPFA may occur in a covert manner, making it difficult for a survivor to clearly attribute abuse to their intimate partner \anote{paying-the-price}. We provide experimental evidence of the potential for language modeling to 
% %play a significant role in 
% detect IPFA in customer complaints. 
% % In addition, due to the trust partners place in each other, it may be hard to recognize instances of abuse. 

% \paragraph{RQ3: What are the self-reported traits of IPFA in customer complaints data?} Securing digital finance against IPFA requires a thorough understanding of the common attributes of IPFA, and the products it affects. IPFA can cause harm that cascades through multiple sectors of a survivor's financial assets. For example, in the following example, the complainant describes how their former partner’s passive and active behaviors started with an IP overcharging a card and has a compounding effect on the complainant's credit score:

% \textit{``Hello, I have a credit card with Barclays Bank. It is a XXXX Mastercard. While it was in my name, my ex husband ran up a ton of debt, than stopped paying it. I have been trying to pay it, and they will not allow me to. [...] It is unfair to ruin my credit when I am desperately trying to settle the debt owed. My credit has been destroyed, I can't get a mortgage, and despite every attempt on my part to fulfill my financial obligations, I keep hitting a wall. [...] ``} 

% We leverage our data set of IPFA complaints to 
% %topic model 
% identify common traits of IPFA 
% %present in customer complaints, 
% and discuss the insights these traits give for future work securing financial services. Finally, we provide suggestions for future work towards building robust systems for mitigating and securing against the harms of IPFA.

% \textit{``Hello, I have a credit card with Barclays Bank. It is a XXXX Mastercard. While it was in my name, my ex husband ran up a ton of debt, than stopped paying it. I have been trying to pay it, and they will not allow me to. It is no longer at the collections agency so I can't pay them, nor does the original creditor have the account, so I can't pay them either. They are destroying my credit but will not allow me to fix it. My account is somewhere in limbo, and despite numerous phone calls to both the collection agency and creditor, I was still told that I can't pay this debt. It is unfair to ruin my credit when I am desperately trying to settle the debt owed. My credit has been destroyed, I can't get a mortgage, and despite every attempt on my part to fulfill my financial obligations, I keep hitting a wall. I even offered to pay the balance in full immediately, and they refused. I should not be held liable for this debt as I have no way of settling it.``}

% \textit{``Starting in XXXX of XXXX, my now ex-boyfriend stopped paying on our XXXX XXXX credit card, when we broke up in XX/XX/XXXX he said that he was continuing to pay on the card ( he was not ) in XXXX of XXXX, I received a notice that he had filed bankruptcy and went to dig into the status of this account….Starting in XXXX of XXXX, my now ex-boyfriend stopped paying on our XXXX XXXX credit card, when we broke up in XX/XX/XXXX he said that he was continuing to pay on the card ( he was not ) in XXXX of XXXX, I received a notice that he had filed bankruptcy and went to dig into the status of this account.’’}




% \anote{Mention the growth and evolution of different NLP/ML techniques, as they are applied towards cases of abuse detection and understanding datasets. We utilize this advancing literature to begin a vein of study that examines IPFA in complaints. } 

% We systematize existing academic and regulatory work in this area to develop a robust definition of IPFA. By applying the definition to CFPB complaint narratives, we demonstrate that it enables consistent identification of IPFA across multiple labellers and distinguishes IPFA from the closely related financial harms of fraud and harassment. While we focus on the CFPB data set, the definition can be used to identify IPFA in any text narrative.

% We also demonstrate that pretrained large language models (LLMs) are effective in identifying IPFA. Our methodology first restricts to complaints mentioning IPs (``IP complaints’’), generates sentence embeddings using LLMs (e.g., \cite{gao2021simcse}) and clusters the embeddings. We provide experimental evidence that this methodology isolates IPFA complaints in a small number of clusters, thus limiting the amount of human review needed to identify IPFA. 

% Using this methodology we build a corpus of $n=527$ examples of IPFA that we will make publicly available on github. In addition, we provide a case study demonstrating how this corpus can be used to identify patterns in IPFA…[[TBD]]

% To summarize, we make the following contributions:

% \begin{itemize}
%     \item A robust definition of IPFA and a data set of $n=527$ CFPB complaints satisfying the definition. %Assemble the first labeled complaints dataset of financial abuse by intimate partners using Consumer Financial Protection Bureau data.
%     \item Experimental evidence of the potential of pretrained LLMs for detecting financial abuse by intimate partners.
%     \item An initial analysis of IPFA attack descriptions using the IPFA data set. [[note: this may change depending on section 4]] %this labeled complaints data.
% \end{itemize}


% \jnote{Not sure we need this to be a subsection. Alternatively, we can include it in the Introduction with a preface like, ``To summarize, in this work we:...''}


==> sections/deprecated/02_background_new.tex <==
%%%% \jnote{Related to Arka's todo above, 3 areas of previous research to cover here: 1. Intimate partner abuse/violence (e.g., research like \cite{tseng2020tools,tseng2022care}, 2. Complaints Triage (e.g., research like \cite{bastani2019latent} as well as complaints in other contexts), 3. Pretrained vs customized models (e.g., comparing our approach with work like \cite{caselli2020hatebert}). It could also be useful to compare/contrast with elder financial abuse.}

\section{Background and Related Work}
%\section{Background and Related Work}
\label{sec:relwork}
\noindent In this section, we cover relevant prior work to contextualize our contributions. First, we investigate technology-enabled financial abuse, machine learning for disclosure datasets, and our definition of intimate partner financial abuse (IPFA).
%We begin with related work in the areas of technology-enabled financial abuse and machine learning approaches for detecting human and system abuse.
%organized as follows: technology-enabled financial abuse, machine learning and text mining for abuse detecting security vulnerabilities and abuse. 
%We then introduce the context of our investigation: the Consumer Financial Protection Bureau (CFPB) Customer Complaints Database.

\paragraph{Technology-enabled financial abuse and social entanglements.}
\label{sec:background-tefa}
\edit{Social entanglements that complicate traditional approaches to computer security are especially common in the financial realm of intimate relationships \cite{levy}.}
Digital technologies can play a devastating role for social groups who face threats to their financial digital wellbeing, such as victims of child sexual abuse \cite{leary2013fighting}, people trafficking \cite{ali2021improving}, and intimate partner violence (IPV) \cite{freed2018stalker, woodlock2017abuse}.
% Victims of child sexual abuse , people trafficking \cite{ali2021improving}, and intimate partner violence (IPV) are just a few examples of groups facing exclusion from mainstream security approaches that design for a mythical ``average user'', thereby failing to take unique vulnerabilities and safety practices into consideration.
A growing body of work has reinforced that many adversaries use easily accessible systems to compromise a target's accounts \cite{freed2019my, bellini2021so, freed2018stalker, chatterjee_spyware_2018}, surreptitiously track and monitor their GPS location, and doxx their personal identifiable information online.
Unlike other forms of digital threats, such as anonymous identity-related crimes (e.g., identity theft) \cite{identity}, IPV survivors are often trapped by complex sociotechnical and legal factors, meaning that escaping may not always end the abuse \cite{freed_digital_2017}.
Survivors may be required to maintain digital contact with an abuser if they share joint custody of their children \cite{}, and may share the same the same social or professional groups \cite{freed_digital_2017, freed2018stalker}.

% Learning more about how emergent digital technologies are used to harm vulnerable groups, and what meaningful trauma-responsive security response might look like \cite{tseng2022care, slakoff2020role, sharp2015review, freeman2022disturbing} is a fruitful area for further research.

\edit{Social entanglements that complicate traditional approaches to computer security are especially common in the financial realm of intimate relationships \cite{levy}. 
Couples in an intimate partnership may often have shared financial assets, such as housing, cash savings, investments, or business ventures that require shared account access and permissions to be configured appropriately \cite{}.
Emergent work has shown that adversaries use familiar technology-enabled pathways to inflict financial abuse \cite{Bellini2023paying}, such as coercing a survivor to add them as an authorized user, or deceiving them about online expenditure.
While adversaries may be motivated to exploit, monitor, restrict, and sabotage a survivor's digital financial well-being, there is a paucity of work in how survivors interact with professional systems, namely with financial organizations 
% \cite{Bellini2023paying, ellie-butt}. little else is known about how a financial abuser operates outside of survivors who are already receiving care in an IPV ecosystem .
Sources for threat intelligence on such adversaries are increasing each year; from forums of would-be abusers online \cite{bellini2021so, tseng2020tools}, to detecting patterns in computer security support accounts \cite{zou2021role}, the wide range of different sources of information on abuse remains under-utilized by the security community.
In this work, we offer the findings from a three-part investigation into how cases of financial abuse as enacted by an intimate partner might be detected, analyzed, and better understood in the interests of protecting vulnerable customers, users and beyond.}

% Financial abuse -- the control of a person's access and maintenance of financial resources -- has recently been understood as an abuse in its own right (rather than a consequence of the impacts of other forms of IPV) and is estimated to be present in the majority of cases of IPV.
% Financial abuse has been shown to play a part in violence against women (VAW), highlighting the longstanding affects of this form abuse and how it intertwines with other forms of abuse such as sexual and physical abuse \cite{eriksson2021s}.
% While we are grateful that work on elder financial abuse -- financial abuse in elder populations -- is fast emerging \cite{black2008not, fraga2022elder, jackson2021recognizing}, we build on such learning to focus our attention on abuse in intimate partnerships.
% New work, such as in Bellini \cite{paying} identify novel ways for abusers of IPV to use commonly available financial products and services to monitor, restrict, exploit, and sabotage survivors financial well-being.
% In Bellini \cite{paying}, they expand on previous attack taxonomies to demonstrate how commonly available financial products and services currently do not defend against an intimate threat.

\paragraph{Machine learning approaches and disclosure datasets}
\label{sec:background-ml}
%In this work, we focus on what Poirer terms as `disclosure dataset' \cite{poirier2022accountable}, tabular datasets produced in accordance with laws requiring various kinds of disclosure.
Machine learning models have been leveraged for exploring and understanding various forms of user harms including bullying on social media (e.g., \cite{xu2012learning}), toxic online content (e.g., \cite{kumar2021designing}) and intimate partner violence \cite{dehingia2022help, amusa2022predicting, chen2023using}. Abuse detection is challenging in many datasets; consequently, it is often the focus of research in this area including detection of child abuse in patient records \cite{amrit2017identifying}, injuries and abuse types in police reports~\cite{karystianis2019automated}.
%In helping to detect threats unique to vulnerable population groups, specialists have been careful to build supervised systems that assist in detection efforts; such as child abuse in patient records \cite{amrit2017identifying}, and police reports of IPV \cite{karystianis2019automated}. 

Deep learning and natural language processing play a growing role in parsing, analysing, and leveraging large datasets to understand different forms of online harm; particularly those where sociotechnical systems are directly leveraged to inflict harm~\cite{Alsoubai2022friends}. 
For instance, BERT-based transformer models have been fine tuned to provide significant improvements in detecting online hate speech \cite{koufakou2020hurtbert, wullach2021fight}. 
Sentence Transformers based on BERT models have also been expanded for topic modeling in large datasets, using approaches such as BERTopic. BERTopic clusters text embeddings produced by sentence transformer models, allowing a user to understand latent topics present in textual data \cite{grootendorst2022bertopic}. 
Indeed, BERT-based topic modeling has been found to be effective in complex task contexts involving rich and unstructured data like modeling polarizing sentiment surrounding climate change and vaccination \cite{falkenberg2022growing} and analyzing coordinated misinformation campaigns by nation-states on social media \cite{hanley2022happenstance}. 
%particularly often with rich, unstructured, and dense nature of social media text, for tasks such as modeling polarizing sentiment surrounding climate change and vaccination, as well as for analyzing coordinated misinformation campaigns by nation-states on social media \cite{falkenberg2022growing,  hanley2022happenstance}. 
We build on this research with a workflow that uses similar techniques (e.g., sentence transformers and clustering) to identify financial abuse by intimate partners in complaints. 
% To the best of our knowledge, this is the first language model-based workflow for identifying IPFA. 
%Given its success across a realm of different domains, we look towards transformer models and deep learning to inform our efforts analyzing financial abuse by intimate partners. 

As mentioned in \Cref{sec:intro}, financial abuse by intimate partners is a relatively new area of research, and hence, our definition, that systematizes previous is a key contribution. Distinguishing IPFA from other harms involves the identification of subtle and complex distinguishing factors (Table~\ref{tab:dependencies_new}). To meet these challenges, we deliberately use an identification workflow that incorporates both automation through NLP and manual review by expert reviewers (e.g., \cite{ratner2019accelerating}). This hybrid approach has been successful in identifying privacy concerns (e.g., \cite{harkous2022hark,nema2022analyzing}), another complex area with subtle distinctions between itself and the adjacent areas of security and abuse.

\edit{While machine learning clearly holds many benefits in exploring under-explored problem spaces, as Arp et al. \cite{arp2022and} state, we agree that it \textit{``has no clairvoyant abilities''} and requires careful reasoning about data, workflow, and conclusions to not lead researchers into a false sense of achievement.
Common fallacies such as sampling biases, inappropriate threat models, and label inaccuracies can all directly hamper the breakthroughs of important areas of researchers.
Naturally, this has critical knock-on-effects, particularly for at-risk populations who find themselves represented in such datasets through inappropriate labelling and categorization \cite{mathur_disordering_2022, salminen_ethics_2020}. 
With emergent work that underlines that significant caution of the digital and physical safety concerns if such systems fail \cite{chancellor_taxonomy_2019}, there is a drive to ensure such approaches are done sensitively, and safely \cite{chancellor_towards_2022}.
We build on emergent work in this space to apply responsible use of machine learning to elicit novel insights into financial abuse in IPV settings as they intersect with financial products.}

\paragraph{Disclosure datasets.} \edit{In this work, we focus on what Poirer terms as `disclosure dataset' \cite{poirier2022accountable}: \textit{tabular datasets produced in accordance with laws requiring various kinds of disclosure}. In disclosure datasets, stories about discrimination and other forms of corporate and government wrongdoing are often told exclusively from the perspective of the institutions they are intended to monitor.
In addition, disclosure datasets record values that are not neutral but rather rhetorically shaped as they evolve in response to political advocacy, contention, and power.
In spite of the fact that the Consumer Financial Protection Bureau's complaints dataset has been extensively used in research (see, for example, \cite{ayres2013skeletons, haendler2021financial, foohey2017calling}) with just a few exceptions (e.g., \cite{bastani2019latent}), machine learning techniques and complex financial harms have largely not been explored to detect and analyze customer complaints for abuse, and we're not aware of any use of machine learning techniques in the context of IPFA.
In addition, there has been limited attention given to issues such as consumer complaint resolution and barriers to just processes when reporting complaints, despite the clear growth in interest in complaint behavior. 
We aim to offer such a study, to employ machine learning techniques to detect indicators for abuse, as well as to demonstrate how these techniques can be used to evaluate textual data for new learnings on complex social financial harms.
To our knowledge, no previous studies have used machine learning approaches to assess customer complaints around financial abuse across such an extended time period.}

\paragraph{Differentiating intimate partner financial abuse.}
\label{sec:background-definition}
\noindent \edit{Consumers may be harmed with regards to the financial products and assets they own, such as being targeted by a scam, becoming unemployed, or being forced to migrate (e.g., conflict, disaster).
We focus on \textit{targeted} digital financial harm --- caused by a digital attack that is deliberate, purposeful and persistent that leaves a person in a detrimental position in relation to wealth, property or other monetary benefits \cite{stylianou2018economic, sharp2015review}.
Common forms of these attacks are fraud, harassment, and the abuse of older adults (elder financial abuse) \cite{deliema2018elder, mentis_upside_2019}, and between intimate partners (intimate partner financial abuse) \cite{Bellini2023paying, hoge2019domestic}. 
We differentiate these based on adversary type, adversarial goals, and the existence of trust in a relationship (\tabref{tab:dependencies_new}).}

% \edit{Moreover, issues such as scams, harassment, fraud, and abuse play a part in financially \textit{impacting} a consumer, leaving both short and long term effects \cite{empty citation}. 


% \ronote{We probably need to talk about what distinguishes financial harm from financial abuse ...}

% We refer to this space of issues broadly as \textit{financial harms}. 
% \edit{We focus on four important phenomena that has important implications;.
% While financial abuse has been researched in other contexts , challenges remain on how to clearly differentiate it from other forms of financial harms (e.g., financial stress, hardship,  exploitation) across several characteristics . %though research efforts are emergent \cite{postmus-2022} -- and the similarity and differences of various 
% % indeed it is an active area of debate (e.g., ).
% As IPFA has significant overlaps with established financial harms; namely fraud and identity theft, here we delineate this phenomena from other harms (shown in ).}
% Upon careful review of 
% That said, a review of the academic and regulatory literature regarding abuse, fraud and harassment, surfaces repeated themes that form the basis of our definition of IPFA. 
% We describe these themes with supporting references below.

% In this section we define IPFA and contextualize it in terms of more well-known harms, in particular, fraud (the focus of much regulation and government groups, e.g., \cite{van2018financial}) elder financial exploitation \cite{needs citation}, and harassment (driven by the large and growing debt collection industry \cite{zywicki2015law}).  
% This contextual definition is important for determining that the techniques of this paper identify abuse, rather than other harms. 

\edit{\begin{itemize}[leftmargin=0.5cm]
    \item \textbf{Financial Fraud.} Fraud involves a single, or group of individuals (organization) to extract funds from a target with whom they do not have a pre-existing interpersonal, trusting relationship \cite{joudaki2015using,smith2000fraud, anderson2004consumer, soltes2017fraud}. Deception is often used to achieve the offender's main goal, which is financial gain. For example, a merchant who sells a financial product under false terms, such as undisclosed interest rates, defrauds a customer of their money.
    \item \textbf{Financial Harassment.} 
    % Debt collectors \textit{openly} commit financial harassment, perhaps aided by regulations that have not kept up with technology (e.g., \cite{hector2011debt, ludwig2008abuse}). 
    Financial harassment involves a group of individuals (organization) with whom they do not have a pre-existing interpersonal, trusting relationship. Offender objectives are primarily financial, and deception may or may not be used to achieve them. A debt collector, for example, makes repeated and unsolicited calls and/or visits to former customers, which may extend to their family members (e.g., \cite{stace2021debt}).
    \item \textbf{Financial Abuse.} Financial abuse involves a single individual with whom they do have a pre-existing interpersonal, trusted relationship. Offender may seek to harm a target by exploiting, sabotaging, restricting, or monitoring a target's activity related to money. While financial abuse can occur across a range of different interpersonal relationships, we focus on two common manifestations; financial abuse of elders, and financial abuse between intimate partners.
    \setlength\itemindent{25pt} \item \textbf{Elder Financial Abuse.}
% \anote{Maybe a comparison diagram here would be helpful for elder financial exploitation, and IPFA}
    Elder Financial abuse is a form of elder abuse targeting the financial assets of vulnerable elderly adults, which the is recognized federally by the Department of Justice as individuals age 60 or higher \cite{doj}.  Elder financial abuse is typically perpetrated by individuals that already have the trust of an elderly target through a \textit{pre-existing relationship} (such as a caretaker-patient relationship friend, or family member \cite{darzins2010financial, deliema2018elder, nguyen2021perceived,noauthor_metlife_nodate}). Similar to harassment, this form of harm may not rely on deception, and often takes advantage of \textit{cognitive decline} with age \cite{deane_elder_nodate}. Indeed, studies have shown that this form of cognitive decline can have an impact on decision making that increases risk of abuse \cite{spreng2016cognitive}. Further, cases of impairment with age have been shown to result in an increased susceptibility to scams \cite{han2016mild}.  Like fraud, Elder Financial Abuse often occurs under the incentive of financial gain for the abuser, as a result of the accumulated wealth and assets that is observed with age \cite{deane_elder_nodate}. With the establishment of a trusted relationship, this culminates in forms ranging from investment fraud, where an elderly target is tricked by a trusted other into providing funds for a false/fraudulent business venture, to a trusted other stealing funds from the target's accounts \cite{nguyen2021perceived, conrad2011conceptual}.  
    \setlength\itemindent{25pt} \item \textbf{Intimate Partner Financial Abuse.} Intimate partner financial abuse occurs in the context of a romantic partnership (the intimate partner context that is the focus of this paper). The offender may have goals beyond financially benefiting themselves, such as a set of complex social aims around the misuse of power and control over a target \cite{freed_digital_2017, Bellini2023paying}.
\end{itemize}}

\edit{For the purpose of this work are mutually exclusive, with two important caveats; first, to clearly distinguish IPFA from fraud and harassment, we exclude actions that financially harm the perpetrator as well as the target. 
Second, we acknowledge that a case of IPFA may occur in older adults, thus also displaying a form of elder financial abuse. While this overlap is non-significant \cite{storey_risk_2020}, we identify that the predominant motivation for misusing power to \textit{harm} a target's financial health --- a factor that would be counter-intuitive to the financial exploitation of elder financial abuse \cite{Bellini2023paying}.}
\\
% \anote{Below two sections need reworking.}\\


% Some organizations use the volume or frequency of financial harms caused by an offender to differentiate abuse from other harmful acts. The survey scale of economic abuse \cite{adams2008development} explicitly asks about the frequency of harmful acts. Because we seek to identify abuse in individual consumer complaints, each of which may only pertain to a single harmful act, we do not require repetition, but instead distinguish intimate partner financial abuse from other forms of financial harm by the pre-existing trust relationship and the offender’s interest in control.

% \textbf{\textit{Financial Abuse:}} Like harassment, abuse does not require deception. Indeed abusers already have the trust of their target through a pre-existing relationship such as either a caretaker-patient relationship (as in elder financial abuse \cite{darzins2010financial, deliema2018elder}) or a romantic partnership (the intimate partner context that is the focus of this paper). Unlike both harassment and fraud, the offender may have goals other than financially benefiting themselves, such as a set of complex social aims around the misuse of power and control over a target \cite{freed_digital_2017, Bellini2023paying}. In order to clearly distinguish abuse from fraud and harassment, we exclude actions that financially harm the perpetrator as well as the target. 

% Some organizations use the volume or frequency of financial harms caused by an offender to differentiate abuse from other harmful acts. The survey scale of economic abuse \cite{adams2008development} explicitly asks about the frequency of harmful acts. Because we seek to identify abuse in individual consumer complaints, each of which may only pertain to a single harmful act, we do not require repetition, but instead distinguish abuse from other forms of financial harm by the pre-existing trust relationship and the offender’s interest in control.

% We summarize these four distinct categories of financial harm: elder financial abuse, intimate partner financial abuse, fraud, and harassment, in~\Cref{tab:dependencies_new}.
%Categories of financial abuse, harassment, and fraud are mutually exclusive, and offer these %definitions as a means to practically help labelling and categorization efforts in large data-sets.
%Interested readers can view the \rnote{add labelling guidance in Appendix} where we go into %greater depth into how these definitions were developed.\\

% 3 x 3 table displaying dependencies by Fraud, Harassment, Abuse
% Individual or set of individuals (organization)
% Trusting, interpersonal relationship 
% Financially motivated (financial benefit)
% Deception used/not

\begin{comment}
\subsection{Machine learning approaches and disclosure datasets}
\label{sec:background-ml}
%In this work, we focus on what Poirer terms as `disclosure dataset' \cite{poirier2022accountable}, tabular datasets produced in accordance with laws requiring various kinds of disclosure.
Machine learning models have been leveraged for exploring and understanding various forms of user harms including bullying on social media (e.g., \cite{xu2012learning}) and toxic content online (e.g., \cite{kumar2021designing}). Abuse detection is challenging for many data sets and consequently is often the focus of research in this area including, detection of child abuse in patient records \cite{amrit2017identifying}, and injuries and abuse types in police reports  \cite{karystianis2019automated}.
%In helping to detect threats unique to vulnerable population groups, specialists have been careful to build supervised systems that assist in detection efforts; such as child abuse in patient records \cite{amrit2017identifying}, and police reports of IPV \cite{karystianis2019automated}. 

Deep learning and natural language processing play a growing role in parsing, analysing, and leveraging large datasets to understand different forms of online harm; particularly those where sociotechnical systems are directly leveraged to inflict harm. 
For instance, BERT-based transformer models have been fine tuned to provide significant improvements in detecting online hate speech \cite{koufakou2020hurtbert, wullach2021fight}. 
Sentence Transformers based on BERT models have also been expanded for topic modeling in large datasets, using approaches such as BERTopic. BERTopic clusters text embeddings produced by sentence transformer models, allowing a user to understand latent topics present in textual data \cite{grootendorst2022bertopic}. 
Indeed, BERT-based topic modeling has been found to be effective in complex task contexts involving rich and unstructured data like modeling polarizing sentiment surrounding climate change and vaccination \cite{falkenberg2022growing} and analyzing coordinated misinformation campaigns by nation-states on social media \cite{hanley2022happenstance}. 
%particularly often with rich, unstructured, and dense nature of social media text, for tasks such as modeling polarizing sentiment surrounding climate change and vaccination, as well as for analyzing coordinated misinformation campaigns by nation-states on social media \cite{falkenberg2022growing,  hanley2022happenstance}. 
We build on this work by applying similar techniques (e.g., sentence transformers and clustering) to the subtle task of identifying and understanding financial abuse by intimate partners. %Given its success across a realm of different domains, we look towards transformer models and deep learning to inform our efforts analyzing financial abuse by intimate partners. 

As mentioned in \Cref{sec:intro}, financial abuse by intimate partners is a relatively new area of research, and hence, our definition is a key contribution. Distinguishing IPFA from other harms involves the identification of subtle and complex distinguishing factors (Table~\ref{tab:dependencies_new}). To meet these challenges, we deliberately use an identification workflow that incorporates both automation through NLP and manual review by expert reviewers (e.g., \cite{ratner2019accelerating}). This hybrid approach has been successful in identifying privacy concerns (e.g., \cite{harkous2022hark,nema2022analyzing}), another complex area with subtle distinctions between itself and the adjacent areas of security and abuse.

While machine learning clearly holds many benefits in exploring under-explored problem spaces, as Arp et al. \cite{arp2022and} state, we agree that it \textit{``has no clairvoyant abilities''} and requires careful reasoning about data, workflow, and conclusions to not lead researchers into a false sense of achievement.
Common fallacies such as sampling biases, inappropriate threat models, and label inaccuracies can all directly hamper the breakthroughs of important areas of researchers.
Naturally, this has critical knock-on-effects, particularly for at-risk populations who find themselves represented in such data-sets through inappropriate labelling and categorization \cite{mathur_disordering_2022, salminen_ethics_2020}. 
With emergent work that underlines that significant caution of the digital and physical safety concerns if such systems fail \cite{chancellor_taxonomy_2019}, there is a drive to ensure such approaches are done sensitively, and safely \cite{chancellor_towards_2022}.
We build on emergent work in this space to apply responsible use of machine learning to elicit novel insights into financial abuse in IPV settings as they intersect with financial products.

In this work, we focus on what Poirer terms as `disclosure dataset' \cite{poirier2022accountable}: \textit{tabular datasets produced in accordance with laws requiring various kinds of disclosure}. In disclosure datasets, stories about discrimination and other forms of corporate and government wrongdoing are often told exclusively from the perspective of the institutions they are intended to monitor.
In addition, disclosure datasets record values that are not neutral but rather rhetorically shaped as they evolve in response to political advocacy, contention, and power.
In spite of the fact that the Consumer Financial Protection Bureau's complaints dataset has been extensively used in research (see, for example, \cite{ayres2013skeletons, haendler2021financial, foohey2017calling}) with just a few exceptions (e.g., \cite{bastani2019latent}), machine learning techniques and complex financial harms have largely not been explored to detect and analyze customer complaints for abuse, and we're not aware of any use of machine learning techniques in the context of IPFA.
In addition, there has been limited attention given to issues such as consumer complaint resolution and barriers to just processes when reporting complaints, despite the clear growth in interest in complaint behavior. 
We aim to offer such a study, to employ machine learning techniques to detect indicators for abuse, as well as to demonstrate how these techniques can be used to evaluate textual data for new learnings on complex social financial harms.
To our knowledge, no previous studies have used machine learning approaches to assess customer complaints around financial abuse across such an extended time period.
\end{comment}

==> sections/deprecated/02_background_notes.tex <==
\begin{comment}
%\paragraph{Machine Learning and (Systems) Abuse} 
% JS: this section talks both about detecting abuse of humans and systems so removed the '(Systems)'
% The security community is well-versed in automated models for significantly reducing the latency between time of attack and system response.

% Machine learning models have been shown to parse open source intelligence sources to help facilitate important decisions around protecting from security threats \cite{azevedo_pure_2019, ghazi_supervised_2018}, even across multiple languages \cite{ranade_generating_2021} and in spite of data injection attacks \cite{ranade_generating_2021}.

\rnote{We're a little light on explaining how we arrived at these definitions -- if we're positioning them as a contribution I think we need to be mindful of showing our `working out' as it were.}
%\jnote{How about ``Defining'' rather than ``Understanding''? Also, this is a sufficiently large contribution that I think it should be a top-level section; not a subsection}
In this section we define financial abuse and contextualize it in terms of harms that are likely more familiar, fraud and harassment.   
%To have a basis for common understanding, we begin this work by offering a set of terms and definitions on financial harm.
%We do this as while 
This contextual definition is important for determining that our approach is identifying abuse, rather than other harms. It is also a contribution of this paper because while financial abuse has been extensively researched outside of the information security community \cite{stylianou2018economic, sharp2015review}, there is no clear consensus on delineating it from other forms of financial harm -- though research efforts are emergent \cite{postmus-2022} -- and the similarity and differences of various harms are an active area of debate (e.g., \cite{deliema2018elder, Bellini2023paying}) .
%For example, while some scholars have argued that financial exploitation and abuse through technology are interchangeable \cite{deliema2018elder}, others highlight that financial sabotage can also be manifested through technology \cite{Bellini2023paying}
%As such a wide range of behaviors can constitute %financial harm, we drew on 
That said, a review of several key sources of financial harms literature surfaced repeated themes that form the basis of our definition of abuse.


We looked for the presence of interpersonal trust when defining financial abuse. \anote{I would suggest explaining why we looked towards this. i.e. refer back to core elements of leading definitions, if that makes sense.} 
This led us to develop three distinct categories of financial harm: abuse, fraud, and harassment. \Cref{tab:dependencies_new}
Categories of financial abuse, harassment, and fraud are mutually exclusive, and offer these definitions as a means to practically help labelling and categorization efforts in large data-sets.
Interested readers can view the \rnote{add labelling guidance in Appendix} where we go into greater depth into how these definitions were developed.\\

% 3 x 3 table displaying dependencies by Fraud, Harassment, Abuse
% Individual or set of individuals (organization)
% Trusting, interpersonal relationship 
% Financially motivated (financial benefit)
% Deception used/not
\begin{table*}[!htb]
    \centering
    \begin{tabular}{L{0.2\textwidth}L{0.2\textwidth}L{0.2\textwidth}L{0.2\textwidth}}
    \toprule
         & \textbf{Financial Abuse} & \textbf{Financial Fraud} & \textbf{Financial Harassment} \\
    \midrule
         \textit{Adversary} & An individual & An individual, group, or business entity & A set of individuals (organization) \\
    \cmidrule{2-4}
         \textit{Goals} & To exert control over the target, damage target's reputation, or broadly harm the target & To financially benefit through deception & To potentially financially benefit through deception \\
    \cmidrule{2-4}
         \textit{Pre-Existing Trust Relationship} & Yes & No & No \\
    \cmidrule{2-4}
         \textit{Instances} & A romantic partner opens financial accounts (e.g. credit cards) without the victim’s knowledge & Romance scams, deceptive business practices & Collections agency that repeatedly contacts the debt owner and their relatives \\
    \bottomrule
    \end{tabular}
    \caption{Preliminary threat modeling of three disparate forms of financial harm, equipped with adversary type (individual, group or organization); goals; trusted relationship with target; and examples.}
    \label{tab:dependencies_new}
\end{table*}
    % \rnote{Table 1 doesn't quite make sense as romance scams work by the fact they are in a trusting relationship with a target. Either: a) we might frame this as were predominantly in a trusting relationship prior to and during a financial attack? or b) we remove romance scams as an instance of this threat model.}
    % \jnote{I think we need to clarify that the trust relationship is pre-existing in abuse. Romance scams are committed by strangers, i.e. no pre-existing trust relationship. For the scam/fraud to work they first have to gain trust}

\textbf{\textit{Financial Fraud:}} any activity where an offender is either an individual or a set of individuals (organization) with whom the target did not have an interpersonal, trusting relationship. The offender's main goal is financial benefit to themselves and deception is used for an offender to achieve their aim. For example, a merchant who advertises the sale of a financial product under false terms, such as undisclosed interest rates and defrauds a customer of their money. 

\textbf{\textit{Financial Harassment:}} any activity where an offender is a set of individuals (organization) with whom the target did not have an interpersonal trusting relationship. The offenders main goal is financial benefit to the set of individuals. Deception may or may not be used by the offenders to achieve their aims. For instance, predatory lending organizations making continuous and unsolicited calls and/or visits to a former customer and their family members who may owe money.

\textbf{\textit{Financial Abuse:}} any activity where an offender is an individual with whom the target did have, or is presently engaged in having, an interpersonal, trusting relationship. The offender may have goals other than financially benefiting themselves, such as a set of complex social aims around the misuse of power and control over a target. We exclude such actions that directly financially harm an offender, indicating a lack of intention to financially harm. For instance, an abusive partner in the context of an intimate partnership who takes out a loan in a target's name.

\jnote{the following should be in our novel contributions section (current section 4) will move it soon, leaving it here for now}
We expand on these key sites by examining CFPB customer complaints, assembling a five researcher labelling team (all authors on this work) to manually code for relevancy to IPFA and our definitions. 
% To combat the noisiness, linguistic diversity, and complexities of these narratives, 
% We assembled a five-researcher labelling team (all authors on this work) to manually code for relevancy to financial abuse in IPV contexts. 
We coded across multiple rounds, taking a randomized sample of 100-300 complaints a round from the larger CFPB dataset. 
% To do this, we took a randomized sample of approximately $50K$? redacted complaint narratives from our dataset to form a seed set.
% We then re-ran an extended version of the keyword search (see \appref{} for a full list) before allocating each coder with an even level of customer complaints. 
The labelling team conducted eight independent rounds of labelling efforts across the space of five months (July--November 2022), resulting in 3414 total labelled complaints.
Coders participated in exhaustive discussion between rounds regarding edge cases, honing our definitions (introduced above), and determining inter-rater reliability (IRR). Although our IRR varied between rounds as we came across new examples and edge cases to discuss, we had an average IRR of 0.65. Our IRR increased as our definitions for IPFA solidified. \anote{Do we need to mention the IRR across rounds in a table?}
\jnote{It would be great to include a brief (e.g. 1-2 sentence summary). e.g, something like, ``across labeling tasks we achieved a min IRR of...''. I don't think a detailed table is necessary}
\anote{Shifted a description of labelling, to provide basis for how we worked out our definitions}
% For our labelling efforts, we synthesized our analysis criteria from the core elements of leading definitions; such as establishing financial exploitation and abuse should not be considered interchangeably,
\end{comment}

% \begin{center}
% \hline
% \vspace{0.35cm}
% \begin{verbatim}
% intimate_partner_keywords = [...]
% abuse_keywords = [...]
% procedure flag(complaint):
%     if any(keyword from intimate_partner_keywords) 
%             in complaint:
%         index = index of keyword in complaint
%         if any(a_keyword from abuse_keywords) in 
%             complaint[index - 5 : index + 5]
%             return true
% return false
% \end{verbatim}
% \end{center}
% \hline

% Examples of current or former intimate intimate partner include: 

% Formal
% Casual 
% Current Partner
% Partner, spouse, husband, wife, girlfriend, boyfriend, 
% Other half, hubby, missus, Former, Partner, Ex, ex-partner, ex-spouse, ex-husband, ex-wife, ex-girlfriend, ex-boyfriend, X partner, ex

%\jnote{For discussion: The definition and labelling guidelines are a big contribution of this paper. Perhaps the definition and threat model should be one section?}

% Google Doc to FA Guidelines: https://docs.google.com/document/d/1HDQQbFKmG72gUFBkPWpf7zfk5rJTg9WGoVuJwmgtzMc/edit# 

% TODO: 

% TODO: Explain financial abuse vs economic abuse
% FA - money and capital
% EA - access

% Old text below 
% [ Mention about S-BERT too. - Vineeth]

% \section{Threat Modeling IPFA}
% \paragraph{Threat model for IPFA.}
% \label{sec:threat}
% % IPFA describes highly-targeted attacks
% Financial abuse by intimate partners is a result of highly targeted and relatively technically unsophisticated attacks between individuals who have been, or are currently, in an intimate relationship. 
% We presume that the adversary---the abuser---is known to the survivor and has a low barrier to entry to cause financial harm.
% Unlike some other adversaries, abusers can cause especially devastating harm because they violate a trusted relationship with the survivor.
% Technology makes this harm even easier to inflict---most abusers are user interface-bound adversaries (\textit{UI-bound adversaries}) because they use digital products without any software exploits or special tools, albeit maliciously~\cite{freed2018stalker}.
% Often an abuser knows a survivor's personal details and personally identifiable information (PII), such as their social security number (SSN), answers to personal knowledge questions, online accounts, and account activity.
% The abuser can then impersonate the survivor to open new accounts or authenticate as them to access existing accounts (e.g., online account recovery, call center authentication).

% Abusers could also have access physical access to a survivor's devices when they are cohabiting or have visitation rights to see shared children.
% This would allow the abuser---through coercion or secrecy---to physically access the survivor's financial assets and devices, such as credit cards, cash, and mobile banking apps on her phone.
% We consider that an abuser being in the same location also forestalls some online security measures like step-up authentication for unrecognized logins.
% Abusers may have varying motivations for committing technology-based attacks that result in financial abuse that go beyond financial gain \cite{Bellini2023paying}, such as a drive to financially damage the survivor for social goals \cite{haendler2021financial}. 
% As such, we presume that abusers can inflict complicated and long-lasting financial harm on survivors through simple means~\cite{jackson2021recognizing,eriksson2021s}. 


% We add to the existing body of research surrounding intimate partner violence and financial health by leveraging the perspective and importance of machine learning and deep learning models. 
% This work contributes to the growing body of knowledge around abuse as perpetrated through technology, and in understanding the power of complaints data to reveal insights into different issues.


% In order to make these contributions with machine learning and modeling, we focus specifically on complaints data, a source of data well-studied in the past for topic modeling and data mining. 
% CFPB data specifically, has been analyzed through Latent Dirichlet Allocation (LDA), BERT-based topic modeling, and other data mining methods \cite{bastani2019latent, fonseka2016use, fonseka2016use}. 
% These bodies of work have used multiple portions of CFPB complaints data, including the unstructured narratives, but with the motivation of exploring the general insights on \textit{financial} topics as opposed to concepts of financial abuse specifically. 
% Finally, work has been done for creating integrated and automated systems for analyzing complaints data for consumer issues \cite{omurca2021automatic, kalyoncu2018customer, ghazzawi2019analysis}, studies we draw from when discussing the results and potential methods for future study into the automated detection of financial abuse in complaints.

% However, prior work has demonstrated that repopulated menu selections are often inconsistent with the narratives, such as an inability to select more than one product or one concern at a time.

==> sections/deprecated/03b_cfpb_methods_new.tex <==
\section{Data, Tools, and Metrics for IPFA Analysis}
\label{sec:data_tools}

In this section we describe how we extract complaints from the CFPB database and the natural language processing (NLP) techniques we use to build and analyze our IPFA corpus in~\Cref{sec:isolating}.

\subsection{CFPB Data}
%\paragraph{Data collection and cleaning.}
We downloaded our working dataset---totaling 2.2 GB---from the CFPB website in June 2022.\footnote{\url{https://www.consumerfinance.gov/data-research/consumer-complaints/\#download-the-data}. (visited on 06/28/2022).}
At this time, the data were structured across 18 data fields, including the date on which complaints were received by CFPB, product description, customer complaint narrative, and company (for a full list see \apref{tab:cfpb-database-schema}).
To prioritize the experience of those subject to financial abuse, we focused our analysis on the customer complaint narrative -- a free-form text box that did not possess a character limit. We further identified that complainants were not required to submit a customer complaint narrative (CCN). Complaints with a CCN were 1,043 tokens long on average, but varied widely with a standard deviation of 1,276 characters (see \Cref{fig:whole_corpus_lengths}).
% \rnote{Arka did you have some figures on the average of CFPB complaints -- if so could you stick that here and add the graph to the appendix?}
We clarified this finding through viewing the CFPB website that confirmed the submission of a complaint without including the CCN.
As our work sought to focus on customer-identified complaints of financial abuse, we excluded 1,786,680 complaints that did not contain a CCN. 
Each complaint is uniquely identified by a Complaint ID, which we use to refer to complaints within this manuscript and in our analysis. 

While each complaint had a unique ID we identified some duplicate entries, presumably due to customer re-submission, or, the submission of the same complaint through a different party.
After deliberation, we chose to remove duplicates that were submitted on the same day and time (indicative of a technical error), yet opted to retain duplicates if they were customer-authored to further investigate if the same complaint was submitted by the complainant at a later date. 
Our total dataset contains 973,860 complaints. 

%\paragraph{Determining relevancy.}
%JS: this section seems to be about reliability
\paragraph{Data reliability.}
Four field types of the CFPB relate to the pre-populated menu selections of consumer complaints, namely product, sub-product, issue, and sub-issue (\apref{tab:cfpb-database-schema}). 
We sampled a subset of 30 customer complaints with CNNs to judge quality and accuracy of field content to the free-form text; in other words we investigated if customers were selecting different products and issues from the complaint form to the ones described.
We identified that in 28 of the 30 customer complaints there was a distinct deviation from the products and issues described, thereby rendering this data-type unreliable for further analysis.
After reviewing the CFPB complaint submission screen, we identified various issues in the user interface leading to form submission, with the most notable being the inability to select more than one option (e.g., more than one financial product at a time) and hidden sub-options that only become visible upon selection of the higher-level menu option.
These inconsistencies reinforced our interest in focusing on the customer-authored narratives in the data.
Determining why the pre-populated menu selections are often inconsistent with the narratives is a topic for future research.

% However, we note that various restrictions in the UI (e.g., inability to select more than one option or return to previous pages to make changes) are likely a factor. 

% Further, we observe that customers may discuss financial harm across multiple different product and issue categories, making the associated selections less representative of the content of the complaint. In fact, latent topics within CFPB data have been studied previously, yielding delineations within customer complaints that deviate from the selections allowed in these menus, as discussed later. 


% In a first cut analysis of the dataset, we trialled a small sample of relevant keywords sourced by prior literature to determine if complainants were sharing complaints with financial abuse-relevant content (e.g., \textit{husband}, \textit{exploit}, \textit{steal}).
% Our search returned several results that were, unsurprisingly, irrelevant to our focus on intimate partner financial abuse; for instance, a person may complain about a bank \textit{`exploit'}ing themselves and their \textit{`husband'}.
% Although results are clearly are indicative of potentially harmful practice by financial institutions, they do not equate to financial abuse in IPV contexts.

In a first cut analysis of the dataset, we trialled a small sample of relevant keywords sourced by prior literature to determine if complainants were sharing complaints with financial abuse-relevant content (e.g., \textit{husband}, \textit{exploit}, \textit{steal}).
Our search returned several results that were, unsurprisingly, irrelevant to our focus on intimate partner financial abuse; for instance, a person may complain about a bank \textit{``exploit''}-ing themselves and their \textit{``husband''}.
Although results are clearly are indicative of potentially harmful practice by financial institutions, they do not equate to financial abuse in IPV contexts.

\paragraph{Qualitative Analysis Method.}
We expanded on these key sites by examining CFPB customer complaints, assembling a five researcher labelling team (all authors on this work) to manually label for relevancy to IPFA and our definitions. We labeled across multiple rounds, taking a randomized sample of 100-300 complaints per round from the larger CFPB dataset. 

In our first eight rounds of labelling, we found 226 total complaints expressing IPFA, resulting in an 7\% rate of finding cases of IPFA in the CFPB dataset. Of these complaints, 199 complaints were included in our final dataset after a secondary review.
We refer to these and any following human-verified examples of IPFA as \textit{IPFA examples} for the remainder of this manuscript. Additionally, the dataset of IPFA examples that was built is referred to as our \textit{IPFA corpus}. We confirmed early on that financial abuse by intimate partners is present in this dataset, but acknowledged that labelling random samples of data may not be the most efficient. We thus looked towards incorporating a set of approaches using LLMs to source data for labeling rounds and to find new examples for enriching this dataset.


% these labelling efforts may not encompass the variety of how financial abuse by intimate partners appears in CCNs. 


\subsubsection{Data Ethics}
The CFPB data we analyzed is a publicly available data-set that can be downloaded via the CFPB website by any interested party. 
Nevertheless, given the sensitivity of the topic of financial abuse, we were careful to attend to the ethics of using online information about people's financial complaints to derive insights on this phenomena.
Three members of the researchers have extensive experience in researching vulnerable or at-risk populations such as survivors of IPV in security contexts.
As a team of cross academia-industry researchers, we received full approval from the offices of our Institutional Review Board (IRB) and internal legal group prior to commencing this study. 
  
We worked with only redacted data of complaints and we did not pursue the identification of the original posters; albeit the ease of identification of such complaint writers may be of interest to the wider security community.

A key part of our approach involveed human review and labeling of complaints by multiple labelers (for more on this see~\Cref{sec:isolating}). Given the topic matter, the multiple meet up rounds of labeling also acted for joint sense-making for individual labelers  whereby any distressing topic matters could be discussed and processed.




\subsection{NLP Tools and Metrics}
\label{sec:tools}

As previously mentioned, our goal is an iterative strategy that manages manual review time by focusing human review on  smaller groups of complaints that are more likely to contain instances of IPFA. This strategy relies upon several  well-established natural language processing and information retrieval techniques that we describe here. The strategy incorporating these techniques is described in detail in~\Cref{sec:isolating}.


\textit{Keyword Search.} As defined in~\Cref{sec:definition}, IPFA complaints contain: (1) at least one mention of an intimate partner, \textit{and} (2) a description of financial abuse. In our work, complaints containing at least one of the keywords or phrases in {\tt intimate\_partner\_keywords} are considered to satisfy (1), and we term the set of such complaints \textit{IP Complaints}. 

We measured the precision of the IP Complaints by manually reviewing a sample of complaints matching at least one keyword or phrase in {\tt intimate\_partner\_keywords} to determine whether each complaint mentions an IP. Based on a random sample of 100 complaints we estimate the precision of the IP keywords to be $0.95$. Recall is challenging to measure given the relatively low overall rate of complaints mentioning IPs -- a random sample is quite unlikely to contain an IP complaint. In experiment 1 from \Cref{tab:experiments}, we anecdotally observed a higher rate of complaints mentioning an IP within one cluster. To estimate recall, we sampled 100 complaints from this cluster and reviewed the complaints in the sample to determine which match with at least one IP keyword, resulting in an estimated recall of \textit{0.93}. 
%%JS: not sure we can claim this is a lower bound on recall, so revised to ``estimate''

We also leveraged a set of {\tt abuse\_keywords} alongside our existing set of {\tt intimate\_partner\_keywords} to perform an initial keyword search as a benchmark for assessing the effectiveness of LLMs in isolating IPFA complaints as described in~\Cref{sec:isolating}. Both keyword sets are available in \Cref{sec:appendix}.



%\textit{Sentence Embeddings and åing.} 
%For both isolating and Topic Modeling IPFA in complaints,
%We leverage text embeddings and clustering as shown in \Cref{fig:model_pipeline}.
\textit{Sentence Embeddings.} 
Text embeddings represent text in numerical vectors in such a way that passages with similar meanings map to nearby vectors in the vector space. We made use of text embeddings from sentence transformer models, in particular: \textit{bert-large-nli-stsb-mean-tokens} and \textit{sup-simcse-roberta-base} \cite{gao2021simcse, reimers-2019-sentence-bert}. Sentence transformer models have been found to be effective in other complaints contexts (e.g., \cite{chang2020generating}. 

The state of the art in transformer models frequently changes, but we emphasize that the methods of this paper work in conjunction with any transformer model and it is common practice to define methodologies that are not dependent on any particular transformer model, thus allowing for the selected model to change as the state of the art evolves (e.g., \cite{garg2020tanda, kumar2020data}).

Finally, we note that while language models customized for the finance domain are available (e.g., FinBERT \cite{yang2020finbert}), they are tuned to financial documents (e.g., analyst reports, company financial disclosures) rather than the consumer narratives that we use.

\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.35]{figures/model_pipeline.drawio.png}
    \caption{Two pipelines for isolating IPFA using the tools described in \Cref{sec:tools}. Each pipeline begins with a random set of complaints sampled from either the entire set of CFPB Complaints or the IP Complaints. A transformer model is used to generate text embeddings for the sampled complaints. Finally, the embeddings are clustered via K-means and the degree to which the clustering isolates IPFA is measured. We find the upper pipeline (with bolded arrows) to be most effective in isolating IPFA (experimental evidence in Table~\ref{tab:experiments}).}
    \label{fig:model_pipeline}
\end{figure*}

%The second step of these methods rely on clustering text embeddings to isolate IPFA %complaints. 
\textit{Clustering.} Due to the high dimensionality, noisiness, and complexity of CFPB complaints, an outlier-sensitive clustering algorithm like HDBScan tends to leave a large proportion of complaints as outliers. Instead, we relied upon  Spherical K-Means clustering, and experiment with K number of clusters (e.g., \cite{schutze2008introduction}).

\textit{Dependency Parsing and Entity Analysis.}
We leveraged sentence dependency parsing with spaCy to find the direct verb and object pairs associated with each mention of an IP. We also identified the top financial entities mentioned in complaints using spaCy.

\textit{Topic Modeling.}
To understand the topics in sentence level complaint clusters, we used the SHAP and Class TFIDF techniques described earlier. We clustered at the sentence level since sentences are less likely to represent multiple topics. %We use the aforementioned text embedding and clustering techniques to topic model our final IPFA corpus. Complainants may discuss multiple different topics within a given complaint text, but a singular sentence within a complaint will likely discuss one topic, and we leverage this intuition in our approach. 
In particular, for each complaint sentence, we stripped whitespace to the left and right of the sentence, and filtered out any ``sentences'' smaller than 3 words, in order to reduce the noise added by sequences of redacted content within complaints. We used the \textit{sup-simcse-roberta-base} model, and set K = 15 for this analysis.


%\textit{Metrics for Isolating and Modeling IPFA.} For understanding how well language models %isolate IPFA complaints, 
\textit{Metrics.} As mentioned earlier, our goal was to identify smaller groups of complaints that are promising as sources of IPFA complaints. We used the notion of \textit{yield} to quantify this; specifically, the yield of a group is the fraction of IPFA complaints it contains. In practice, we estimated yield in two ways: (1) matching members of a previously identified reference set of IPFA complaints to the clusters they are assigned to, or (2) manually reviewing complaints to determine if they meet the IPFA definition in ~\Cref{sec:definition}. For any experiment, we focused on finding the yield of IPFA complaints in a small number of clusters. 

% by sampling complaints and either: 1. Match members of the sample to previously identified IPFA complaints or 2. Manually review the complaints to determine if they meet the IPFA definition of~\Cref{sec:definition}. For any given experiment in \Cref{tab:experiments}, we estimate the IPFA \textit{yield} for a cluster (or small set of clusters) through random sampling and comparison with known IPFA examples. 

In addition to measuring yield we also evaluated the output of our methods qualitatively, both to ensure the definition of financial abuse is respected and to gain a deeper understanding of the characteristics of financial abuse in CFPB complaints. To achieve these goals we utilized Class TFIDF (as described in BerTopic) \cite{grootendorst2022bertopic}, SHAP (Shapley Additive exPlainability) scores \cite{shapley1953value}, and a \textit{reference set} of previously identified IPFA examples. We determined SHAP scores for a particular cluster by training a random forest classifier on an experiment's results. We used the TFIDF vectors of each complaint as an input to this classifier, and each complaint's cluster assignment as its classification. 



%%The original Section 4 follows commented out
\begin{comment}
\section{Data, Tools and Metrics for IPFA Analysis}
\label{sec:data_tools}
%\subsection{Obtaining a Corpus of CFPB Complaints} 
% To establish the reliability and validity of our definitions, we put together a corpus of CFPB complaints representing IPFA.
In this section we describe how we extract complaints from the CFPB database and the natural language processing (NLP) techniques we use to build and analyze our IPFA corpus in Section~\ref{}.

\subsection{Working with CFPB Complaints}
Recall that we hand code CFPB complaints to gain confidence and hone the bounds of our definitions. In this section, we highlight the steps taken to understand and expand our understanding of the CFPB dataset during that process. 

\paragraph{Data collection and cleaning.}
Our working dataset was pulled from the CFPB website\footnote{\url{https://www.consumerfinance.gov/data-research/consumer-complaints/\#download-the-data}. (visited on June 28, 2022).} at 2.2GB in June 2022.
At this time, data were structured across 18 data fields, inclusive of date complaint were received by CFPB, product description, customer complaint narrative, and company (for a full list see \apref{tab:cfpb-database-schema}).
To prioritize the experience of those subject to financial abuse, we focused our analysis on the customer complaint narrative -- a free-from text box that did not possess a character limit. 
\rnote{Arka did you have some figures on the average of CFPB complaints -- if so could you stick that here and add the graph to the appendix?}
We identified that consumer consumer complaint were not required to submit a customer complaint narrative (CNN).
We clarified this finding through viewing the CFPB website that confirmed the submission of a complaint without including the CCN.
As our work sought to focus on customer-identified complaints of financial abuse, we excluded 1,786,680 complaints that did not contain a CCN. 
Each complaint is uniquely identified by a Complaint ID, which we use to refer to complaints within this manuscript and in our analysis. 

\rnote{I noticed the sentences below were commented out - I've re-added them to the manuscript as reviewers often ask how data were cleaned prior to analysis. If the lines are incorrect, please edit them.}
While each complaint had a unique ID we identified some duplicate entries, presumably due to customer re-submission, or, the submission of the same complaint through a different party.
After deliberation, we chose to remove duplicates that were submitted on the same day and time (indicative of a technical error), yet opted to retain duplicates if they were customer-authored to further investigate if the same complaint was submitted by the complainant at a later date. 
Our total dataset contained 973860 complaints. 

%\paragraph{Determining relevancy.}
%JS: this section seems to be about reliability
\paragraph{Data reliability.}
Four field types of the CFPB relate to the pre-populated menu selections of consumer complaints, namely product, sub-product, issue, and sub-issue (\apref{tab:cfpb-database-schema}). 
We sampled a subset of 30 customer complaints with CNNs to judge quality and accuracy of field content to the free-form text; in other words we investigated if customers were selecting different products and issues from the complaint form to the ones described.
We identified that in 28 of the 30 customer complaints there was a distinct deviation from the products and issues described, thereby rendering this data-type unreliable for further analysis.
After reviewing the CFPB complaint submission screen, we identified various issues in the user interface leading to form submission, with the most notable being the inability to select more than one option (e.g., more than one financial product at a time) and hidden sub-options that only become visible upon selection of the higher-level menu option.
These inconsistencies reinforced our interest in focusing on the customer-authored narratives in the data.
Determining why the pre-populated menu selections are often inconsistent with the narratives is a topic for future research.

% However, we note that various restrictions in the UI (e.g., inability to select more than one option or return to previous pages to make changes) are likely a factor. 

% Further, we observe that customers may discuss financial harm across multiple different product and issue categories, making the associated selections less representative of the content of the complaint. In fact, latent topics within CFPB data have been studied previously, yielding delineations within customer complaints that deviate from the selections allowed in these menus, as discussed later. 


% In a first cut analysis of the dataset, we trialled a small sample of relevant keywords sourced by prior literature to determine if complainants were sharing complaints with financial abuse-relevant content (e.g., \textit{husband}, \textit{exploit}, \textit{steal}).
% Our search returned several results that were, unsurprisingly, irrelevant to our focus on intimate partner financial abuse; for instance, a person may complain about a bank \textit{`exploit'}ing themselves and their \textit{`husband'}.
% Although results are clearly are indicative of potentially harmful practice by financial institutions, they do not equate to financial abuse in IPV contexts.

In a first cut analysis of the dataset, we trialled a small sample of relevant keywords sourced by prior literature to determine if complainants were sharing complaints with financial abuse-relevant content (e.g., \textit{husband}, \textit{exploit}, \textit{steal}).
Our search returned several results that were, unsurprisingly, irrelevant to our focus on intimate partner financial abuse; for instance, a person may complain about a bank \textit{`exploit'}ing themselves and their \textit{`husband'}.
Although results are clearly are indicative of potentially harmful practice by financial institutions, they do not equate to financial abuse in IPV contexts.

\subsection{Data Ethics.}
The CFPB data we analyze is a publicly available data-set that can be downloaded via the CFPB website by any interested party. 
Nevertheless, given the sensitivity of the topic of financial abuse, we were careful to attend to the ethics of using online information about people's financial complaints to derive insights on this phenomena.
Three members of the researchers have extensive experience in researching vulnerable or at-risk populations such as survivors of IPV in security contexts.
As a team of cross academia-industry researchers, we received full approval from the offices of our Institutional Review Board (IRB) and internal legal group prior to commencing this study. 
  
We worked with only redacted data of complaints and we did not pursue the identification of the original posters; albeit the ease of identification of such complaint writers may be of interest to the wider security community. 
Given the topic matter, the multiple meet up rounds of labelling also acted for joint sense-making for individual coders whereby any distressing topic matters could be discussed and processed.

\jnote{plan to move this to the main methodology section}
\paragraph{Labeled IPFA Complaints.}
In our first eight rounds of labelling, we found 226 total complaints expressing IPFA, resulting in an 7\% rate of finding cases of IPFA in the CFPB dataset. 
Of these complaints, 199 complaints were included in our final dataset after a secondary review. 
We refer to these and any following human-coded examples of IPFA as our \textit{IPFA corpus} for the remainder of this manuscript. 
Further, we confirm that IPFA is present in this dataset, but acknowledge that these labelling efforts may not encompass the variety of IPFA cases that appear in CCNs. We thus look towards incorporating a set of language model-based approaches to find new examples for enriching this corpus.


\subsection{NLP Tools and Metrics}

Having defined IPFA and begun building our IPFA corpus with manual labelling, we now examine existing modelling techniques to (1) efficiently build our IPFA corpus further and (2) inform insights for future detection systems (RQ2) \Cref{sec:isolating}. After accomplishing these elements, we work towards identifying natural topics and traits in our final IPFA corpus in \Cref{sec:findings} (RQ3).
%in CFPB complaints}
%\subsection{Obtaining and Analyzing a corpus of IPFA complaints}
% \subsection{IPFA Isolation and Analysis Tools}
\label{sec:obtaining}
\jnote{update: added a new subsection title for discussion}

\paragraph{Tools and Metrics. }We rely on well-established natural language processing techniques and a set of metrics to answer both RQ2 and RQ3.
\label{sec:tools}

\textit{Keyword Matching.}As defined in Section~\ref{sec:definition}, IPFA complaints contain: (1) at least one mention of an intimate partner, \textit{and} (2) a description of financial abuse. In our work, complaints containing at least one of the keywords or phrases in {\tt intimate\_partner\_keywords} (Appendix ?) are considered to satisfy (1), and is used to create a smaller subset of complaints to work from. 

\textit{Sentence Embeddings and Clustering.} For both isolating and Topic Modeling IPFA in complaints, we leverage text embeddings and clustering as shown in \Cref{fig:model_pipeline}. Text embeddings represent text in numerical vectors in such a way that passages with similar meanings map to nearby vectors in the vector space. We make use of text embeddings from sentence transformer models, in particular: \textit{bert-large-nli-stsb-mean-tokens} and \textit{sup-simcse-roberta-base}\cite{gao2021simcse, reimers-2019-sentence-bert}. The state of the art in transformer models frequently changes, but we emphasize that the methods of this paper work in conjunction with any transformer model and it is common practice to  define methodologies that are not dependent on any particular transformer model thus allowing for the selected model to change as the state of the art evolves (see, for example, \cite{garg2020tanda, kumar2020data}).


The second step of these methods rely on clustering text embeddings to isolate IPFA complaints. Due to the high dimensionality, noisiness, and complexity of CFPB complaints, an outlier-sensitive clustering algorithm like HDBScan tends to leave a large proportion of complaints as outliers. Instead, we rely upon  Spherical K-Means clustering, and experiment with the number of clusters (K) (e.g., \cite{schutze2008introduction}).

\textit{Metrics for Isolating and Modeling IPFA.} For understanding how well language models isolate IPFA complaints, we utilize class-TFIDF (as described in BerTopic) \cite{grootendorst2022bertopic}, SHAP (Shapley Additive exPlainability) scores \anote{need a citation here}, and a \textit{reference set} of IPFA complaints. We determine SHAP scores for a particular cluster by training a random forest classifier on an experiment's results. We use the TFIDF vectors of each complaint as an input to this classifier, and each complaint's cluster assignment as it's classification. For any given experiment in \Cref{sec:detection}, we determine the \textit{proportion of reference set assignment} for a cluster (or small set of clusters) as a measure of the proportion of this reference set assigned to the cluster(s) of interest. 

We would also like to analyze how many \textit{new} IPFA examples may be present in clusters. To study this, we take a random sample of complaints in the cluster and via human review, determine the percentage of \textit{new} examples that satisfy the definitions of \Cref{sec:definition}. We term this proportion as the \textit{estimated yield} of a cluster/set of clusters.

\paragraph{Baseline Keyword Search.}
Using the keyword search approach highlighted in \ref{sec:tools}, we flag a total of 1179 complaints. 

Of these, two human coders vet that 359 complaints may or definitely express financial abuse by an intimate partner. Of the complaints labeled in our original labelling, 118 were also found in this search, and 241 were new complaints. 

291 complaints from this search were later confirmed to represent IPFA in our final review, and 115 of these confirmed examples were shared with complaints that were confirmed from our dataset of hand-labeled examples. 

Already, we find a larger quantity of IPFA examples than from our initial labelling efforts relative to the efficiency of our initial efforts. This search method relies on two key assumptions, amongst others:
\begin{enumerate}
    \item The complainant mentions \textit{explicitly} identifies and mentions the abusive behavior of an intimate partner.
    \item The complainant \textit{explicitly} attributes the abusive behavior to an intimate partner and mentions this as the first point/focus of a complaint, hence attributing abuse within a certain textual vicinity of the first mention of an intimate partner. 
\end{enumerate}

These assumptions may not hold in all cases, such as (1) when the complainant is not entirely sure that their intimate partner is financially abusing them, (2) when the complainant does not focus on abusive behavior from the beginning of their complaint, and (3) the complainant is actually a perpetrator of abuse, and hence does not describe their behavior towards an intimate partner as abusive.

\paragraph{Language Models and Isolating IPFA Complaints.}
Given the simplicity of our keyword search method, we leverage our other tools as seen in Figure \ref{fig:model_pipeline} to identify additional complaints by isolating IPFA. Using our existing IPFA corpus as our reference set, we deploy our previously described text embedding and clustering tools on subsets of the larger CFPB dataset. Running the pipeline on the entire complaints dataset was determined to be prohibitively time consuming. Consequently, we experiment with two different subsets:
\begin{enumerate}
    \item A 50,359 complaint subset that contains 50,000 randomly sampled complaints, and 359 complaints present in our reference set. 
    \item A 44,604 complaint subset that contains all complaints in the larger CFPB dataset that mention an intimate partner at least once (using the algorithm mentioned in \ref{sec:tools}). Note that all complaints in this set will necessarily include the mention of an Intimate Partner, therefore guaranteeing that the majority of our reference set is present in the corpus being modeled, based on the precision and recall rates of our keyword search. 
\end{enumerate}

To account for the noisiness of our data, we also experiment with different levels of preprocessing on CCNs, prior to passing into the modeling pipeline. The details of this can be found in \Cref{tab:experiments}. Ultimately, we show that this pipeline, despite no fine-tuning of models, can reveal \textit{new} examples of IPFA that have not been uncovered using our previous approaches. 

\paragraph{Analyzing the IPFA Corpus.}
Recall that to answer RQ3, we aim to identify natural topics and traits present in our final IPFA corpus. To do so, we leverage sentence dependency parsing with spaCy to find the direct verb and object pairs associated with each mention of an IP, and identify the top financial entities mentioned in complaints. Finally, we use the aforementioned text embedding and clustering techniques to topic model our final IPFA corpus. Complainants may discuss multiple different topics within a given complaint text, but a singular sentence within a complaint will likely discuss one topic, and we leverage this intuition in our approach. For each sentence, we strip whitespace to the left and right of the sentence, and filter out any 'sentences' smaller than 3 words, in order to reduce the noise added by sequences of redacted content within complaints. We use the \textit{sup-simcse-roberta-base} model, and set K = 15 for this analysis. 
\end{comment}




==> sections/deprecated/04a_isolating_ipfa.tex <==
%\subsection{Iterative Detection Pipeline}
% \section{Findings: Isolating IPFA Complaints}
\section{Building an IPFA Corpus}
\label{sec:isolating} 
%We conduct 
%3 total 
Through a series of experiments we developed an iterative pipeline for building an IPFA corpus, and we  examined \textit{how} LLMs influenced the identification of IPFA. The final pipeline is shown in the upper flow of Figure~\ref{fig:model_pipeline}. In short, the pipeline works by comparing clusters of complaints embeddings with a reference set of known positive examples, helping to focus human review of complaints, which results in additions to the corpus. In the following we describe the pipeline in more detail, provide qualitative insights into \textit{how} the pipeline identifies IPFA and provide quantitative evidence that the pipeline improves over 2 other approaches: a simpler pipeline (the lower flow in Figure~\ref{fig:model_pipeline}), and keyword matching.

\begin{table*}[ht]
\begin{tabular}{L{.003\textwidth}L{.36\textwidth}C{.25\textwidth}C{.1\textwidth}L{.16\textwidth}}
\toprule
& Experiment summary & LLM & Number of Clusters (K) & Est. IPFA yield by cluster \\
\midrule
1 & \textbf{Sample:} $50K$ randomly selected complaints and $359$ IPFA Corpus complaints\newline\textbf{Preprocessing}: Removed named entities, punctuation, numbers and stopwords; lemmatized &
  %We preprocessed these complaints by removing \\ named entities, punctuation, numbers, and stopwords. \\ Then, we lemmatized and passed the entire processed \\ complaints into the modeling pipeline.\end{tabular} &
  bert-large-nli-stsb-mean-tokens &
  20 &
 % \begin{tabular}[c]{@{}c@{}}50000 randomly selected complaints\\ and 359 high-confidence IPFA complaints\\ from keyword search.\end{tabular} &
  Max: $.1$\newline
 2 clusters: $.02$ \newline
 other clusters: $0$\\  
\midrule
  %2 & \begin{tabular}[c]{@{}c@{}}Random sample of $50,000$ and initial IPA corpus ($n=359$).\\
 % All complete complaints?\\
% \end{tabular} &
% miniLM? & 5 & [\textit{don't need this?}] & %\begin{tabular}[c]{@{}c@{}} Max: $.033$\\
% 2 clusters: $.033$ \\
% other clusters: 0
% \end{tabular} \\ \hline
%\begin{tabular}[c]{@{}c@{}} 
2 & \textbf{Sample}: $44,604$ randomly selected \textit{IP complaints} \newline\textbf{Preprocessing}: Removed numbers, redacted content; trimmed to $\sim$5 sentence  window around first mention of IP & 
 %We preprocessed these complaints by removing\\ redacted content and numbers. After, we trimmed \\ each complaint to be a $\sim$5 sentence  window around \\ the first mention of an IP. Then, we passed the trimmed \\ complaints into the modeling pipeline\end{tabular} &
  sup-simcse-roberta-base &
  12 &
  %44464 complaints containing IP keywords &
  Max: $.3$\newline
  2 clusters: $.3$;\newline 1 cluster: $.15$ \newline
  other clusters: $\leq{.05}$ \\  
\midrule 
3 &
\textbf{Sample}: $44,604$ randomly selected \textit{IP complaints} \newline\textbf{Preprocessing}: None  &
  
  %We performed no preprocessing on the complaints. \\ Then, we passed the complaints into the \\ modeling pipeline.\end{tabular} &
  sup-simcse-roberta-base &
  8 &
  %44464 complaints containing IP keywords &
  Max: $.26$\newline
  other clusters: $\leq{.06}$\\  
\bottomrule 
\end{tabular}
\label{tab:experiments}
\caption{A summary of 3 experiments instantiating the detection pipeline of Figure~\ref{fig:model_pipeline}. The experiment in row 1 samples from the entire CFPB complaint narrative corpus, while rows 2 and 3 are sampled from the IP Complaints (i.e. complaints that include at least 1 IP term). While all experiments isolate IPFA in a small number of clusters, the latter two experiments have an IPFA yield that is more than twice the yield of experiment 1. The third experiment is described in more detail in~\Cref{sec:isolating}.}
% \ronote{missing reference}
\end{table*}

 
% At a high level, 

%\jnote{Arka, there are 4 experiments in the deck -- 2 for each method?}
% RESOLVE: Change of tense in this section
\paragraph{Pipeline Overview.}
 %We combine the newly found complaints from this search with previously manual-coded examples to create a reference set for assessing the capabilities of LLMs. 
To form an initial reference set of IPFA examples, we used the keyword search approach from \Cref{sec:tools} in conjunction with the keyword sets, {\tt intimate\_partner\_keywords} and {\tt abuse\_keywords}. Through this, we identified 1,179 complaints mentioning an intimate partner \textit{and} an abuse keyword. 
Two human labelers reviewed the 1,179 complaints and determined that 291 meet the definition of IPFA (\Cref{sec:definition}). 

We initiate the pipeline with a random sample of IP complaints and our reference set. The pipeline generates text embeddings on this set  and clusters the embeddings using K-means. The clusters are then assessed for the proportion of reference set examples.  The cluster(s) with the highest IPFA yield (with respect to the reference set) are reviewed by humans. Any complaints found to match the definition of IPFA during review are added to the reference set and used in subsequent iterations of the pipeline. 

We executed this pipeline several times for various values of K, ranging from 3 to 20, 
% \jnote{can we add a range? do we have a rough idea of how many executions?} 
and with 2 different sentence transformer models. In each iteration, our input  was limited to a sample of approximately $50,000$ random IP complaints, in addition to the reference set, for efficiency reasons. The iterative executions of the pipeline resulted in a final set of IPFA examples (the ``IPFA Corpus'') of size $n=527$.

\subsection{Comparison with Other Approaches}
\label{sec:compare}
We compare the performance of our recommended pipeline with the keyword search strategy that we used to form the first reference set of IPFA examples, and the simpler pipeline shown in the lower flow of Figure~\ref{fig:model_pipeline}.

\paragraph{Keyword Matching.}
Keyword matching using a conjunction of the 2 keyword lists {\tt intimate\_partner\_keywords} and {\tt abuse\_keywords} relies on three key assumptions:
\begin{enumerate}
    \setlength\itemsep{0em}
    \item The complainant \textit{explicitly} identifies and mentions the abusive behavior using keywords contained in {\tt abuse\_keywords}.
    \item The complainant \textit{explicitly} attributes the abusive behavior to the intimate partner and mentions this as the first point / focus of a complaint, hence attributing abuse within a certain textual vicinity of the first mention of an intimate partner.
\end{enumerate}

These assumptions may not hold in all cases, such as (1) when the pairs of intimate partner and abuse keywords are too restrictive and do not encompass all forms of IPFA, and (2) when the complainant is not entirely sure that their intimate partner is financially abusing them. 

Additionally, any keyword search strategy decreases the possibility of discovering new patterns or forms of IPFA due to its dependence on a pre-determined model (by proxy of keywords) of IPFA. In the final IPFA corpus of 527 complaints, 233 complaints were new complaints found using \textit{only} our LLM pipelines, 176 complaints were found using \textit{only} our keyword search, and 118 were found by \textit{both} of the above methods. Of the 233 complaints produced \textit{only} by our LLM pipeline, just four matched the criteria of our keyword search. That is, over 98\% of complaints identified with our LLM approaches were unidentifiable by the keyword search approach, demonstrating that our LLM pipeline found a wider and larger corpus of IPFA complaints. 


% (the others coming from random sampling (3) and our keyword search (176) and only 2 of these satisfy the keyword match criteria. 
% RESOLVE: change in tense
\paragraph{Alternative Pipeline.}
We tested the hypothesis that restricting our input sample to IP Complaints (i.e., the top flow in~\Cref{fig:model_pipeline}) improves IPFA yield over using a random sample. We summarized three experiments testing this hypothesis in Table~\ref{tab:experiments}. The two experiments sampling from IP Complaints provide an IPFA yield that is more than twice the experiment that samples from the entire complaint population (a difference that consistently holds across experiments). We describe one of these higher yield experiments (experiment 3) in detail below.

% Experimental Evidence



%\paragraph {Assessing Yield.}
%We observe that 
Experiment 3 yielded new IPFA complaints that were not present in our IPFA corpus thus far, and also isolates existing IPFA complaints from our reference set well. We first looked at the proportions of reference set assignments across clusters as an estimator of yield. 

\begin{figure}[!ht]
    \includegraphics[width=\columnwidth, trim={0 0 0 1cm}, clip]{figures/ipfa_approach_simcse.png}
    \caption{The distribution of complaints from our reference set present in the corpus that was clustered in experiment 3. Note the evidently higher proportion of reference set complaints contained in clusters 3, 6, and 7.}
    \label{fig:simcse}
\end{figure}

As seen in \Cref{fig:simcse}, a large proportion of our reference set fell into a few clusters. Notably, we observed that cluster 6 encompasses 54.2\% of this initial set. Clusters 3, 6, and 7 encompass 84\% of this initial set. The other clusters contained very small proportions of IPFA reference set complaints when compared to the aforementioned clusters. Spherical K-Means clustering assigns complaints to the same cluster if they are close (by a particular distance metric) to a common cluster ``center'' in vector space. Given that 84\% of our IPFA reference set is contained in a few small clusters, it is evident that LLMs are able to group and isolate IPFA as the text embeddings produced are close in the projected vector space. 

If a set of our reference set of IPFA complaints are close together in the projected vector space, it is sensible to hypothesize that \textit{other} IPFA complaints may also be assigned to the same cluster. Upon performing further labelling on a random sample of 500 complaints in cluster 6, we found 123 \textit{new} IPFA examples after review by three total human coders, leaving a yield of 123 / 500 = 24.6\%. Not only does this methodology cluster
%seem to encompass 
complaints identified using previous approaches, but it also finds \textit{new} complaints that express IPFA that were not identified with previous approaches. This demonstrates further how LLMs are able to effectively isolate IPFA complaints, even if they are not fine-tuned on notions of financial abuse.
\subsection{Qualitative Insights from the Pipeline}
\label{sec:qual}

An important challenge when using an LLM-methodology for detection is understanding \textit{how} the methodology detects the intended phenomenon. In our context, this means understanding what linguistic patterns the methodology recognizes as similar (resulting in clustering) and how this may bias the IPFA corpus toward certain forms of IPFA.

To qualitatively describe how our proposed methodology works we provide Class TFIDF and SHAP scores (Section~\ref{sec:data_tools}) for a specific execution of our pipeline, experiment 3 from Table~\ref{tab:experiments}.

The Class TFIDF scores of experiment 3 provided additional evidence proving the notion that LLMs can isolate IPFA. The highest scoring Class TFIDF words (or n-grams) of a particular class are words that are particularly important to the complaints in that class, or in this case, to the cluster assigned to a set of complaints. As a result, these can be used to determine the traits that describe a particular cluster, and contribute to the regional locality of the text embeddings of complaints in the projected vector space. 
% RESOLVE: Change in tense
For cluster 6, the cluster with the highest proportion of reference set IPFA complaints, we observed the presence of words describing previous intimate partners ("ex husband", "ex wife", "ex spouse"). Further, we noted that \textit{no} other clusters have such a high density of ex intimate partners in their highest scoring Class TFIDF words. Recall from our definitions that IPFA necessitates a pre-existing trusted relationship. The highest scoring Class TFIDF words included the mention of pre-existing trust relationships, and showed that this aspect of IPFA plays a role in the text embeddings produced by LLMs. 

% †c

SHAP scores are a common explainability metric used in understanding the effect or weight of certain features in a machine learning model's classification. In the case of language modeling, this can involve identifying particular words or phrases that may invoke a \textit{positive} or \textit{negative} weight towards a body of text being assigned a particular class. Further still, in the context of our experiments, SHAP scores were used to give us general benchmarks on the words that have \textit{positive} and \textit{negative} influence on a particular complaint being assigned to its relative cluster. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/6_train_explainer.png}
    \caption{The SHAP Explainability Summary for cluster 6 of experiment 3 -- this cluster had the highest proportion of reference set complaints. Note how self-possessive words such as "my", as well as the word "ex" describing a previous intimate partner, weight complaints \textit{towards} being classified as a part of cluster 6. On the other hand, words such as "we" and "us" weight complaints \textit{against} being classified in this cluster.}
    \label{fig:six_shap}
\end{figure}

We ran SHAP explainability on cluster 6 from experiment 3 (see \Cref{fig:six_shap}), and produced a summary showing the 20 words with the highest influences on the classification of a complaint as a part of cluster 6. We found that the word "ex" had a high positive impact on multiple complaints as being classified as a part of cluster 6. This further confirmed the prevalence of prior intimate partners we observed with Class TFIDF on this cluster, as it often precedes the mention of a prior intimate partnership.


\begin{table}[!ht]
\begin{tabular}{C{.06\linewidth}L{.84\linewidth}}
\toprule
{\scriptsize\textbf{Cluster}} & {\scriptsize \textbf{20 highest scoring cTF-IDF bigrams}} \\
\midrule
% \scriptsize{0} & {\scriptsize{[}`student loans' `student loan' `loan modification' `make payments' `repayment plan' `lost job' `make payment' `payment plan' `monthly payment' `making payments' `mortgage company' `late payments' `monthly payments' `credit score' `credit report' `income based' `years ago' `mortgage payment' `mortgage payments' `received letter'{]}} \\ 
% \midrule
% \scriptsize{1} & {\scriptsize {[}`loan modification' `mortgage company' `mortgage payment' `mr cooper' `mortgage payments' `credit report' `make payment' `customer service' `late fees' `make payments' `monthly payment' `late payment' `escrow account' `received letter' `mortgage loan' `credit score' `short sale' `late payments' `making payments' `credit bureaus'{]}} \\ 
% \midrule
% \scriptsize{2} & {\scriptsize {[}`loan officer' `loan modification' `mortgage company' `short sale' `mortgage payment' `mr cooper' `mortgage loan' `closing date' `title company' `escrow account' `mortgage payments' `credit report' `received letter' `monthly payment' `closing costs' `home loan' `credit score' `real estate' `quicken loans' `customer service'{]}} \\ 
% \midrule
% \scriptsize{3} & {\scriptsize {[}`credit card' `checking account' `customer service' `debit card' `bank account' `account closed' `close account' `savings account' `closed account' `credit cards' `money account' `fraud department' `new account' `business days' `opened account' `card account' `joint account' `account number' `phone number' `new card'{]}} \\ 
% \midrule
% \scriptsize{4} & {\scriptsize {[}`credit card' `credit report' `customer service' `credit score' `did'nt' `received letter' `collection agency' `phone number' `make payment' `did receive' `received email' `card company' `let know' `did want' `days later' `called told' `credit cards' `annual fee' `phone calls' `insurance company'{]}} \\ 
% \midrule
\scriptsize{5} & {\scriptsize {[}`phone number' `cell phone' `stop calling' `phone calls' `times day' `debt collector' `collect debt' `called number' `debt collection' `collection agency' `legal action' `number called' \textbf{`ex husband'} `place employment' `received phone' `personal information' `social security' `phone numbers' `family members' `multiple times'{]}} \\ 
\midrule
\scriptsize{6} & {\scriptsize {[}`credit report' \textbf{`ex husband' `ex wife' `divorce decree'} `credit card' `credit score' `credit bureaus' `filed bankruptcy' `collection agency' `removed credit' `years ago' `credit reports' \textbf{`ex spouse'} `identity theft' `social security' `court order' `credit cards' `authorized user' `credit reporting' `passed away'{]}} \\ 
\midrule
\scriptsize{7} & {\scriptsize {[}`credit reporting' `credit report' `consumer report' `fair credit' `reporting act' `reporting agency' `identity theft' `consumer reporting' `debt collection' `reporting agencies' `credit reports' `collection practices' `fair debt' `credit bureaus' `practices act' `credit card' `section title' `debt collector' `employment purposes' `united states'{]}} \\ 
\bottomrule
\end{tabular}%
\caption{The 20 highest class TFIDF Scored bigrams for clusters 5, 6, and 7. The keywords and phrases related to intimate partners are in bold. Note that most of these phrases are in cluster 6 and all refer to partnerships that have ended (E.g. ``ex husband''). All other clusters had no relevant high scoring words.}
\label{fig:trigram_tfidfs}
\end{table}

According to our definitions, an abuser's primary motivation for IPFA often involves harming the target, or survivor. If \textit{both} a complainant and their intimate partner are being harmed, we observed that the motivation of harming an IP becomes less clear, and often results in cases where IPFA is not present at all or more difficult to parse. An example of this, from our CFPB dataset is as follows (from complaint 3735484:

\begin{quote}
    \textit{``My husband and I have had a \redact{Capital One} credit card for several years. Due to the COVID-19 State of Delaware mandates, non essential businesses were ordered closed on XX/XX/20 ... my husband is XXXX and the XXXX  he XXXX  and XXXX  was ordered to shut down indefinitely due to the crisis. We contacted our landlord, utility companies and creditors[...]``}
\end{quote}

The above complaint does not contain IPFA, and both the complainant and their IP are being harmed by the financial issue being discussed. In our SHAP summary, we saw that words such as "our", "we", and "us" had negative impacts on a complaint being classified as a part of cluster 6. Complaints mentioning words such as "our", "we", and "us", may refer to a complainant and their IP as \textit{both} being financially harmed, and may: (1) fall outside the classification of IPFA according to our definitions or (2) involve IPFA that cannot be easily identified due to the abuse having repercussions for the IP and the complainant. This is clearly reflected in the SHAP scores of cluster 6, and exemplifies the previous notion of inclusionary language, showing that LLMs will be less certain regarding IPFA within complaints where inclusionary language is used, matching our observations and definitions.

We present a strong body of evidence that our iterative LLM pipeline supports the isolation and identification of cases of IPFA, and does so better than other approaches. Further, we develop an IPFA corpus of 527 total complaints that align with our definitions of IPFA, giving us a benchmark data set to study various characteristics of IPFA.

\begin{comment}
%Of the complaints labeled from our manual labelling previously, 115 were shared with this set.
%%Arka, do we need the above sentence? (the one I commented out -- I think we will lose reviewers
%based on our initial definitions and labelling guide. 

% Of the complaints labeled in our manual labelling previously, 118 were also found in this search, and 241 were new complaints. After honing our labelling strategy and definitions,  176 / 241 complaints were later confirmed upon second review to represent IPFA, in addition to 115 / 118 complaints that were common with manual labelling.
% \jnote{I'm not understanding the previous paragraph. Also wondering if we need this much detail -- in the end, it seems most important how many complaints match the final definition, not sure we need to track matching as the defn evolved}

Using keyword search, we have already found a larger quantity of IPFA examples at a higher rate than from our initial manual labelling efforts. This search method relied on two key assumptions, amongst others:
\begin{enumerate}
    \setlength\itemsep{0em}
    \item The complainant mentions \textit{explicitly} identifies and mentions the abusive behavior of an intimate partner.
    \item The complainant \textit{explicitly} attributes the abusive behavior to an intimate partner and mentions this as the first point / focus of a complaint, hence attributing abuse within a certain textual vicinity of the first mention of an intimate partner. 
\end{enumerate}

These assumptions may not hold in all cases, such as (1) when the pairs of intimate partner and abuse keywords are too restrictive and do not encompass all forms of IPFA, (2) when the complainant is not entirely sure that their intimate partner is financially abusing them, and (3) the complainant is actually a perpetrator of abuse, and hence does not describe their behavior towards an intimate partner as abusive. 

\paragraph{LLMs and Isolating IPFA Complaints.}
Given the simplicity and assumptions of our keyword search method, we leveraged our other tools as seen in Figure \ref{fig:model_pipeline} to identify additional complaints by isolating IPFA. 
Using our existing set of IPFA corpus as our reference set, we deployed our previously described text embedding and clustering tools on subsets of the larger CFPB dataset. To account for the noisiness of our data, we experimented with different levels of preprocessing on CCNs, prior to passing into the modeling pipeline. The details of this can be found in \Cref{tab:experiments}. Running the pipeline on the entire complaints dataset was determined to be prohibitively time consuming. Consequently, we experimented with two different subsets: (1) a 50,359 complaint subset that contains 50,000 randomly sampled complaints, and 359 complaints present in our reference set and (2) a 44,604 complaint subset that contains all complaints in the larger CFPB dataset that mention an intimate partner at least once (using the algorithm mentioned in \Cref{sec:tools}).

In particular, we tested the hypothesis that restricting to IP Complaints (i.e., the top flow in~\Cref{fig:model_pipeline}) improves IPFA yield. In the interest of space, we summarized three experiments testing this hypothesis in~\Cref{tab:experiments}. The two experiments sampling from IP Complaints provide an IPFA yield that is more than twice the experiment that samples from the entire complaint population (a difference that consistently holds across experiments). We describe one of these higher yield experiments (experiment 3) in detail below.

% Experimental Evidence



\paragraph {Assessing Yield.}
%We observe that 
Experiment 3 yielded new IPFA complaints that were not present in our IPFA corpus thus far, and also isolates existing IPFA complaints from our corpus well. We first looked at the proportions of reference set assignments across clusters as an estimator of yield. 

\begin{figure}[!ht]
    \includegraphics[width=\columnwidth, trim={0 0 0 1cm}, clip]{figures/ipfa_approach_simcse.png}
    \caption{The distribution of complaints from our reference set present in the corpus that was clustered in experiment 3. Note the evidently higher proportion of reference set complaints contained in clusters 3, 6, and 7.}
    \label{fig:simcse}
\end{figure}

As seen in \Cref{fig:simcse}, a large proportion of our reference set fell into a few clusters. Notably, we observed that cluster 6 encompasses 54.2\% of this initial set. Clusters 3, 6, and 7 encompass 84\% of this initial set. The other clusters contained very small proportions of IPFA reference set complaints when compared to the aforementioned clusters. Spherical K-Means clustering assigns complaints to the same cluster if they are close (by a particular distance metric) to a common cluster 'center' in vector space. Given that 84\% of our IPFA reference set is contained in a few small clusters, it is evident that LLMs are able to group and isolate IPFA as the text embeddings produced are close in the projected vector space. 

If a set of our reference set of IPFA complaints are close together in the projected vector space, it is sensible to hypothesize that \textit{other} IPFA complaints may also be assigned to the same cluster, if the language and associated text embeddings from LLMs are close to the existing complaints. Upon performing further labelling on a random sample of 500 complaints in cluster 6, we found 123 \textit{new} IPFA examples after review by three total human coders, leaving a yield of 123 / 500 = 24.6\%. Not only does this methodology cluster
%seem to encompass 
complaints identified using previous approaches, but it also finds \textit{new} complaints that express IPFA that were not identified with previous approaches. This demonstrates further how LLMs are able to effectively isolate IPFA complaints, even if they are not fine-tuned on notions of financial abuse.
%could not reveal.


\begin{table}[!ht]
\begin{tabular}{C{.06\linewidth}L{.84\linewidth}}
\toprule
{\scriptsize\textbf{Cluster}} & {\scriptsize \textbf{20 highest scoring cTF-IDF bigrams}} \\
\midrule
% \scriptsize{0} & {\scriptsize{[}`student loans' `student loan' `loan modification' `make payments' `repayment plan' `lost job' `make payment' `payment plan' `monthly payment' `making payments' `mortgage company' `late payments' `monthly payments' `credit score' `credit report' `income based' `years ago' `mortgage payment' `mortgage payments' `received letter'{]}} \\ 
% \midrule
% \scriptsize{1} & {\scriptsize {[}`loan modification' `mortgage company' `mortgage payment' `mr cooper' `mortgage payments' `credit report' `make payment' `customer service' `late fees' `make payments' `monthly payment' `late payment' `escrow account' `received letter' `mortgage loan' `credit score' `short sale' `late payments' `making payments' `credit bureaus'{]}} \\ 
% \midrule
% \scriptsize{2} & {\scriptsize {[}`loan officer' `loan modification' `mortgage company' `short sale' `mortgage payment' `mr cooper' `mortgage loan' `closing date' `title company' `escrow account' `mortgage payments' `credit report' `received letter' `monthly payment' `closing costs' `home loan' `credit score' `real estate' `quicken loans' `customer service'{]}} \\ 
% \midrule
% \scriptsize{3} & {\scriptsize {[}`credit card' `checking account' `customer service' `debit card' `bank account' `account closed' `close account' `savings account' `closed account' `credit cards' `money account' `fraud department' `new account' `business days' `opened account' `card account' `joint account' `account number' `phone number' `new card'{]}} \\ 
% \midrule
% \scriptsize{4} & {\scriptsize {[}`credit card' `credit report' `customer service' `credit score' `did'nt' `received letter' `collection agency' `phone number' `make payment' `did receive' `received email' `card company' `let know' `did want' `days later' `called told' `credit cards' `annual fee' `phone calls' `insurance company'{]}} \\ 
% \midrule
\scriptsize{5} & {\scriptsize {[}`phone number' `cell phone' `stop calling' `phone calls' `times day' `debt collector' `collect debt' `called number' `debt collection' `collection agency' `legal action' `number called' \textbf{`ex husband'} `place employment' `received phone' `personal information' `social security' `phone numbers' `family members' `multiple times'{]}} \\ 
\midrule
\scriptsize{6} & {\scriptsize {[}`credit report' \textbf{`ex husband' `ex wife' `divorce decree'} `credit card' `credit score' `credit bureaus' `filed bankruptcy' `collection agency' `removed credit' `years ago' `credit reports' \textbf{`ex spouse'} `identity theft' `social security' `court order' `credit cards' `authorized user' `credit reporting' `passed away'{]}} \\ 
\midrule
\scriptsize{7} & {\scriptsize {[}`credit reporting' `credit report' `consumer report' `fair credit' `reporting act' `reporting agency' `identity theft' `consumer reporting' `debt collection' `reporting agencies' `credit reports' `collection practices' `fair debt' `credit bureaus' `practices act' `credit card' `section title' `debt collector' `employment purposes' `united states'{]}} \\ 
\bottomrule
\end{tabular}%
\caption{The 20 highest class TFIDF Scored bigrams for clusters 5, 6, and 7. The keywords and phrases related to intimate partners are in bold. Note that most of these phrases are in cluster 6 and all refer to partnerships that have ended (E.g. ``ex husband''). All other clusters had no relevant high scoring words.}
\label{fig:trigram_tfidfs}
\end{table}

%\jnote{Arka, is there a way to show the ``us'' vs ``them'' language variation across the clusters more clearly? Maybe we need more than 20 per cluster? Alternatively, there are some experiments in which we see phrases like ``my husband'' highly ranked in the cluster.}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figures/6_train_explainer.png}
    \caption{The SHAP Explainability Summary for cluster 6 of experiment 3 -- this cluster had the highest proportion of reference set complaints. Note how self-possessive words such as "my", as well as the word "ex" describing a previous intimate partner, weight complaints \textit{towards} being classified as a part of cluster 6. On the other hand, words such as "we" and "us" weight complaints \textit{against} being classified in this cluster.}
    \label{fig:six_shap}
\end{figure}

\paragraph{Assessing Class TFIDF and SHAP scores}
The Class TFIDF scores of experiment 3 provided additional evidence proving the notion that LLMs can isolate IPFA. The highest scoring Class TFIDF words (or n-grams) of a particular class are words that are particularly important to the complaints in that class, or in this case, to the cluster assigned to a set of complaints. As a result, these can be used to determine the traits that describe a particular cluster, and contribute to the regional locality of the text embeddings of complaints in the projected vector space. 

For cluster 6, the cluster with the highest proportion of reference set IPFA complaints, we observed the presence of words describing previous intimate partners ("ex husband", "ex wife", "ex spouse"). Further, we noted that \textit{no} other clusters have such a high density of ex intimate partners in their highest scoring Class TFIDF words. Recall from our definitions that IPFA necessitates a pre-existing trusted relationship. The highest scoring Class TFIDF words included the mention of pre-existing trust relationships, and showed that this aspect of IPFA plays a role in the text embeddings produced by LLMs. 

% †c

SHAP scores are a common explainability metric used in understanding the effect or weight of certain features in a machine learning model's classification. In the case of language modeling, this can involve identifying particular words or phrases that may invoke a \textit{positive} or \textit{negative} weight towards a body of text being assigned a particular class. Further still, in the context of our experiments, SHAP scores were used to give us general benchmarks on the words that have \textit{positive} and \textit{negative} influence on a particular complaint being assigned to it's relative cluster. 

We ran SHAP explainability on cluster 6 from experiment 3 (see \Cref{fig:six_shap}), given the high proportion of reference set complaints in said cluster, and produced a summary showing the 20 words with the highest influences on the classification of a complaint as a part of cluster 6. In doing so, we found that the word "ex" has a high positive impact on multiple complaints as being classified as a part of cluster 6. Recall that from Class TFIDF, we found that complaints in cluster 6 are clustered partly based on the mention of a pre-existing trust relationship -- or more specifically, a former pre-existing intimate partnership. The positive impact of the word "ex" further confirmed this notion, as it often precedes the mention of such an intimate partnership. 

According to our definitions, an abuser's primary motivation for IPFA often involves harming the target, or survivor. If \textit{both} a complainant and their intimate partner are being harmed, we observed that the motivation of harming an IP becomes less clear, and often results in cases where IPFA is not present at all or more difficult to parse. An example of this, from our CFPB dataset is as follows (from complaint 3735484:

\begin{quote}
    \textit{``My husband and I have had a Capital One credit card for several years. Due to the COVID-19 State of Delaware mandates, non essential businesses were ordered closed on XX/XX/20 ... my husband is XXXX and the XXXX  he XXXX  and XXXX  was ordered to shut down indefinitely due to the crisis. We contacted our landlord, utility companies and creditors. We also have several credit cards that are used for personal and business purposes.[...]``}
\end{quote}

The above complaint does not contain IPFA, as a result of both the complainant and their IP being harmed by the financial issue being discussed. In our SHAP summary, we saw that words such as "our", "we", and "us" had negative impacts on a complaint being classified as a part of cluster 6. On the other hand, the possessive word "my" had a positive impact on a complaint being classified as a part of cluster 6. Complaints mentioning words such as "our", "we", and "us", may refer to a complainant and their IP as \textit{both} being financially harmed, and may: (1) fall outside the classification of IPFA according to our definitions or (2) involve IPFA that cannot be easily identified due to the abuse having repercussions for the IP and the complainant. This is clearly reflected in the SHAP scores of cluster 6, and exemplifies the previous notion of inclusionary language, showing that LLMs will be less certain regarding IPFA within complaints where inclusionary language is used, matching our observations and definitions.

\paragraph{Comparing LLM to Keyword Search}
We produce a final IPFA corpus with 527 total complaints -- 135 of these complaints were new complaints found using our LLM approaches (the others coming from manual labelling and our keyword search). Of these new complaints, our keyword search method is only able to flag 2 of them. This means that over 98\% of complaints identified with our LLM approaches were not able to be identified by the previous keyword search, demonstrating that LLM approaches find a wider corpus of IPFA complaints. 

We present a strong body of evidence that LLMs support the isolation and identification of cases of IPFA using LLMs where an IP explicitly harms the complainant. Given this evidence, we think it is important to further study the language-based detection of IPFA with an aim to achieve higher precision and recall in isolating and identifying cases of IPFA. 
\end{comment}

% \begin{figure*}[ht]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccc}
% \hline
% \multicolumn{1}{l}{} &
%   \begin{tabular}[c]{@{}c@{}}Experiment \\ Summary\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}LLM\\ %Used
%   \end{tabular} &
%   \multicolumn{1}{l}{Number of Clusters (K)} &
%   %\begin{tabular}[c]{@{}c@{}}Dataset \\ Used\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Est. IPFA \\ Yield by Cluster\end{tabular} \\ \hline
% 1 &
%   \begin{tabular}[c]{@{}c@{}}
%   \textbf{Sample}: $50K$ randomly selected complaints \\
%   and $359$ IPFA Corpus complaints \\
%   \textbf{Preprocessing}: Removed named entities, punctuation,  \\
%   numbers and stopwords; lemmatized \end{tabular}&
%   %We preprocessed these complaints by removing \\ named entities, punctuation, numbers, and stopwords. \\ Then, we lemmatized and passed the entire processed \\ complaints into the modeling pipeline.\end{tabular} &
%   bert-large-nli-stsb-mean-tokens &
%   20 &
%  % \begin{tabular}[c]{@{}c@{}}50000 randomly selected complaints\\ and 359 high-confidence IPFA complaints\\ from keyword search.\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}} Max: $.1$\\
%  2 clusters: $.02$ \\
%  other clusters: $0$
%  \end{tabular} \\  \hline
%   %2 & \begin{tabular}[c]{@{}c@{}}Random sample of $50,000$ and initial IPA corpus ($n=359$).\\
%  % All complete complaints?\\
% % \end{tabular} &
% % miniLM? & 5 & [\textit{don't need this?}] & %\begin{tabular}[c]{@{}c@{}} Max: $.033$\\
% % 2 clusters: $.033$ \\
% % other clusters: 0
% % \end{tabular} \\ \hline
% %\begin{tabular}[c]{@{}c@{}} 
% 2 &
%   \begin{tabular}[c]{@{}c@{}}
%   \textbf{Sample}: $44,604$ randomly selected \textit{IP Complaints} \\
%   \textbf{Preprocessing}: Removed numbers, redacted content;\\trimmed to $\sim$5 sentence  window around \\ first IP mention \end{tabular} & 
%  %We preprocessed these complaints by removing\\ redacted content and numbers. After, we trimmed \\ each complaint to be a $\sim$5 sentence  window around \\ the first mention of an IP. Then, we passed the trimmed \\ complaints into the modeling pipeline\end{tabular} &
%   sup-simcse-roberta-base &
%   12 &
%   %44464 complaints containing IP keywords &
%   \begin{tabular}[c]{@{}c@{}} Max: $.3$\\
%  2 clusters: $.3$; 1 cluster: $.15$ \\
%  other clusters: $\leq{.05}$
%  \end{tabular} \\  \hline 

% 3 &
%   \begin{tabular}[c]{@{}c@{}}
%   \textbf{Sample}: $44,604$ randomly selected \textit{IP Complaints} \\
%   \textbf{Preprocessing}: None \end{tabular} &
  
%   %We performed no preprocessing on the complaints. \\ Then, we passed the complaints into the \\ modeling pipeline.\end{tabular} &
%   sup-simcse-roberta-base &
%   8 &
%   %44464 complaints containing IP keywords &
%   \begin{tabular}[c]{@{}c@{}} Max: $.26$\\
 
%  other clusters: $\leq{.06}$
%  \end{tabular} \\  \hline 
% \end{tabular}%
% }
% \label{fig:experiments}
% \caption{A summary of 3 experiments instantiating the detection pipeline of Figure~\ref{fig:model_pipeline}. The experiment in row 1 samples from the entire CFPB complaint narrative corpus, while rows 2 and 3 are sampled from the IP Complaints (i.e. complaints that include at least 1 IP term). While all experiments isolate IPFA in a small number of clusters, the latter 2 experiments have an IPFA yield that is more than twice the yield of experiment 1. The third experiment is described in more detail in Section~\ref{sec:evidence}  }
% \end{figure*}


==> sections/deprecated/04aa_analysis_metadata.tex <==
% \paragraph{Corpus metadata.}
% \label{sec:analysis-metadata}
% \anote{Can we shorten this section? (i.e. perhaps we can remove the sentences regarding self selection and distributions across states?}

% this does entail that there acknowledgement of margin for error, this suggests our corpus is thus predominantly 

% % of 283.5 tokens and a median of 196 tokens 
% Complaints in our corpus vary greatly in length, and as a result delve into different levels of detail with regards to a consumer's report of IPFA. Further, we note that most of the complaints in our corpus were submitted between 2018 and 2020 (n = 276, see \Cref{fig:corpus-years}), and see a visual dropoff in IPFA examples in 2021 (n = 145) and prior to 2018 (n = 71). Most of the complaints in our corpus were submitted in the state of California (n = 63), with Florida (n = 41) and Texas (n = 41) being the next most frequent states of submission. \anote{these are the three most populous states in the USA, but not sure if we have enough to describe this as a confirmed relation}.  
% We observe that 21 complainants self-select that the complaint is being filed with regards to an older american, 86 self-select that the complaint is being filed with regards to a servicemember, and 2 being filed as both. The majority of the complaints (n = 404) do not self-select for either criteria. From this, we can identify that within our corpus, IPFA is reported as occurring mainly to complainants who do \textit{not} select/identify as an 'Older American'. This is in line with the fact that abuse within an intimate partner context may occur across age groups, as opposed to being particularly concentrated in older adult populations. \anote{Anything we can say about service members?}
% \ronote{For Arka.}

% {'Older American': 21, 'Older American, Servicemember': 2, 'Servicemember': 86, 'nan': 404}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=0.45]{figures/corpus_graphs/final_corpus_complaint_lengths.png}
%     \caption{Distribution of Complaint Lengths within our Corpus \jnote{how does this compare to the entire CFPB sample?}}
%     \label{fig:corpus-lengths}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%     \includegraphics[width=\textwidth]{figures/corpus_graphs/final_corpus_dates_counts.png}
%     \caption{Number of Complaints Submitted Per Year within our Corpus \jnote{how compares to the whole sample?}}
%     \label{fig:corpus-years}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.45\textwidth}
%          \centering
%     \includegraphics[width=\textwidth]{figures/corpus_graphs/final_corpus_state_counts.png}
%     \caption{Number of Complaints Submitted Per State within our Corpus}
%     \label{fig:corpus-states}
%     \end{subfigure}
% \end{figure}


% \begin{itemize}
%     \item Date complaint submitted (bar chart/year) \url{https://texample.net/tikz/examples/tag/charts/}
%     \item CCN length distribution table incl. of duplicates
%     \item General comment on state distribution
%     \item Proportion of companies, credit bureaus, misc.
%     \item Self-selected tags, Older American, Older American and Servicemember, Servicemember
% \end{itemize}

==> sections/deprecated/04b_analysis_attacks.tex <==
\subsection{RQ2: Commonly reported technology-facilitated attacks}
\noindent 
\edit{Our analysis elicit 23 independent forms of financial attacks across a 24 different technical products, systems and services, where \ref{Figure} shows the distribution of each across our set, many of further validate previously identified attacks in the IPV context \cite{Bellini2023paying, freed_digital_2017, freed2018stalker}.
Overall, complainants described \textit{unauthorized account creation}, \textit{financial negligence}, \textit{identity-related harms}, and, \textit{financial deception} to be the most commonly reported concerns.
In contrast \textit{forgery with respect to cheques}, \textit{unauthorized financial transfers}, and \textit{unauthorized credit report requests} were the least commonly reported.
Here we focus on the under-represented attacks with respect to prior literature, namely that of financial coercion, financial deception, and account takeover for criminal activity.}

\edit{The attacks were independent from each other, however we identified significant dependency between pairs of attacks, namely identity-related harms could also involve unauthorized account creation, while financial negligence could be expressed through failing to remove a complainant from a shared financial asset or dependency.
Overall, we identified that just over half of complaints were dealing with more than one type of attack (50.9\%), with a substantive minority dealing with three or more types of attack (34.7\%).
Namely, complainants reported that there was rarely a single event that constituted an attack, but rather that they were under attack while recovering from a prior attack, or discussing preparing for an imminent one.
In so much, at any point in time, a complainant reported that they could be in one or more stages of financial abuse, highlighting the complexity of multi-layered, and multi-staged nature of even technically unsophisticated technical attacks.}

% \edit{We discover that our analyses validate and extend known financial and technical attacks as reported by Bellini et al.  and Freed et al. \cite{freed2018stalker}, such as \textit{account and device compromise}, \textit{exposure of private information}, \textit{deception}, and, \textit{harassment}.
% In \tabref{tab:attacks}, we categorize these attacks in to five overarching types; \ronote{to fill in when ready....}.}
% Our efforts were able to uncover an entirely new attack; \textit{financial negligence}; the refusal to, reneging or failing to fulfil an established financial agreement. 
% A similar but subtly different form of attack and significantly extend Bellini et al. \cite{Bellini2023paying}'s \textit{financial deception} category. 

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.56]{figures/corpus_graphs/product-prop-bre.png}
    \caption{\small \edit{The proportion of products described in our analysis, which extend to credit, loan, insurance, debt, utilities, payment, claims, mortgage, and online accounts. The label [unspecified] determines that a complainant mentions the high-level category but not the low-level.}}
    \vspace{-0.6cm}
\end{figure}

\paragraph{Financial coercion.} 
We categorize cases where a target describes being coerced or pressured by an IP into a financial action against their will as cases where the attack is carried as financial coercion.
We identified instances where complainants were compelled to perform financial actions, with many describing that they \textit{``complied out of fear''} (1336631) of the consequences.
While the IP was the most common offender, we also identified instances where members of financial organizations either knowingly or unknowingly colluded with an offender:

\begin{quote}
    \textit{''...In the year [redacted], my husband and his colleague forced me into a reverse mortgage against my will. This loan was orchestrated under severe duress for fear of divorce ... the loan officer knew of my objections and the fact that I did not want to sign the loan documents. I had repeatedly expressed my fear and duress about this type of loan...''} (4536981)
\end{quote}

Coercion appeared in several forms within our corpus, such as through threats of legal action or divorce as seen in complaint.
We identified that it was also often associated with another attack or type of IPFA (11 of 12 identified) in many cases.
This can lead to escalating impacts on a target and may be useful for future studies exploring how FSPs can detect IPFA in the future. 

\paragraph{Financial deception.}
Financial deception, as originally identified by Bellini et al. \cite{Bellini2023paying} was a common occurance across this dataset and manifested in many different ways.
Each version of this attack necessitated deceptive and malicious behavior from an offender, from actions that would financially benefit the offender, to ones that facilitate sabotage of a complainant well-being.
In the former example, an offender could trick a complainant into taking on substantive debt in their name under the guise of good intentions:

\begin{quote}
    \textit{``...According to my husband, it would be necessary for me to sign the papers for a HELOC loan ... The entire amount of the loan was deposited in to my husband's account. I had no access to the HELOC account at all ... I have since discovered that the house, mortgage and HELOC are all in arrears ... I was never given a choice...''} (3134442)
\end{quote}

We identified that financial deception can have some overlap with financial negligence, in that deception or lying may play a part \textit{alongside} reverting or refusing to fulfill a previously established financial agreement or obligation. 

\paragraph{Financial negligence.}
Financial negligence, unlike many other forms of attack, necessitate a lack of action on behalf of an offender, often explicitly violating a prior financial agreement between themselves and a complainant.
We identified that such agreements can be both legal in nature (e.g., child support, division of debt in a separation) or informal (e.g., refusing to pay rent, utility bills).
Abuse by financial negligence then, can include attacks ranging from the refusal to cooperate in creating or managing the terms of an agreement in the first place to reverting on a prior established agreement: 

\begin{quote}
    \textit{``...I was court ordered to be responsible for repayment of our consolidated student loans. He will rarely speak with me and I can not submit any documents without my ex-husband of 14yrs signature. This is just NOT POSSIBLE. He is bitter and will not cooperate...''} (Complaint 2417487)
\end{quote}

In this example, an IP refuses to cooperate with the management of student loans knowing of the harm this may incur on a complainant.
Most notably, we saw significant overlap between this form of attack and divorce proceedings whereby there is a legal precedence to \textit{``adhere to stipulations''} (3838460) as one complainant described.

\paragraph{Account takeover.}
\ronote{Arka can you remind me of the example where there were descriptions of an account being taken over for criminal purposes?}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figures/corpus_graphs/product-matrixes.png}
    \caption{\small Top 20 products to financial attack mapping identified from our $n=\set$ complaints. Attacks involving physical and digital credit card  are the most prevalent, while unauthorized opening of account in C's name is the most common attack type in this set.}
    \vspace{-0.6cm}
\end{figure}


\begin{table}[!t]
    \centering
    \input{figures/timelines-processes/tables/attacks-table-3}
    \caption{An overview of new identified financial attacks in the corpus ($n=\set$), organized by high-level category. \ronote{For Arka to finish w/ me}}
    \label{tab:attacks}
\end{table}



==> sections/deprecated/04b_analysis_attacks_new.tex <==
\subsection{Commonly reported technology-facilitated attacks}
\label{sec-analysis-attacks}
\noindent 
\edit{Our analysis elicited 23 independent forms of financial attacks across 24 different technical products, systems, and services, where~\cref{fig:attack-product-matrices} shows the distribution of each across our set, many of which further validate previously identified attacks in the IPV context \cite{Bellini2023paying, freed_digital_2017, freed2018stalker}.
Overall, complainants described \textit{unauthorized account creation}, \textit{financial negligence}, \textit{identity-related harms}, and \textit{financial deception} to be the most commonly reported concerns.
In contrast, \textit{forgery with respect to cheques}, \textit{unauthorized financial transfers}, and \textit{unauthorized credit report requests} were the least commonly reported. 
}
We focus on the technical attacks that are underrepresented in prior literature, namely that of financial coercion, financial negligence, financial deception, unfair attribution, and access + control for criminal activity.\jnote{I expected to see coercion, deception and AT as the paragraphs below, but they are different. Can we align?} While these attacks are distinct, we identified co-occurrences between certain attacks from different attack types; harm from financial negligence could also occur with deceiving a complainant regarding an offender's willingness to pay off an assigned debt, and unauthorized access to accounts can result in a complainant being held responsible for newly accrued debt. 

% \edit{While these attacks are distinct, we identified dependencies between pairs of attacks; identity-related harms could also involve unauthorized account creation, and financial negligence could be expressed through failing to remove a complainant from a shared financial asset or dependency. \jnote{In the previous sentence it seems like we are saying financial coercion, deception and account takeover have dependencies between them but that is not what follows. Can the author clarify the sentence?}

% All in all, just over half of complaints contained more than one type of attack (50.9\%), with a substantive minority dealing with three or more types of attack (34.7\%). Namely, in cases where more than one attack was identified, complainants described these as occurring consecutively without an opportunity to recover. \anote{Is there an example we can provide for the above?}

% was rarely a single event that constituted an attack, but rather that they were under attack while recovering from a prior attack, or discussing preparing for an imminent one. \knote{This previous sentence is clunky. Also, if I'm reading correctly, 100\%-50.9\% = 49.1\% isn't ``rarely'' }
% In so much, at any point in time, a complainant reported that they could be in one or more stages of financial abuse, highlighting the complexity of multi-layered, and multi-staged nature of even technically unsophisticated technical attacks.
\begin{table}[!t]
    \centering
    \input{figures/timelines-processes/tables/attacks-table-3}
    \caption{An overview of identified financial attacks in the ($n=\set$), organized by the relevant financial process the attack might involve and the type of attack present.}
    \label{tab:attacks}
\end{table}

We characterize \textit{new} attacks identified in our analysis in \Cref{tab:attacks} by the type of attack and the processes within a financial institution an attack may involve. In doing so, we identify the possible areas within financial systems that may be studied further to understand particular types of attacks as described within our corpus.

% \edit{We discover that our analyses validate and extend known financial and technical attacks as reported by Bellini et al.  and Freed et al. \cite{freed2018stalker}, such as \textit{account and device compromise}, \textit{exposure of private information}, \textit{deception}, and, \textit{harassment}.
% In \tabref{tab:attacks}, we categorize these attacks in to five overarching types; \ronote{to fill in when ready....}.}
% Our efforts were able to uncover an entirely new attack; \textit{financial negligence}; the refusal to, reneging or failing to fulfil an established financial agreement. 
% A similar but subtly different form of attack and significantly extend Bellini et al. \cite{Bellini2023paying}'s \textit{financial deception} category. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[scale=0.56]{figures/corpus_graphs/product-prop-bre.png}
%     \caption{\small \edit{The proportion of products described in our analysis, which extend to credit, loan, insurance, debt, utilities, payment, claims, mortgage, and online accounts. The label [unspecified] determines that a complainant mentions the high-level category but not the low-level.} \jnote{what does 'generic' mean here?}}
%     \vspace{-0.6cm}
% \end{figure}

\paragraph{Coercion and Duress.}
Often, complainants are coerced into performing certain financial actions and / or are harmed by an offender who capitalizes on the stressors they are facing. A majority of these cases involved the offender leveraging threats (e.g., a threat of separation, a threat of legal action). We also saw offenders leveraging fear of facing other forms of abuse, as well as the restriction of financial capital to force complainants to cooperate. While coercion can be hidden from many of a financial institution's processes, we saw evidence of these attacks being surfaced in complainants' direct interactions with a financial institution's representatives (e.g., during a branch visit, support call, or in complaint narratives). Notably, we observed that cases of coercion and duress may be accompanied with mention of the emotional toll attacks of this form can have, with descriptions such as how the complainant \textit{``complied out of fear''} (1336631) of the consequences. The mention of emotional toll can reveal the possibility of coercion in the various forms of interaction with an FSP, and is already leveraged as a possible indicator in cases of elder financial abuse \cite{add citation}.

While the intimate partner was the most common offender, we also identified instances where members of financial organizations either knowingly or unknowingly colluded with an offender, particularly in direct interactions between the customer and a representative:

\begin{quote}
    \textit{``...In the year [redacted], my husband and his colleague forced me into a reverse mortgage against my will. This loan was orchestrated under severe duress for fear of divorce ... the loan officer knew of my objections ... I had repeatedly expressed my fear and duress about this type of loan...''} (4536981)
\end{quote}

We identified that attacks involving coercion and duress were often associated with another attack or type of IPFA (11 of 12 identified), exemplifying how these attacks can be just one in a chain of attacks the complainants mention. 

% \paragraph{Negligence}
\paragraph{The intricacies of financial negligence: violations, agreements, and ownership in abusive contexts.} Financial negligence, unlike many other forms of attack, can necessitate a lack of action on behalf of an offender, often explicitly violating a prior financial agreement between themselves and a complainant.
We identified that such agreements can be both legally binding (e.g., child support, division of debt in a separation) or informal (e.g., refusing to pay rent, utility bills).
Abuse by financial negligence then, can include attacks ranging from the refusal to cooperate in creating the terms of an agreement in the first place (``\textit{he will rarely speak with me and I can not submit any documents without my ex-husband of 14yrs signature}``, 2417487) to reverting on a prior established agreement (\textit{``Since my ex husband was not taking care of his half of the debt...``}, 1854030).
Most notably, we saw significant overlap between this form of attack and divorce proceedings whereby there is a legal precedence to \textit{``adhere to stipulations''} (3838460) as one complainant described. 
Many agreements, particularly as a result of legal separation, also came with notions of ownership around a particular asset or debt, such as being \textit{``awarded property``} (1369215). Negligence occurred along with questions about ownership; processes surrounding asset and debt ownership became an evident realm of a financial institution's services that this form of abuse interacts with. For instance, we observed that complainants often face harm from this type of attack \textit{because} they are still held liable when they view that they shouldn't be, whether that misunderstanding be related to a financial institution's policy or inaccuracies around ownership after settling on an agreement:
\begin{quote}
    \textit{``My ex husband and I had a joint account at [redacted]. He agreed to take the account and the debt in our divorce agreement. [redacted] is refusing to remove me as a joint account holder although I am no longer legally responsible for any debt incurred on that account from the date of separation...''}
    (3425863)
\end{quote}

\paragraph{Deception.}
Financial deception, as initially identified by Bellini et al.\cite{Bellini2023paying}, exhibited various manifestations in our dataset (n = 47), all of which necessitated deceptive and malicious behavior from the offender. These actions encompassed behaviors that aimed to financially benefit the offender, as well as ones that would undermine the well-being of the complainant.
In an example of the former, an offender could trick a complainant into taking on substantive debt in their name under the guise of good intentions:

\begin{quote}
    \textit{``...According to my husband, it would be necessary for me to sign the papers for a HELOC loan ... The entire amount of the loan was deposited in to my husband's account. I had no access to the HELOC account at all ... I was never given a choice...''} (3134442)
\end{quote}

We found that deception can overlap with negligence. That is, deception or lying may play a part in the refusal to create or fulfill a financial obligation. We observed one complainant dealing with the unfortunate circumstance of an offender who (``\textit{wrote me a few checks for a very small amount to begin to pay me back... After that he disappeared...}``, 3764702). Like coercion and duress, deception occurs most often alongside another form of attack within our corpus (39/47), showing that it may also play a part in a chain of financial attacks on a complainant. Some complainants described attacks involving deception resulting in the unwanted ownership of an asset or debt (as seen in 3134442). We also observe that deception can often reflect in the asset or account behaviour of a complainant, such as when a complainant's funds are stolen with a promise of returning (as seen in 3764702). 


\paragraph{Unfair Attribution.}
Financial attacks involving unfair attribution are unique in that the offender \textit{actively} opens or assigns a financial asset or debt in a complainant's name (without the presence of a financial agreement). These types of attacks have been identified previously by Bellini et. al \cite{Bellini2023paying}, but we saw new forms of attribution such as disputing valid transactions to create unanticipated debt (``I allege my ex-wife fraudulently processed a chargeback on prior payments made on my lease to [redacted]...``, 3356032).
In addition, one complainant describes unfair attribution where an offender uses the complainant's financial assets to carry out fraudulent activity on \textit{other parties}, thereby leaving the complainant responsible for any subsequent repercussions when that activity is reported:
\begin{quote}
    \textit{``It came to my attention recently that an ex-girlfriend had fraudulently used my [redacted] credit cards... The fraud included a gentleman facilitating phone calls and posing as me... About three days later, [redacted] called and said that since i had been a beneficiary of the fraud, even though it was unknowingly, they could not substantiate it as fraud.''(2349007)}
\end{quote}

Unfair attribution deals largely with asset and debt ownership, in addition to a financial institution's fraud/dispute policies. As seen in 3356032, chargebacks are a possible point of interaction between complainants and a financial institution when attacks of this type occur.

\paragraph{Access + Control.}
Like deception and unfair attribution, attacks dealing with access and control have been identified previously \cite{Bellini2023paying}. In our corpus, complainants describe new forms of attacks in this realm, such as an offender leveraging existing fraud policies to block a complainant's access (``\textit{I went thru a traumatic divorce, so my ex-wife did fraudulent checks on my account and the bank put a freeze on my accounts.}``, 48835804). 
% \begin{quote}
%     \textit{``I went thru a traumatic divorce, so my ex-wife did fraudulent checks on my account and the bank put a freeze on my accounts. My accounts were in Colorado. I was out of state on business and the bank called, so they froze my account, fast forward I moved to [redacted] to start a new life but I end of losing my house and became homeless because I did not have access to any of my accounts. '' (4883504)}
% \end{quote}
We also observe offenders interacting directly with financial institutions through impersonation or social engineering to gain access to a complainant's account information (``\textit{My ex husband used the automated IVR phone system for [redacted] to obtain my current credit card balance and last payment information to use against me.}``, 4096714). As identified in prior literature, attacks relying on impersonation leveraged the fact that an offender \textit{already} knows a complainant's personal information (\textit{`` He knew my phone number, address and last 4 of SSN to use the automated system to obtain information he is not authorized to access...``}, 4096714), allowing for what \textit{seems} like authenticated and valid behavior from the perspective of the financial institution. Attacks involving unauthorized access or control can reflect in the information release and authentication processes followed by financial institutions, and draws attention to the importance of studying this form of compromise further in a financial context. 


% \paragraph{Financial coercion.} 
% We categorize cases where a target describes being coerced or pressured by an IP into a financial action against their will as cases where the attack is carried as financial coercion.
% We identified instances where complainants were compelled to perform financial actions, with many describing that they \textit{``complied out of fear''} (1336631) of the consequences.
% While the IP was the most common offender, we also identified instances where members of financial organizations either knowingly or unknowingly colluded with an offender:

% \begin{quote}
%     \textit{''...In the year [redacted], my husband and his colleague forced me into a reverse mortgage against my will. This loan was orchestrated under severe duress for fear of divorce ... the loan officer knew of my objections and the fact that I did not want to sign the loan documents. I had repeatedly expressed my fear and duress about this type of loan...''} (4536981)
% \end{quote}

% Coercion appeared in several forms within our corpus, such as through threats of legal action or divorce as seen in complaint.
% We identified that it was also often associated with another attack or type of IPFA (11 of 12 identified) in many cases.
% This can lead to escalating impacts on a target and may be useful for future studies exploring how FSPs can detect IPFA in the future. 

% \paragraph{Financial deception.}
% Financial deception, as originally identified by Bellini et al. \cite{Bellini2023paying} was a common occurance across this dataset and manifested in many different ways.
% Each version of this attack necessitated deceptive and malicious behavior from an offender, from actions that would financially benefit the offender, to ones that facilitate sabotage of a complainant well-being.
% In the former example, an offender could trick a complainant into taking on substantive debt in their name under the guise of good intentions:

% \begin{quote}
%     \textit{``...According to my husband, it would be necessary for me to sign the papers for a HELOC loan ... The entire amount of the loan was deposited in to my husband's account. I had no access to the HELOC account at all ... I have since discovered that the house, mortgage and HELOC are all in arrears ... I was never given a choice...''} (3134442)
% \end{quote}

% We identified that financial deception can have some overlap with financial negligence, in that deception or lying may play a part \textit{alongside} reverting or refusing to fulfill a previously established financial agreement or obligation. 


% \paragraph{Account takeover.}
% \ronote{Arka can you remind me of the example where there were descriptions of an account being taken over for criminal purposes?}

==> sections/deprecated/04c_finding_traits.tex <==
\section{Identifying Traits of IPFA}
\label{sec:findings}
%%JS: removed 'findings'; don't want reviewers to think this is the only section with novel contributions
We used tools from~\Cref{sec:data_tools} to understand the dominant attributes, or \textit{traits}, in the IPFA corpus built using the iterative pipeline in~\Cref{sec:isolating}.
%In our entity analysis, we find that the top 12 words mentioned in our final The most prevalent noun entities in the IPFA corpus are: 
We found that the top 12 entities mentioned in the IPFA corpus are: \textit{credit, account, name, report, time, debt, year, card, information, payment, divorce, and loan}. Each  entity was mentioned at least once in a minimum of 144 unique complaints. We used this, along with dependency parsing and Topic Modeling to identify the dominant IPFA traits  mentioned by complainants in our final IPFA corpus. Dependency parsing (see \Cref{tab:ipfa_corpus_triples}), highlights the most frequently mentioned root verb and object  related to  an intimate partner within a unique complaint. This parsing provided insight into  the different actions intimate partners took in the IPFA corpus, as well as the entities being affected by this action. Paired with entity analysis, this provided valuable understanding into common abuse / vectors in the IPFA corpus. 

\input{figures/topic_modelling}

% \anote{do i need to mention parameters for Topic Modeling here? Or is it mentioned previously alread? - arka please look at htis - arka}
\begin{comment}
Topic modeling the individual sentences within each IPFA complaint using LLMs surfaces latent topics in the IPFA corpus. These latent topics give us insights into the different types of statements being made by complainants when describing complaints involving IPFA, and hence give us insight into co-occuring traits and attributes of IPFA complaints within this corpus. We highlight a few of the key takeaways using this set of tools below. 

\anote{is the above good or needs more work? - arka look tomorrow - note - arka}
\jnote{The Topic Modeling paragraph seems redundant. Can we replace some of the text with examples of the statements/traits?}
\end{comment}


\subsection{Types of Financial Attacks}
In our analyses we identified that opening unathorized accounts and refusing to uphold financial agreements were the primary mechanisms that adversaries inflicted financial abuse on survivors. 
Unauthorized opening of accounts hold common links with identity-related crimes (e.g., `identity theft' \cite{moskovitch2009identity}), but we drew out distinctive elements that helped reinforce new found capabilities of adversaries.

\paragraph{Opening unauthorized accounts.} In our dependency parsing (see \Cref{tab:ipfa_corpus_triples}), four out of the six top triples mentioned in our IPFA corpus addressed an intimate partner opening some form of an account without the complainant's permission. Authorized accounts opened without a complainant's permission, if allowed to be overdrafted or go into negative balance, can result in action taken by institutions for collecting on said debt. If this account was opened in a complainant's name, this collection typically falls on the complainant, and also harms a complainant's credit score. 

% \paragraph{Opening unauthorized credit cards.} 
Similar to opening accounts, we found one triple referring to an intimate partner opening a card, and is the third most frequently mentioned entity in our IPFA corpus. Opening credit cards can cause multiple levels of harm. Foremost, a complainant's credit score is harmed by the initial opening of a new credit card. Second, outstanding debts that are left unpaid on these credit cards result in an additional decrement in credit score. These two elements together can prevent victims of this form of IPFA from opening or utilizing their credit for any future financial obligations, having both short and long term impacts.  

\paragraph{Taking out loans in a target's name.} Like credit cards and accounts, taking out unauthorized loans was a common vector of abuse, given how "debt" and "loan" appeared in our top 12 entities mentioned across complaints, and how prevalent the mentioning of "opening" assets was in our dependency parsing. Similar to previous categories, the harms of unauthorized loans involve unsolicited debt collection, and large impacts on a complainant's credit score.


\paragraph{Withholding capital from previous fiscal responsibilities.}
Divorce appeared in our top 12 entities mentioned in complaints, and is often the source of legal agreements regarding finances from a previous intimate partnership. In our Topic Modeling experiment, we found an isolated cluster of sentences that primarily discussed divorce or forms of separation (cluster 8). Within this cluster of sentences, we often observed complainants mentioning an intimate partner refusing to fulfill a financial responsibility or agreement that was settled previously. Although the act of opening various forms of assets without a complainant's permission or knowledge causes harm in numerous ways, it is evident that rejecting previously agreed upon fiscal responsibilities is common form of IPFA. This is most often observed, as in our Topic Modeling, in the case of legal agreements reached during divorce or separation, where the joint financial assets of an intimate partner and the complainant are split up, but an intimate partner refuses to fulfill their end of the agreement (e.g. child support payments, taking responsibility for previous joint accounts, paying off previously accrued debts). 

\begin{table}[!ht]
\centering
\small
\begin{tabular}{C{.2\linewidth}C{.22\linewidth}C{.2\linewidth}C{.18\linewidth}}
\toprule
First Word & Second Word & Third Word & Count \\
\midrule
husband & open  & account  & 21 \\ 
wife    & open  & account  & 17 \\ 
wife    & open  & card     & 12 \\ 
spouse  & open  & account  & 10 \\ 
husband & steal & identity & 10 \\ 
account & open  & husband  & 9 \\
\bottomrule
\end{tabular}
\caption{Frequency of the top 6 triples of IP, Verb, and Related Object from dependency parsing on our final IPFA corpus. A majority of the triples involve opening assets.}
\label{tab:ipfa_corpus_triples}
\end{table}

\subsection{Targets, Risks and Impact}
Our CCN were rich sources of information that allowed us to better understand the contexts of intimate adversaries.
We identified that there were common targets that intimate adversaries consistently targeted, the risk of this happening during divorce proceedings was acute, and had a significant impact on a survivor. 

\paragraph{Targets: Credit, Bank Accounts, Loans, and Cash.}
In our analysis, we identified that credit cards, bank accounts, loans, and household related expenditure are common targets for adversaries. 
As mentioned previously, we observed that 5 of the 12 most commonly mentioned financial entities in our IPFA corpus were: \textit{credit, account, report, debt, and card}. We further observed the prevalence of housing-related financial responsibilities (such as mortgages and rent) in IPFA complaints with topic modelling (see cluster 9). The isolation of such a cluster of sentences from IPFA complaints showed that complainants often mentioned forms of mortgages and housing-related financial responsibilities in IPFA complaints, showing its importance as a commonly impacted entity. Further, some of these impacted entities, such as account and card, aligned with our previous findings regarding common vectors of IPFA within our corpus. Together, this set of entities highlighted the importance of further focus on securing assets in these categories. 

\paragraph{Risks: Divorce or Separation.}
From topic modelling, we observed an isolated cluster (8) describing cases of divorce in our IPFA complaints. Paired with the fact that 'divorce' was one of the most frequently mentioned entities within our IPFA corpus, this demonstrated the importance of considering divorce / separation of a survivor and intimate partner as a potential co-occurring trait with IPFA. Previously, we highlighted how one way IPFA occurs is through the refusal by an intimate partner to adhere to agreed-upon fiscal responsibilities. One common source of these fiscal responsibilities came from legal requirements as set out by divorce decrees. An example of this is a sentence present in our cluster of interest from complaint 4823719: 

\begin{quote}
   \textit{ "Furthermore, I have produced the divorce documents stating that my ex-wife, ( name redacted per your request ) takes full responsibility for addressing the balance of the \redact{Discover} Card.". }
\end{quote}

In this case, the complainant was describing the responsibility of debt for an unauthorized credit card opened by their IP. Being able to leverage this co-occurrence may prove valuable for future systems detecting and mitigating IPFA, as it can provide vital context regarding unpaid debts that are harming a survivor. 

 \paragraph{Impacts: Financial and Emotional Toll.} In our Topic Modeling, we observed two clusters (10 and 14) that consisted of sentences describing the distress and toll financial harm was having on the complainant. Requests for help were common in the sentences within these clusters, such as the following from complaint 4823719: 

\begin{quote}
 \textit{"Please, I beg your agency to use a modicum of discernment regarding this circumstance."}
\end{quote}

Upon further analysis of these clusters, we observed the harms of IPFA often extending beyond the complainant to other individuals the complainant has a relationship with, such as a child. For example, one sentence from complaint 3022607 stated: 

\begin{quote}
\textit{"The people involved are myself, [redacted] and my children, [redacted], and [redacted], all of which had to suffer because of this hardship."}.
\end{quote}

This clearly describes the harm IPFA has had not just on the complainant, but also on the complainant's children. Similarly, accounts opened by the complainant's previous intimate partner in complaint 5428002 had resulted in debt collection efforts that culminated in distressing calls to the complainant's mother:

\begin{quote}
\textit{"I called [redacted-organization] and told them about they sent information to my mothers house that lives like almost a hour away and she opened the letter and feared for my life because of the threats."}
\end{quote}

The distress and emotional toll of IPFA is evidently significant, and re-enforces the importance of being able to detect and mitigate its propagation through the enforcement of secure practices. Further, being able to identify these notions of toll can be valuable for detecting cases of IPFA within verbal and textual customer interactions with financial representatives, and should be considered for the development of future detection systems. It is also clear that hardship from IPFA can extend beyond just the complainant, and create situations where the complainant deals with multiple levels of harm in the long term. Future systems and methods of mitigation should therefore focus not only on securing the financial assets of a survivor, but other trusted parties involved with the survivor. 

==> sections/notes.tex <==
% Security advice 
They denied my claim when they shouldnt be able to let anyone take out money they dont have in their bank account (5174599)
Charged thousands for frauduluent transactions 
to me that my " signature was not required '' and the debt is " mutually yours (33421816)

the clerks on the phone are uninformed and no past record or notes are available to them from my many phone conversations and paperwork I had sent to them. I have to continually restate my grievances and request information on why the account is delinquent (2098427)

the clerks on the phone are uninformed and no past record or notes are available to them from my many phone conversations and paperwork I had sent to them. I have to continually restate my grievances and request information on why the account is delinquent (2829475)

I didn't authorize at all I contact chase to tell them and they said take it up with her (3601686)

Evidence 
Court docs (3187582)
I've included some of the documents I receive on a regular basis regarding the charges I have taken out on my [redacted] to further solidify my identity as a victim of [redacted] in many forms, financial [redacted] being one of the many (4288879)
I informed Capitol One of these issues by phone and letter on multiple occasions in [redacted]. I called and wrote letters and provided a then report of identity theft that was filed through the Federal Government Identity Theft Site that detailed what happened. I offered documentation and spoke to them about it. (3237644)
have sent supporting documents to [redacted], [redacted], [redacted] concerning this matter. (2799518)

This account was opened by my ex husband without my authorization and I have filed an identity theft report with the FTC that outlines this account. The Bank will not talk to me about this account because it is not in my name, so why do they continue to report it to my credit file? (3937452)
